ABC: A Simple Explicit Congestion Controller for Wireless Networks

We propose Accel-Brake Control (ABC), a simple and deployable explicit congestion control protocol for network paths with time-varying wireless links. ABC routers mark each packet with an "accelerate" or "brake", which causes senders to slightly increase or decrease their congestion windows. Routers use this feedback to quickly guide senders towards a desired target rate. ABC requires no changes to header formats or user devices, but achieves better performance than XCP. ABC is also incrementally deployable; it operates correctly when the bottleneck is a non-ABC router, and can coexist with non-ABC traffic sharing the same bottleneck link. We evaluate ABC using a Wi-Fi implementation and trace-driven emulation of cellular links. ABC achieves 30-40% higher throughput than Cubic+Codel for similar delays, and 2.2X lower delays than BBR on a Wi-Fi path. On cellular network paths, ABC achieves 50% higher throughput than Cubic+Codel.

==> challenges.tex <==
\section{Challenges}
\label{s:challenges}

Any explicit flow control schemes has to solve three challenges 
\begin{enumerate}
    \item \textbf{Deployability/Middleboxes/Endhost stack changes}: \pg{I think end host modification is a big point. If we wanted phones to use XCP, then the entire stack would have to be modified to support it. If we included XCP feedback as payload in packets then all the applications would require modifications.}
    \item \textbf{Coexistence with other bottlenecks}
    \item \textbf{Coexistence with non-explicit flows}
\end{enumerate}



==> deployment.tex <==
~\section{Deployment with ECN}
\label{s:deployment}
We now describe two deployment options for \name{}. We begin with a brief review of standard ECN~\cite{ecn-rfc}, which our scheme builds on. Then we discuss how to deploy \name{} in networks without legacy ECN in the routers. In this case, we can deploy \name{} without any modifications to TCP receivers, i.e., mobile phones can take advantage of \name{} for download traffic without any software changes.\footnote{The transport stack on mobile phones of course needs to change to use \name{} for upload traffic.} Finally, we present a way to deploy \name{} that is compatible with legacy ECN but requires a simple modification to TCP receivers.

\smallskip
\noindent {\bf Standard ECN:}
IP packets have two ECN-related bits: ECT and CE. These two bits are traditionally interpreted as follows
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & ECN-Capable Transport ECT(1)\\
 1 & 0 & ECN-Capable Transport ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
Routers interpret both (01) and (10) for these bits to indicate that the connection is ECN capable. To mark a packet with ECN, a router changes the bits to (11). Upon receiving an ECN mark (11), the receiver sets the {\em ECN Echo (ECE)} flag in {\em all} subsequent ACKs until it receives a {\em Congestion Window Reduced (CWR)} notification from the sender, \ie a packet with the CWR flag in the TCP header set to 1. Thus receivers echo ECN marks for a full round-trip worth of ACKs. 

\smallskip
\noindent{\bf No legacy ECN:}
Many cellular networks use {\em TCP proxies} to split connections at the network boundary~\cite{wang2011untold, ravindranath2013timecard}. The operators of such networks can easily disable ECN on the routers inside the cellular network. This allows a straight forward deployment of \name{}. \name{} senders simply use either (01) or (10) for \textit{accelerate} and routers use (11) to indicate \textit{brake}. We evaluate two designs, with and without and receiver modification, such that for a packet the receiver echoes back the ECN bit only once. We implemented both versions in linux as a kernel module using the pluggable TCP API.

\textit{With receiver modification:} Using the pluggable TCP API we modified the receiver such that it simply echoes back the ECN bit once and doesn't wait for CWR from sender. The receiver behaviour is identical to that of dctcp~\cite{dctcp}. We use this version of TCP implementation in all the experiments in this paper.

\textit{Without receiver modification:} To ensure that the receiver conveys accelerate/brake signals accurately, we modified the kernel such that the sender sets the CWR flag on {\em every} packet. This ensures that the receiver echoes a brake exactly once (instead of for a full RTT), assuming all packets are acknowledged and ACKs are not lost. More accurate ECN feedback mechanisms in the presence of delayed/lost ACKs have been proposed~\cite{accurate-ecn}, which require receiver modifications. \name{} can also leverage these techniques.

Appendix ~\ref{app:cwr} compares throughput and $95^{th}\%$ile per-packet delay of the two TCP variants on 8 cellular traces. Both the variant's achieve similar throughput and delay (within 1\% of each other) averaged across the traces.

\smallskip
\noindent{\bf With legacy ECN:}
\name{} can coexist with legacy ECN by reinterpreting the ECT and CE bits as follows
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & \textit{accelerate} ECT(1)\\
 1 & 0 & \textit{brake} ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
The \name{} sender begins with (01) on every packet ({\em accelerate}). An \name{} router can signal {\em brake} by flipping the bits to (10). For legacy routers, both (01) and (10) are equivalent and indicate ECN capable transport. Thus a legacy routers can simply use (11) to signal congestion, exactly as in standard ECN. Finally, the receiver can distinguish between accelerate (01), brake (10) and ECN set (11). 

The receiver must convey both standard ECN and accelerate/brake for \name{}. We can use the ECE flag for ECN feedback. For \name{} feedback, we can reuse the NS (nonce sum). The NS bit was originally proposed to ensure integrity of ECN feedback~\cite{nonce}, but this feature has since been reclassified as historic~\cite{accurate-ecn} since it was never deployed. Therefore, we can repurpose the NS bit for \name{}'s feedback. Using this scheme, the sender can react to drops/ECN marks same as standard TCP.

\name{} routers do not interfere with the proper operation of ECN for standard TCP flows. All TCP implementations transmit packets with ECT/CE set to (10)  to indicate ECN-capable transport. Since \name{} only converts ``accelerate'' (01) to ``brake'' (10), it will ignore any packet marked with (10). As a result, there is no need for senders to convey \name{} capability in packet headers.

Note that any internal encryption used by the cellular network provider does not hinder the \name{} router's ability to modify ECN bits. The \name{} router (base station or mobile phone) is typically the location where any form of in-network encryption is removed, which means that the \name{} router will have access to the unencrypted packets and can modify the ECN bits.

A potential vulnerability of the above scheme is that a malicious router on the path can convert a brake to an accelerate. However, we can easily detect this at the senders by sending packets marked with brake once in a while; if any of these packets return with accelerate, then there are malicious entities on the path. 


==> design.tex <==
\section{Design}
\label{s:design}

The bottleneck \name router uses estimates of the link rate, the queuing delay and the sender's current dequeue rate to calculates a target rate. The router uses single bit of per-packet to signal an increase (accelerate) or decrease (brake) it's rate to achieve the desired target rate.

\subsection{\name Sender}
\label{s:abc-sender}
\textbf{Sender's window update rule:} On receiving an ``accelerate'' in an ACK, the sender increases its congestion window by 1, and sends out two packets, one in response to the ACK and one foe increase in congestion window. On receiving a ``brake'', the sender reduces it congestion window by 1, and a result it doesn't send out a packet to replace the packet corresponding to the received ACK. The intuition for \name can be drawn from a car on a busy road, the driver of the car and can either accelerate/brake. The driver uses these two actions in quick succession to maintain a desired car speed. 

When the single bit feedback is aggregated over a duration (e.g., an RTT) the feedback becomes quite expressive. If the sender's current congestion window is $w$, and the router marks accelerate with probability $f$, then the receiver will receive $w$ ACKS. Out of these $w$ ACKS, $w$ . $f$ will be accelerates and the remaining $w$ - $w$ . $f$ ACKs will be brakes. Congestion window in the next round will be 2 . $w$ . $f$. In case of delayed ACKs, we use a byte based solution that increases/decreases congestion window by new bytes ACKed on receiving an accelerate/brake in the ACK.

If the router selects $f = 0$, then the transmission will be throttled with 1 RTT. If the router selects $f = 1/2$, then the sender will maintain it's current window, if the router uses $f = 1$, then the sender will receive receive accelerate and increase its congestion window by 1, doubling its congestion within 1 RTT akin to slow start. So the router can vary sender's rate from 0 to twice the current window withing 1 RTT, providing a dynamic range for accurate and fast adaptation to variations in link capacity.

\textbf{Starting Condition:} Each packet starts with an accelerate marked on it. A router can change an accelerate to a brake, not vice versa. Thus by default the behaviour corresponds to that of slow start. This situations stops when the current dequeue rate at the router starts approaching the target rate. Routers are not allowed to change a brake to an accelerate , the reason that an \name router can unilaterally decide to reduce rate, but acceleration requires consensus along the path. We discuss multiple bottlenecks in detail in the forthcoming sections in the paper.

\subsection{\name Router}
\label{s:abc-router}

\textbf{Target rate:} The \name router determines the target rate, $tr(t)$, using the link capacity $\mu(t)$ and the queuing delay $x(t)$, using the rule

\begin{equation}
tr(t) = \eta {\mu(t)} - \beta \frac{\mu(t)}{\delta} (x(t) - d_{t})^{+}.
\label{eq:abctargetrule}
\end{equation}

This control rule is inspired from ideas in earlier works. First, similar to TUB from ATM networks ~\cite{jain1996congestion}, AVQ~\cite{avq}, and
HULL~\cite{hull}, ABC sets $tr(t)$ to $\eta . \mu$, where $\eta < 1$ represent target utilization. This allows \name flows to operate just below the link capacity, trading a little bandwidth for significant reductions in delay. This approach works because \name doesn't requires senders to fill the queues to estimate the link capacity. Note that for Cellular and networks with user isolation (per-user queuing), the target rate is calculated separately for each user using the per-user link capacity and queuing delay. 

The target rule above is not sufficient as there is a 1 delay of 1 RTT in feedback to the sender. Moreover, inaccuracies in estimation can lead to transient queues. We add a second term to the rule to drain out any stagnant queues. The router
reduces the target rate, if the queuing delay, $x(t)$ exceeds a delay threshold, $d_{t}$
(the notation $y^{+}$ is defined as $\max(y,0)$). The reason is that wireless systems exhibit non deterministic service times (e.g., batching of packet in WiFi), as a result any packet arrival process will observe some queue build up.  A non-zero delay threshold $d_{t}$ ensures that the target rate does not react to minor delay fluctuations. The value of $d_{t}$ could, in principle, change with time, but ABC currently uses a static value for simplicity.

The target rate calculation in Eq.~\ref{eq:abctargetrule}, requires an estimate of the link capacity ($\mu$). In ~\Sec{wifi} we present a method for estimation the link capacity on WiFi MAC 802.11 n. In cellular networks, because the scheduler manages all the traffic, it knows exactly what resources have been allocated to each user and can thus calculate per user link-capacity. Note that the scheduler also guarantees fairness between users while allocating resources; ABC does not affect inter-user fairness.

Equation (~\ref{eq:abctargetrule}) has three constants, $\eta$, $\beta$, and $\delta$, which govern the stability of the scheme. $\delta$ should be on the order of one RTT; since the router does not know the RTT precisely, we use 100 ms in our tests. $\beta$ governs how quickly queues drain. We do not explicitly establish the stability conditions of Eq. (~\ref{eq:abctargetrule}) here, but prior methods ~\cite{xcp, rcp} apply.

\textbf{Packet marking:} To achieve the target rate, $tr(t)$, the router measures the current dequeue rate, $cr(t)$, and calculates the fraction of packets,
$f(t)$, that remain marked as ``accelerate'' using the following rule:
\begin{equation}
f(t) = \min\Big\{\frac{1}{2} \cdot \frac{tr(t)}{cr(t)}, 1 \Big\}.
\label{eq:f}
\end{equation}

The \name{} router ensures that no more than a fraction $f(t)$ of packets have the ``accelerate'' indication set. The pseudocode for the packet marking algorithm is shown below.

\begin{algorithm}[h]
\SetAlgoLined
\caption{Packet marking at an \name{} router. The exponential decay limits the burstiness of ``accelerate'' signals.}
 \textbf{On each idle period with no packets:}\\
 spare\_accel $=$ 0\;
\textbf{In steady state:}\\
\For{each packet}{
    calculate $f(t)$ using Eq.~(\ref{eq:f})\;
    spare\_accel = spare\_accel $+ f(t)$\;
    \If{packet marked with accelerate}{
        \eIf{spare\_accel $>$ 1}{
            spare\_accel = spare\_accel $-$ 1\;
        }{
            mark brake\;
        }
    }
    spare\_accel *= $ e^{-\frac{now-last\_update}{\delta}}$\;
    last\_update = now;\\
    //Exponential decay.
}
\label{alg:abc}
\end{algorithm}

In this algorithm, packet marking is deterministic; it is also possible to mark probabilistically, but the results will be burstier. 

\textbf {Rate measurement timescales:} We use a moving window of time to calculate the target rate and current dequeue rate. When the access link's rate varies quickly, using a shorter time window gives better performance, but if the time window is too short, then the rate estimates might be incorrect. For cellular networks, the time window used for measurements should be at least the average inter-schedule time of a user at the router. Thus, at a base station, the time window should be greater than $\frac{N \cdot S}{M}$, where $N$ is the number of active users, $S$ is the sub-frame size ($\approx$ 1 ms for LTE), and $M$ is the number of ``resource blocks'' per sub-frame. We use a window size of 20 ms in our experiments over traces. For WiFi, in MAC 802.11n, we observe that inter-schedule for a router can go upto 20ms (~\Fig{ampdu_burst}), as a result we use a window size of 40 ms in our experiments over WiFi. 


\subsection{Multiple Bottlenecks}
\label{s:multiple-bottleneck}

So far we have described our solution for a single bottleneck, but a \name flow can encounter multiple bottlenecks on a path. For paths with multiple bottlenecks there are two possible scenarios. First, all the bottlenecks on the path are \name. Second, the path has both \name and non-\name bottlenecks.

\textbf{\name Bottlenecks:} An Example of such a scenarios is, cellular uplink and a cellular downlink in a video conference between two smartphone users. In such settings, the sender should send at the smaller of the two target rates, which implies that the final ``accelerate'' fraction received by the sender should be the minimum over the multiple \name links. The packet marking mechanism described above automatically achieves this behavior because access routers can only convert an accelerate to a brake.

\textbf{\name and Non-\name Bottlenecks:} An example is a path with a WiFi bottleneck and an ISP bottleneck router enforcing the internet plan speed in a home setting. WiFi exhibits variation in link capacity, when the link capacity drops, the WiFi router becomes the bottleneck. When the capacity increase, the ISP routers becomes the bottleneck.

In the scheme described so far, if a non-\name becomes a bottleneck, then the \name bottleneck will remain under utilized and will keep on signalling an increase to the sender. The sender will keep increasing it's rate, leadin to high loss rates the non-\name bottleneck. The problem is that \name is not reacting to congestion signals (drops or ECN) from non-\name routers. A natural solution is to modify \name to adjust its congestion window based on drops and ECN as well.

Earlier RCP~\cite{rcp}, an explicit flow control scheme proposed a heuristic to deal with non-RCP bottlenecks. If a RCP flow experiences drops or  if the RTT goes beyond twice the base RTT delay, then the flow infers presence of a non-RCP bottleneck and switches to Cubic like behaviour. This approach has a two problems. One, there is no mechanism to switch back to default RCP behaviour. Even if the non-RCP router ceases to be the bottleneck, the RCP flow will keep behaving like cubic, filling up queues unnecessarily. Second, the heuristic is not robust and a RCP flow can switch to cubic even if there are no non-RCP bottlenecks. In networks with time varying capacity, even without a non-RCP bottleneck RTTs can go beyond twice the base RTT. Moreover WiFi and other wireless networks can have non congestion drops due to low signal-to-noise ratio. 

\name's solution doesn't have these problems. A \name flow maintains two congestion windows, \name{}\_CWND and Cubic\_CWND. \name{}\_CWND evolves based on accelerate/brake feedback in ACKs as described in \Sec{abc-sender}. Cubic\_CWND evolves based on drop and ECN signal and emulates a Cubic flows congestion window. \name flows sets its own congestion window (CWND), as CWND=min(\name{}\_CWND, Cubic\_CWND). 

In case \name router is the bottleneck there will be no drops and Cubic\_CWND will be higher than \name{}\_CWND, \name flow will adjust CWND based on accelerates and brakes only, achieving low queuing delays. In case the bottleneck is a non-\name router, \name{}\_CWND will be higher than Cubic\_CWND, \name will thus behave like a cubic flow, competing fairly with other flows on the non-\name bottleneck. 

Note that in the scenario with only \name bottlenecks, Cubic\_CWND will keep on increasing. This can prove to a problem if a non-\name router becomes a bottleneck, Cubic\_CWND will be much higher than CWND and \name flow will take time to react to congestion signals from non-\name routers, causing excessive packet drops. Similarly in case of only non-\name bottlenecks \name{}\_CWND will keep on increasing, when a \name router becomes the bottleneck, \name will cause transient high queuing delays on the \name router. To prevent these, \name restricts Cubic\_CWND and \name{}\_CWND to twice the number of packets in flight.

\subsection{Fairness}
\label{s:fairness}

What happens when a \name flow shares bottleneck with other flows. We consider two scenarios. First, all competing flows are \name. Second, both \name and non-\name flows share the bottleneck.

\textbf{Coexistence with other \name flows:} Multiple \name flows sharing the same bottleneck should be able to compete fairly with each other. \name{}'s window update rule is effectively a multiplicative-increase/multiplicative-decrease (MIMD) strategy (\S\ref{s:design}), which does not provide fairness among flows contending on a link . 

We modify \name by adding a simple {\em additive-increase} (AI) component to the window update rule; where the senders increases its congestion window every 1 RTT, in addition to reacting to accelerate/brake feedback. This idea, inspired by traditional additive-increase/multiplicative-decrease (AIMD) congestion control protocols, works because \name{}'s brakes reduce the window via multiplicative-decrease during congestion. Adding an additive component thus creates an AIMD-like behavior. 

A potential drawback of this approach is that the \name{} router will receive more traffic than it anticipates. This can cause persistent queues and delay, if there are large number of flows sharing the link. Potentially, adding a penalty based on the integral of the queuing delay to the target rate calculation (similar to the PI~\cite{hollot2001designing} AQM) can solve this problem. Since, in cellular networks it is unlikely for a user to have large no of flows, we didn't investigate this solution.

\textbf{Coexistence with non-\name flows:}A \name router can have both \name and non-\name flows sharing the bottleneck. To avoid \name flows from starving, \name router stores \name and non-\name packets in separate queues. The \name router assign weights, $w_{\name}$ and 1-$w_{\name}$, to \name and non-\name queues respectively, and schedules packets in proportion to the weights. For \name queue, the target rate is calculated based on \name{}'s share of the link capacity. For non-\name{} we use a droptail buffer.

Our approach is similar to that of prior work XCP~\cite{xcp} and RCP~\cite{rcp} in the sense that both of them seperate traffic into two queues. The difference is in how we assign weights. XCP, calculates average congestion window for XCP flows using congestion window of individual XCP flows from packet headers. XCP also estimates congestion window of non-XCP flows based on drops using equation based congestion control EBCC ~\cite{ebcc}. XCP then assigns weights to match the two congestion windows. This solution cannot be generalized to \name as congestion window for \name flows is not known. Moreover, using EBCC can lead to an inaccurate estimate of congestion window for non-\name flows, this is because  EBCC relies on drops which are infrequent. Another problem is that EBCC works only if non-\name flows use the same congestion control protocol as EBCC.

RCP estimates the no of flows for each class (RCP and non-RCP) using Zombie Lists proposed in ~\cite{sred}. RCP calculates average throughput for RCP and non-RCP flows, by dividing capacity assigned to each queue and estimate of the no. of flows for that queue. RCP assigns weights so that average throughput is same for both the classes. This solution works well in case of long-lived flows, but deviates from the desired max-min fairness in presence of short flows. Consider a scenario with long lived RCP flows, and both long and short non-RCP flows. RCP will try to assign same average throughput to both the classes. Since non-RCP class has short flows, the throughput of long live non-RCP flows will be greater than the average throughput for non-RCP class. This implies long lived non-RCP flows will have throughput than long lived RCP flows, leading to unfairness. Experiment in ~\Sec{non-abc-flow} demonstrates this unfairness.

For each class (\name and  non-\name), every RTT \name router estimates the throughput of the $K$ biggest flows using a heavy hitter strategy from ~\cite{vibha}. For each class, \name router also calculates aggregated throughput of remaining flows (considered short flows) by subtracting throughput of these top $K$ flows from aggregate throughput of the class. Assuming biggest $K$ flows in each class can send at a $X\%$ higher rate in the next RTT, and that the aggregated throughput of the short flows \textbf{will} increase by $X\%$, \name calculates max-min allocation of throughput. For achieving max-min fairness, \name updates $w_{ABC}$ as ratio of max-min throughput of \name and non-\name flows. 

Note that this method can lead to some unfairness if flows are not able to increase their rate by $X\%$. In such a scenario the extra $X\%$ throughput assigned to a flow of class can cause the class to have a higher weight than its fair share. Note that the unfairness in weight for each class is bounded by $X\%$. In our experiments we use $X=10\%$, using a smaller value for $X$ can slow down convergence to fair throughput allocation.

==> design2.tex <==
\section{Design}
\label{s:design}

%\pg{In this section, we describe the design of \name and how it achieves the desired key properties (\S\ref{s:case_explicit}).} \name requires small modifications to both bottleneck routers and senders. An \name router uses link rate estimates and queuing delays to compute a target rate. The router then uses a single bit to mark each packet, echoed to the sender by the receiver in the ACK stream, to guide the senders to achieve that target rate. Each bit signals either a one packet increase (``accelerate'') or a decrease (``brake'') to the sender's congestion window. \pg{Should we say here that receiver echoes back accelerate and brake in the ACKs?}
%In the rest of this section, we will describe \name in more detail, and explain how it is able to overcome the challenges described in ~\Sec{introduction}.

\name is a window-based protocol: the sender limits the number of packets in flight to the current congestion window. Window-based protocols react faster to the sudden onset of congestion than rate-based schemes (which set a transmission rate). On a wireless link, when the capacity drops and the sender stops receiving ACKs, \name will stop sending packets immediately, avoiding further queue buildup. In contrast, a rate-based protocol would take time to reduce its rate and may queue up a large number of packets at the bottleneck link in the meantime.

\name senders adjust their window size based on explicit feedback from \name routers. An \name router uses its current estimate of the link capacity and queuing delay to compute a {\em target rate}. The router then sets one bit of feedback in each packet to guide the senders towards the target rate. Each bit is echoed to a sender by a receiver in an ACK, and it signals either a one-packet increase (``accelerate'') or a one-packet decrease (``brake'') to the sender's congestion window.

\subsection{The ABC Protocol}
We now present \name's design in the most basic case where all routers are \name-capable and all flows use \name. We later discuss how to extend the design to handle non-ABC routers and scenarios with competing non-ABC flows.

\subsubsection{ABC Sender\\}
\label{s:abc-sender}

On receiving an ``accelerate'' ACK, an \name sender increases its congestion window by 1 packet. This increase results in two packets being sent, one in response to the ACK and one due to the window size increase. On receiving a ``brake,'' the sender reduces its congestion window by 1 packet, preventing the sender from transmitting a new packet in response to the received ACK. As we discuss in \S\ref{s:fairness}, the sender also performs an additive increase of 1 packet per RTT to achieve fairness. For ease of exposition, let us ignore this additive increase for now.

Though each bit of feedback translates to a small change in the congestion window, when aggregated over an RTT, the feedback can express a large dynamic range of window size adjustments. For example, suppose a sender's window size is $w$, and the router marks accelerates on a fraction $f$ of packets in that window. Over the next RTT, the sender will receive $w \cdot f$ accelerates and $w - w \cdot f$ brakes. Then, the sender's window size one RTT later will be $w + w f - (w - w f) = 2wf$ packets. Thus, in one RTT, an ABC router can vary the sender's window size between zero ($f$ = 0) to double its current value ($f = 1$). The set of achievable window changes for the next RTT depends on the number of packets in the current window $w$; the larger $w$, the higher the granularity of control.

%reduces the window to zero, $f$ = 1/2 maintains the current window, and $f$ = 1 doubles it. 

In practice, \name senders increase or decrease their congestion window by the number of newly acknowledged bytes covered by each ACK. Byte-based congestion window modification is a standard technique in many TCP implementations~\cite{allman2003tcp}, and it makes \name robust to variable packet sizes and delayed, lost, and partial ACKs. For simplicity, we describe the design with packet-based window modifications in this paper.

%\name senders take special care to react to all ACKed packets in the event of delayed ACKs, and support byte-level congestion window modifications to support varying packet sizes. \ma{this sentence isn't clear.}


%An alternate design, can interpret accelerate-brake differently (e.g., increase/decrease window by 2 instead of 1), allowing \name to increase its rate faster than slow start. Slow start is deemed safe in the internet, anything faster might lead to excessive congestion on non-\name links. 
%Thus, using only a single-bit of feedback, an \name router can vary a sender's rate from 0 ($f$ = 0) to double ($f$ = 1) the current congestion window within a single RTT.
%Thus, values of 0, 1/2, and 1 for $f$ correspond to throttling, maintaining, or doubling the sender's current window within 1 RTT, respectively.

\subsubsection{\name Router\\}

\label{s:abc-router}
\textbf{Calculating the target rate:} %\pg{The rate control rule used by existing explicit schemes such as XCP and RCP were designed for fixed capacity links and are not well suited for time varying links.} 
\name routers compute the target rate $tr(t)$ using the following rule:
\begin{equation}
tr(t) = \eta {\mu(t)} - \frac{\mu(t)}{\delta} (x(t) - d_{t})^{+},
\label{eq:abctargetrule}
\end{equation}
where $\mu(t)$ is the link capacity, $x(t)$ is the observed queuing delay, $d_{t}$ is a pre-configured delay threshold, $\eta$ is a constant less than 1,  $\delta$ is a positive constant (in units of time), and $y^{+}$ is $\max(y,0)$. This rule has the following interpretation. When queuing delay is low ($x(t) < d_t$), \name sets the target rate to $\eta \mu(t)$, for a value of $\eta$ slightly less than 1 (e.g., $\eta = 0.95$). By setting the target rate a little lower than the link capacity, \name aims to trade a small amount of bandwidth for large reductions in delay,  similar to prior work~\cite{jain1996congestion,hull,avq}. However, queues can still develop due to rapidly changing link capacity and the 1 RTT of delay it takes for senders to achieve the target rate. \name uses the second term in Eq.~\eqref{eq:abctargetrule} to drain queues. Whenever $x(t) > d_t$, this term reduces the target rate by an amount that causes the queuing delay to decrease to $d_t$ in at most $\delta$ seconds. 

The threshold $d_t$ ensures that the target rate does not react to small increases in queuing delay. This is important because wireless links often schedule packets in batches. Queuing delay caused by batch packet scheduling does not imply congestion, even though it occurs persistently. To prevent target rate reductions due to this delay, $d_{t}$ must be configured to be greater than the average inter-scheduling time at the router.
%(e.g., WiFi 802.11n \ma{what about 802.11n?})
%\Fig{wifi} shows that reducing $d_{t}$ can hurt throughput of \name on Wi-Fi. 

\name's target rate calculation requires an estimate of the underlying link capacity, $\mu(t)$. In \Sec{linkrate}, we discuss how to estimate the link capacity in cellular and WiFi networks, and we present an implementation for WiFi.


%\name's target rate calculation requires an estimate of the underlying link capacity, $\mu(t)$. Techniques for accurately computing link capacity depend on the underlying network platform. In ~\Sec{wifi}, we present and implement a method for estimating link capacities on a Wi-Fi router, which incorporates MAC 802.11n-specific properties and assumes a single queue \pg{across users (the dominant queuing strategy on commodity routers)}. Similarly, a cellular base station implementing ABC can use information from the scheduler to control resource allocation across users. Base stations typically employ per-user queues for isolation, so target rate calculations should consider per-user link capacities and queuing delay measurements. This strategy preserves the inter-user fairness provided by the base station scheduler.\footnote{This approach also applies to Wi-Fi routers that use per-user scheduled queues.}


%For a fixed link capacity, if $x(t)>0$, then $\dot_{x}(t) \leq (1-\eta)$, this implies within a fixed amount of time the queue will go to zero and remain zero.

%Prior methods can be directly applied to identify value ranges for each parameter to ensure stability~\cite{xcp,rcp}. In our experiments, we used $\eta=0.98$, $\beta=0.75$, $\delta=100$ ms.

%\textbf{Packet marking:} Each packet begins with an accelerate marking, seeking to increase the window by the maximum allowed amount. \name routers may change any accelerate to a brake, but not vice versa. This policy ensures that an \name router can independently reduce rates to ensure that its target rate is not exceeded, but it cannot increase rates without consensus along the path, guaranteeing that no router's target rate is exceeded (assuming non-malicious routers and cooperating senders). 

\smallskip
\noindent {\bf Packet marking:} To achieve a target rate, $tr(t)$, the router computes the fraction of packets, $f(t)$, that should be marked as accelerate. Assume that the current {\em dequeue rate}\,---\,the rate at which the router transmits packets\,---\,is $cr(t)$. If the accelerate fraction is $f(t)$, for each packet that is ACKed, the sender transmits $2f(t)$ packets on average. Therefore, after 1 RTT, the {\em enqueue rate}\,---\,the rate at which packets arrive to the router\,---\,will be $2cr(t)f(t)$. To achieve the target rate, $f(t)$ must be chosen such that $2cr(t)f(t)$ is equal to $tr(t)$. Thus, $f(t)$ is given by:
\begin{equation}
f(t) = \min\Big\{\frac{1}{2} \cdot \frac{tr(t)}{cr(t)}, 1 \Big\}.
\label{eq:f}
\end{equation}
An important consequence of the above calculation is that $f(t)$ is computed based on the {\em dequeue} rate. Most explicit protocols compare the enqueue rate to the link capacity to determine the feedback (e.g., see XCP~\cite{xcp}). 
%However, it is difficult to determine the appropriate feedback based on the enqueue rate when the link capacity fluctuates significantly over time. 
\name uses the dequeue rate instead to exploit the ACK-clocking property of its window-based protocol. Specifically, Eq.~\eqref{eq:f} accounts for the fact that when the link capacity changes (and hence the dequeue rate changes), the rate at the senders changes automatically within 1 RTT. As shown in Appendix~\ref{app:deque-vs-enque}, computing $f(t)$ based on the dequeue rate at the router enables \name to track the link capacity much more accurately than using the enqueue rate. 

%Recall that if the current congestion window is $w$, then the congestion window 1 RTT later will be $2wf(t)$. This implies that if the current dequeue rate at the router is $cr(t)$, then the rate after 1 RTT will be $2cr(t)f(t)$. $f(t)$ must be chosen such that $2cr(t)f(t)$ is equal to $tr(t)$. Thus, $f(t)$ is given by:
% \abovedisplayskip
% \begin{equation}
% f(t) = \min\Big\{\frac{1}{2} \cdot \frac{tr(t)}{cr(t)}, 1 \Big\}.
% \label{eq:f}
% \end{equation}
%  \belowdisplayskip
\name recomputes $f(t)$ on every dequeued packet, using measurements of $cr(t)$ and $\mu(t)$ over a sliding time window of length $T$. Updating the feedback on every packet allows \name to react to link capacity changes more quickly than schemes that use periodic feedback updates (e.g., XCP and RCP).

%\footnote{\pg{ToDo: Say something about complexity at the router? To reduce overhead at the router this computation can be dont every 1 ms instead of every packet.}} traversal using a sliding time window. \pg{This continuous update allows \name to further reduce delays in comparison to XCP, which updates its aggregated feedback ($\phi$) once per RTT. We evaluate the impact of the periodic update on XCP in \S\ref{ss:performance}.} 

Packet marking can be done deterministically or probabilistically. To limit burstiness, \name uses the deterministic method shown in Algorithm~\ref{alg:abc}. The variable {\tt token} implements a token bucket that is incremented by $f(t)$ on each outgoing packet (up to a maximum value {\tt tokenLimit}), and decremented when a packet is marked accelerate. To mark a packet accelerate, {\tt token} must exceed 1. This simple method ensures that no more than a fraction $f(t)$ of the packets are marked accelerate. 

%Notice that the router never changes the mark for a packet that was previously marked with brake 

%. If {\tt token} is greater than 1, the packet is marked accelerate and {\tt token} is decremented; otherwise it is marked brake. This simple method ensures that no more than a fraction $f(t)$ of the packets are marked accelerate. 

\begin{algorithm}[t]
\SetAlgoLined
\caption{Packet marking at an \name{} router.}% The exponential decay limits the burstiness of ``accelerate'' signals.}
token $=$ 0\;
\For{each outgoing packet}{
    calculate $f(t)$ using Eq.~(\ref{eq:f})\;
    token = min(token $+ f(t)$, tokenLimit)\;
    \If{packet marked with accelerate}{
        \eIf{token $>$ 1}{
            token = token $-$ 1\;
            mark accelerate\;
        }{
            mark brake\;
        }
    }
}
\label{alg:abc}
\end{algorithm}

\smallskip
\noindent{\bf Multiple bottlenecks:} An \name flow may encounter multiple ABC routers on its path. An example of such a scenario is when two smartphone users communicate over an \name-compliant cellular network. Traffic sent from one user to the other will traverse a cellular uplink and cellular downlink, both of which could be the bottleneck. To support such situations, \name endhosts should send traffic at the smallest of the router-computed target rates along their path.  To achieve this goal, each packet is initially marked accelerate by the sender. \name routers may change a packet marked accelerate to a brake, but not vice versa (see Algorithm~\ref{alg:abc}). This rule guarantees that an \name router can unilaterally reduce the fraction of packets marked accelerate to ensure that its target rate is not exceeded, but it cannot increase this fraction. Hence the fraction of packets marked accelerate will equal the minimum $f(t)$ along the path. 

% \smallskip
% \noindent {\bf Comparison to XCP:} In contrast to \name, XCP's control rule doesn't include a target utilization and delay threshold term, reducing performance on wireless links. Our evaluations (\S\ref{ss:performance} show that \name outperforms XCP on emulated cellular traces. \name achieves similar average throughput as XCP, but XCP incurs 105\% higher $95^{th}$ percentile per-packet delay on average. ... talk about per-packet vs. periodic feedback updates: further reduce delays in comparison to XCP, which updates its aggregated feedback ($\phi$) once per RTT.



%In other words, ACKs received by the endhost should have an accelerate fraction that matches the minimum value of $f(t)$ for the routers on the path.

%In case a given \name router is not acting as the bottleneck, and the fraction of incoming packets marked with accelerate is lesser than $f(t)$, then the \name router can accumulate tokens. When the \name router becomes the bottleneck again, the accumulated tokens can cause a burst. To limit this burstiness, we use an exponential delay on accumulated tokens.

%The design of \name presented in ~\Sec{abc-router} achieves this property because routers can only convert accelerates to brakes. 

%\Fig{ts_multilink} shows the throughput and aggregate queuing delay for an \name{} flow traversing two different emulated cellular links, each running \name{}. At any given time, either one of the two links can be the bottleneck link. The dashed line in the Figure's top graph shows the bottleneck link rate across the two cellular links. As shown, \name{} is able to closely track the bottleneck link rate, and sends traffic just below that rate to maintain low queuing delays.
% \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.8\columnwidth,height=1.5in]{images/ts_multi_v2.pdf}
%      \vspace{-5mm}
%      \caption{\small {\bf \pg{Coexistence of multiple \name bottlenecks ---}} \name{}'s rate tracks the bottleneck closely.}
%      \label{fig:ts_multilink}
% \end{figure}


\subsubsection{Fairness\\}

Multiple \name flows sharing the same bottleneck link should be able to compete fairly with one another. However, the basic window update rule described in ~\Sec{abc-sender} effectively employs a multiplicative-increase / multiplicative-decrease (MIMD) strategy,\footnote{All the competing \name senders will observe the same accelerate fraction, $f$, on average. Therefore, each flow will update its congestion window, $w$, in a multiplicative manner, to $2fw$, in the next RTT.} which does not provide fairness among contending flows (see \Fig{fairness:no_ai} for an illustration). To achieve fairness, we add an additive-increase (AI) component to the basic window update rule. Specifically,  \name senders adjust their congestion window on each ACK as follows:
\begin{equation}
w \leftarrow 
\begin{cases}
      w + 1 + 1/w & \text{if accelerate} \\
      w - 1 + 1/w & \text{if brake}
    \end{cases}
    \label{eq:abc_cwnd_rule}
\end{equation}
This rule increases the congestion window by 1 packet each RTT, in addition to reacting to received accelerate and brake ACKs. This additive increase, coupled with \name's MIMD response, makes \name a multiplicative-and-additive-increase / multiplicative-decrease (MAIMD) scheme. Chiu and Jain~\cite{chiujain} proved that MAIMD schemes converge to fairness (see also~\cite{akella2002exploring}).

To give intuition, we provide a simple informal argument for why including additive-increase gives \name fairness. Consider $N$ \name flows sharing a link, and suppose that in steady state, the router marks a fraction $f$ of the packets accelerate, and the window size of flow $i$ is $w_i$. To be in steady state, each flow must send 1 packet on average for each ACK that it receives. Now consider flow $i$. It will send $2f+1/w_i$ packets on average for each ACK: $2f$ for the two packets it sends on an accelerate (with probability $f$), and $1/w_i$ for the extra packet it sends every $w_i$ ACKs. Therefore, to be in steady state, we must have: $2f + 1/w_i = 1 \implies w_i = 1 / (1-2f)$. This shows that the steady-state window size for all flows must be the same, since they all observe the same fraction $f$ of accelerates! Hence, with equal RTTs, the flows will have the same throughput, and otherwise their throughput will be inversely proportional to their RTT. 

\Fig{fairness:ai} shows how with an AI component, competing \name flows achieve fairness. 

%also showed that inter-flow fairness for MAIMD is similar to AIMD (e.g., Reno).

%To ensure fairness across \name flows, we modify \name by adding a simple additive-increase (AI) component to the window update rule. Specifically, \name senders increase their congestion window by 1 packet each RTT, in addition to reacting to received accelerate and brake ACKs. This additive increase, coupled with \name's multiplicative-decrease response to congestion (i.e., brakes), creates an overall additive-increase/multiplicative-decrease (AIMD) which guarantees fairness.

%It is important to note that, while this modification ensures fairness, it will increase the traffic that passes through an \name router, potentially resulting in persistent queues and delays. Though we do not expect users to have a substantial number of concurrently backlogged flows (\pg{wireless links are usually present at the edge}) to create significant queues, delays could be alleviated by having \name routers add a penalty term to their target rate calculation (Equation~\ref{eq:abctargetrule}) based on the integral of queuing delay (as done with Pi~\cite{pie}).

 %\pg{To illustrate fairness, we consider a scenario in which five \name flows are competing on a fixed 24 Mbits/s link. At the beginning of the experiment, a new \name flow is introduced every 30 seconds, and at the end of the experiment, an \name flow is terminated every 30 seconds. \Fig{fairness} show that the \name flows are able to quickly adapt to both arrivals and departures of other \name flows, achieving inter-flow fairness throughout the entire experiment. The queuing delays remain close to 0 during the entire duration of the experiment. There is a slight $\sim$5 ms increase in queuing delay between the 90--180 second experiment time frame, which includes the maximum of five concurrent \name flows. This delay can be attributed to extra packets in the network that result from the additive increase mechanism used by each of the five \name flows.


\begin{figure}
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/fairness_complicated_no_ai.pdf}
        \vspace{-7mm}
        \caption{\name w/o AI}
        \label{fig:fairness:no_ai}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/fairness_complicated_ai.pdf}
        \vspace{-7mm}
        \caption{\name with AI}
        \label{fig:fairness:ai}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf Fairness among competing \name flows ---} 5 flows with the same RTT start and depart one-by-one on a 24~Mbit/s link. The additive-increase (AI) component leads to fairness.}
    \label{fig:fairness}
    \vspace{-4mm}
\end{figure}


\subsubsection{Stability Analysis\\}
\name's stability depends on the values of $\eta$ and $\delta$. $\eta$ determines the target link utilization, while $\delta$ controls how long it will take for a queue buildup to drain. In Appendix~\ref{app:stability} we prove the following result for a fluid model of the \name control loop.
\begin{theorem}
Consider a single \name link, traversed by $N$ \name flows. Let $\tau$ be the maximum round-trip propagation delay of the flows. \name is globally asymptotically stable if
\begin{align}
    \delta > \frac{2}{3} \cdot \tau.
\end{align}
Specifically, if $\mu(t) = \mu$ for $t > t_0$ (i.e., the link capacity stops changing after some time $t_0$), the enqueue/dequeue rate and the queuing delay at the \name router will converge to certain values $r^*$ and $x^*$ that depend on the system parameters and the number of flows. In all cases: $\eta \mu < r^* \leq \mu$.
\label{thm:stablity}
\end{theorem}
This stability criterion is simple and intuitive. It states that $\delta$ should not be much smaller than the RTT (i.e, the feedback delay). If $\delta$ is very small, \name reacts too forcefully to queue build up, causing under-utilization and  oscillations.\footnote{Interestingly, if the sources do not perform additive increase or if the additive increase is sufficiently ``gentle,'' \name is stable for any value of $\delta$. See the proof in Appendix~\ref{app:stability} for details.} Increasing $\delta$ well beyond $2/3\tau$ improves the stability margins of the feedback loop, but hurts responsiveness. In our experiments, we used $\delta=133$ ms for a propagation RTT of $100$ ms. 

% \pg{The control rule is stable for all values of $\delta$, given $\eta$ is less than 1. The primary reason is that the target rate set by \name is always lesser than $\eta\mu$. Since $\eta<1$, any persistent queue will eventually drain and remain drained. Appendix ~\ref{app:stability} includes the complete proof establishing stability. The stability condition also implies that \name doesn't need to know the exact RTT for setting $\delta$ and using an incorrect estimate only impacts the rate of drain of transient queues. \name's control rule drains a standing queue within $\delta$ time, and the drain time ($\delta$) must be order of 1 RTT. If the drain time is too small ($<<$ RTT) then the link can become temporarily underutilized, if the drain time is too high ($>>$ RTT), then it might take a long time to drain the queues. In our experiments, we used $\eta=0.98$, and $\delta=133$ ms (conservative approximate for RTT).}









\subsection{Coexistence with non-\name bottlenecks}
\label{s:multiple-bottleneck}

%Our description of \name endpoints has thus far assumed only \name bottleneck routers. However, in practice, an \name flow can encounter non-\name bottleneck routers. An example of this scenario is a home Wi-Fi user whose traffic traverses the Wi-Fi router and an ISP router that enforces the corresponding Internet plan speed. Due to the link rate variance with Wi-Fi, either router can become the bottleneck: Wi-Fi link rate drops would yield the Wi-Fi router as the bottleneck, while link rate increases could make the ISP router the bottleneck.

%Based on the \name design described thus far, \name only reacts to signals from an \name router, if a non-\name router becomes a bottleneck, the \name router will remain underutilized and will thus keep signaling accelerates to the sender. This, in turn, will cause the sender to increase its rate, leading to high loss rates at the non-\name bottleneck. The inherent problem is that \name routers are not reacting to congestion signals (i.e., drops or ECN markings) which are sent from non-\name routers. Thus, a natural solution is to modify \name to react to these congestion signals as well. We discuss how an \name sender can distinguish between accelerate/brake marks and traditional congestion signals (drops of legacy ECN marking) in \S\ref{ss:deployment}.


In practice, an \name{} flow can encounter both \name and non-\name bottleneck routers. For example, a Wi-Fi user's traffic will traverse both a Wi-Fi router (running \name{}) and an ISP router (not running \name{}); either router could be the bottleneck at any given time. To handle such situations, \name flows must react to traditional congestion signals (e.g., drops or ECN marks), and they must determine when to ignore accelerate feedback from \name routers. 

%However, our description of \name{} endpoints has thus far assumed only \name{} bottleneck routers, whereby \name senders only react to signals from \name{} routers, and ignore congestion signals (e.g., drops or ECN markings) sent by non-\name{} routers. With this approach, if a non-\name{} router ever became the bottleneck, an \name{} router would remain underutilized and continually signal accelerates to the server. This, in turn, would cause the sender to increase its rate, leading to high loss rates at the non-\name{} bottleneck. Thus, to support cases with both \name{} and non-\name{} bottleneck routers, we extend \name to react to congestion signals from non-\name{} routers as well.


% There are two possible multiple bottleneck scenarios: 1) all bottlenecks on a path are \name routers, or 2) a path includes both \name and non-\name bottleneck routers. We discuss how \name handles these scenarios in turn.


%\textbf{Only-\name bottlenecks:} An example of this scenario is when two smartphone users communicate over an \name-compliant cellular network. Traffic sent from one user to the other will traverse base stations both for the cellular uplink and cellular downlink, each of which can be a bottleneck. To support such situations, \name endhosts should send traffic at the smallest of the router-computed target rates. In other words, ACKs received by the endhost should have an accelerate fraction that matches the minimum marking fraction across all bottleneck routers. 

%\pg{Each packet begins with an accelerate marking, seeking to increase the window by the maximum allowed amount. \name routers may change any accelerate to a brake, but not vice versa, as shown in Algorithm~\ref{alg:abc}. This policy ensures that an \name router can independently reduce rates to ensure that its target rate is not exceeded, but it cannot increase rates without consensus along the path, guaranteeing that no router's target rate is exceeded (assuming non-malicious routers and cooperating senders). In case a given \name router is not acting as the bottleneck, and the fraction of incoming packets marked with accelerate is lesser than $f(t)$, then the \name router can accumulate tokens. When the \name router becomes the bottleneck again, the accumulated tokens can cause a burst. To limit this burstiness, we use an exponential delay on accumulated tokens.}

%The design of \name presented in ~\Sec{abc-router} achieves this property because routers can only convert accelerates to brakes. 

%\pg{\Fig{ts_multilink} lists throughput and aggregate queuing delay value for an \name{} flow traversing two different emulated cellular links, each running \name{}. At any given time, either one of the two links can be the bottleneck link. The dashed line in the Figure's top graph shows the bottleneck link rate across the two cellular links. As shown, \name{} is able to closely track the bottleneck link rate, and sends traffic just below that rate to maintain low queuing delays.}

%\textbf{\name and non-\name bottlenecks:} 

%Based on the \name design described thus far, \name only reacts to signals from an \name router, if a non-\name router becomes a bottleneck, the \name router will remain underutilized and will thus keep signaling accelerates to the sender. This, in turn, will cause the sender to increase its rate, leading to high loss rates at the non-\name bottleneck. The inherent problem is that \name routers are not reacting to congestion signals (i.e., drops or ECN markings) which are sent from non-\name routers. Thus, a natural solution is to modify \name to react to these congestion signals as well. We discuss how an \name sender can distinguish between accelerate/brake marks and traditional congestion signals (drops of legacy ECN marking) in \S\ref{ss:deployment}.

%Prior explicit congestion control schemes have tried to incorporate congestion signals into their control loops. For example, RCP~\cite{rcp} senders infer non-RCP bottlenecks when drops are incurred or when the observed RTT grows larger than twice a base RTT value. In these scenarios, RCP switches to Cubic-like behavior. This approach has two primary problems. First, it lacks a mechanism to switch back to the default RCP behavior. As a result, the RCP router's queues will unnecessarily grow if it becomes the bottleneck again. Second, the heuristics for detecting other bottlenecks are not robust to time-varying wireless links, where RTTs can rapidly fluctuate and drops can occur due to non-congestion reasons (e.g., low signal-to-noise values).

To this end, \name senders maintain two congestion windows, one for tracking the available rate on \name routers ($w_{abc}$), and one for tracking the rate on non-\name{} routers ($w_{cubic}$). $w_{abc}$ obeys accelerates/brakes using Eq.~\eqref{eq:abc_cwnd_rule}, while $w_{cubic}$ follows Cubic's standard window update rule~\cite{cubic} and responds to drop and ECN signals.\footnote{We discuss how \name senders can distinguish between accelerate/brake and ECN marks in \S\ref{ss:deployment}.} An \name sender must send packets to match the minimum of the two available rates. Thus, \name uses min($w_{abc}$, $w_{cubic}$) as its congestion window. 
%If an \name router is the bottleneck, the sender will be limited by $w_{abc}$, and if a non-\name router is the bottleneck, the sender will follow $w_{cubic}$, competing fairly with other flows sharing the link. 
Although we chose to behave as Cubic on non-\name routers, the same technique can be used to emulate other protocols.

%We chose Cubic for fairness, as most of the cross traffic flows will be Cubic at the non-\name routers, but this technique can be generalized to non-Cubic protocols.

%\name senders maintain two congestion windows, one for ABC (\name{}$_{CWND}$) and one for non-\name{}; here, we consider Cubic cross-traffic (i.e., $w_{cubic}$), but note that this technique can be generalized to non-Cubic protocols. \name{}$_{CWND}$ evolves according to accelerates/brakes and tracks the feasible rate on \name routers, while $w_{cubic}$ follows Cubic's typical increase policy and responds to drop and ECN congestion signals, tracking feasible throughput on non-\name bottlenecks. Since either window can correspond to the bottleneck at any given time, \name senders must send packets to match the minimum of the two rates. Thus, \name sets CWND = min(\name{}$_{CWND}$, $w_{cubic}$). As a result, if an \name router is the bottleneck, the \name sender will not incur congestion-based drops and will modify its CWND based on accelerates and brakes to achieve low queuing delay. In contrast, if a non-\name router is the bottleneck, the \name sender will follow $w_{cubic}$ and compete fairly with other competing flows.

%\pg{Note that in a scenario where non-\name link is the bottleneck, the \name inks will remain underutilized and ABC$_{CWND} will continually increase; if an \name router becomes the bottleneck, the \name router will incur temporarily high queuing delays. To prevent this scenario, \name senders caps ABC$_{CWND} to twice the number of in-flight packets. This cap ensures that an \name sender won't send increase its rate more than twice per RTT (limited to slow-start) when \name router becomes the bottleneck again. Similarly, if only a \name bottleneck exists, $w_{cubic}$ will continually increase as there will be no drops to react to.}

With this approach, the window that is not the bottleneck could grow very large. For example, when a non-\name router is the bottleneck, the \name router will continually send accelerates. These accelerates do not cause the sender to transmit new packets, but they do cause $w_{abc}$ to grow. Thus if the \name router becomes the bottleneck, it will (temporarily) incur very large queues. To prevent this problem, \name senders cap both $w_{abc}$ and $w_{cubic}$ to twice the number of in-flight packets.

%With this approach, in a scenario with only \name bottlenecks, $w_{cubic}$ will continually increase as there will be no drops to react to. In the event that a non-\name router becomes the bottleneck, $w_{cubic}$ will be far larger than the CWND that the \name sender is using, resulting in excessive packet drops. Similarly, if only non-\name bottlenecks exist, \name{}$_{CWND}$ will continually increase; if an \name router becomes the bottleneck, the \name router will incur temporarily high queuing delays. To prevent both scenarios, \name senders caps all CWNDs to twice the number of in-flight packets. This cap ensures that an \name sender won't increase its rate more than twice per RTT, limiting the increase behaviour to slow-start. Anything faster might lead to excessive drops in the internet.

 \begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/abccubic_cwnd.pdf}
     \vspace{-5mm}
     \caption{\small {\bf Coexistence with non-\name bottlenecks ---} When the wired link is the bottleneck, \name becomes limited by $w_{cubic}$ and behaves like a cubic flow. When the wireless link is the bottleneck, \name uses $w_{abc}$ to achieve low delays and high utilization.}
     \label{fig:ts_droptail_cell}
     \vspace{-4mm}
\end{figure}

\Fig{ts_droptail_cell} shows the throughput and aggregate queuing delay for an \name flow traversing a path with an \name-capable wireless link and a wired link with a droptail queue. For illustration, we vary the capacity of the wireless link in a series of steps every 5 seconds. Over the experiment, the bottleneck switches between the wired and wireless links several times. \name is able to adapt its behavior both quickly and accurately. Depending on which link is the bottleneck, either $w_{cubic}$ or $w_{abc}$ becomes smaller and controls the rate of the flow. When the wireless link is the bottleneck, \name maintains low queuing delay, whereas the queuing delay exhibits standard Cubic behavior when the wired link is the bottleneck. In either case, the larger window grows to the upper limit of 2$\times$ the smaller window. Notice that $w_{cubic}$ does not limit \name's ability to increase its rate when the wireless link is the bottleneck. At these times (e.g., around the 70~s mark), as soon on $w_{abc}$ increases, the inflight packets  and the cap on $w_{cubic}$ increases, and $w_{cubic}$ rises immediately.

%\noindent \textbf{Comparison to prior schemes:} RCP~\cite{rcp} uses packet drops or high RTTs ($2\times$ a base value) to detect non-RCP links and switch to Cubic-like behavior. This approach has two drawbacks. First, it lacks a mechanism to switch back to the default RCP behavior. As a result, the RCP router's queues will unnecessarily grow if it becomes the bottleneck again. Second, the heuristics for detecting other bottlenecks are not robust to time-varying wireless links, where RTTs can rapidly fluctuate and drops can occur for non-congestion-related reasons (e.g., low signal-to-noise values). \ma{We can cut this.} 


%When the wired link becomes the bottleneck, $w_{cubic}$ reacts to packet drops and becomes smaller than $w_{abc}$. The wireless link becomes underutilized and the \name{}$_{CWND}$ keeps increasing until it becomes bounded by the upper cap (cubic like pattern in \name{}$_{CWND}$ is a result of this cap). Since \name uses the minimum of two windows, it behaves like a Cubic flow--the illustrated queuing delays mimic those expected with Cubic. In contrast, when the cellular link becomes the bottleneck, there are no drops (or legacy ECN signal) and the \name{}$_{CWND}$ becomes lower than $w_{cubic}$ (bounded by twice the number of in-flight packets). The \name sender immediately starts reacting to accelerates and brakes, tracking the fluctuation in bottleneck link capacity, reducing queuing delays while maintaining high link utilization. Note that the cap on $w_{cubic}$ doesn't limit \name's ability to increase its rate when an \name router is the bottleneck. In such a setting, as soon on \name{}$_{CWND}$ increases, the inflight packets  and the cap on $w_{cubic}$ increases, and the $w_{cubic}$ increases immediately (look at 70 s mark in \Fig{ts_droptail_cell}). %TODO: Say more on why $w_{cubic}$ increases instantly?

%\textbf{Comparison to prior schemes:} RCP~\cite{rcp} senders also infer non-RCP bottlenecks when drops are incurred or when the observed RTT grows larger than twice a base RTT value. In these scenarios, RCP switches to Cubic-like behavior. This approach has two primary problems. First, it lacks a mechanism to switch back to the default RCP behavior. As a result, the RCP router's queues will unnecessarily grow if it becomes the bottleneck again. Second, the heuristics for detecting other bottlenecks are not robust to time-varying wireless links, where RTTs can rapidly fluctuate and drops can occur due to non-congestion reasons (e.g., low signal-to-noise values).

%Prior explicit congestion control schemes have also tried to incorporate traditional congestion signals into their control loops. For example, RCP~\cite{rcp} senders infer non-RCP bottlenecks when drops are incurred or when the observed RTT grows larger than twice a base RTT value. In these scenarios, RCP switches to Cubic-like behavior. This approach has two primary problems. First, it lacks a mechanism to switch back to the default RCP behavior. As a result, the RCP router's queues will unnecessarily grow if it becomes the bottleneck again. Second, the heuristics for detecting other bottlenecks are not robust to time-varying wireless links, where RTTs can rapidly fluctuate and drops can occur due to non-congestion reasons (e.g., low signal-to-noise values).

\subsection{Coexistence with non-\name flows}
\label{s:fairness}
\name flows are potentially at a disadvantage when they share an \name bottleneck link with non-\name flows.\footnote{\name and non-\name flows may also share a non-\name  link, but in such cases, \name flows will behave like Cubic and compete fairly with other traffic (\Sec{multiple-bottleneck}).} If the non-\name flows fill up queues and increase queuing delay, the \name router will reduce \name's target rate. To ensure fairness in such scenarios, \name routers isolate \name and non-\name packets in separate queues. Using separate queues allows \name flows to achieve low delays even if the non-\name flows build up a large queue.

%We now describe how we can ensure fairness when \name and non-\name flows share an \name bottleneck router. We note that scenarios where \name and non-\name flows share a non-\name bottleneck router are also possible. However, in such cases, \name flows will behave like Cubic (\Sec{multiple-bottleneck}) and compete fairly with other traffic. 

%\pg{Note that, while cellular networks do ensure user-level fairness by scheduling users out of separate queues, the scheduling doesn't ensure inter flow fairness for a given user.}. 

%This section describes how we can ensure fairness when competing with cross-traffic. We consider two different scenarios for \name bottleneck routers: 1) all competing flows use \name, and 2) both \name and non-\name flows share the router. We note that scenarios where \name and non-\name share a non-\name bottleneck router are possible. However, in such cases, \name flows will automatically switch to behaving like Cubic (~\Sec{multiple-bottleneck}) and respond to the generated packet drops, ensuring fairness. \pg{Note that, while cellular networks do ensure user-level fairness by scheduling users out of separate queues, the scheduling doesn't ensure inter flow fairness for a given user.}. 


%\begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{images/fairness.pdf}
%     \vspace{-3mm}
%     \caption{\small \pg{{\bf Coexistence with \name flows ---}} \name flows compete fairly with each other while maintaining low aggregate queuing delays.}
%     \label{fig:fairness}
%\end{figure}

We assume that \name routers can determine whether a packet belongs to an \name flow. In some deployment scenarios, this is relatively straightforward. For example, many cellular networks deploy TCP proxies at the edge of the network~\cite{wang2011untold,ravindranath2013timecard}. In such networks, the operator can deploy \name at the proxy, and configure the base station to assume that all traffic from the proxy's IP address uses \name. Other deployment scenarios may require \name senders to set a predefined value in a packet field like the IPv6 flow label. 
%\ma{This seems to defeat the purpose of our reliance on ECN. Not sure if there's anything stronger to say}

%This could be done with by setting a predefined value in the IPv6 flow label, or it could be implicit in cellular networks that use a TCP proxy where all traffic from the proxy's IP address could be assumed to use ABC if the cellular network operator has deployed ABC. 

%\textbf{Coexistence with non-\name flows:} To ensure fairness in the scenario where \name and non-\name flows traverse an \name bottleneck router, \name routers store \name and non-\name (includes UDP traffic) packets in separate queues. \pg{Separate queues allow \name flows to achieve low delays even if the non-\name flows are filling up the queue.} Senders must signal to the router each packet that uses ABC; this could be done by setting a predefined value in the IPv6 flow label, or it could be implicit in cellular networks that use a TCP proxy where all traffic from the proxy's IP address could be assumed to use ABC if the cellular network operator has deployed ABC. 

%We consider non-\name queues to employ DropTail or CoDel, though our approach is agnostic to the queuing discipline used. 

The \name router assigns weights of $w_{\name}$ and 1-$w_{\name}$ to the \name and non-\name queues, respectively, and it schedules packets from the queues in proportion to their weights. In addition, \name's target rate calculation considers only \name's share of the link capacity (which is governed by the weights). The challenge is how to set the weights to ensure that the average throughput of long-running \name and non-\name flows is the same, irrespective of the number of flows.

Prior explicit control schemes have considered two approaches. XCP estimates the average window size of competing TCP flows based on their packet loss rate, using a TCP-Friendly-Rate-Control-like~\cite{ebcc} calculation. XCP then dynamically adjusts the weights to equalize the average window size for XCP and TCP flows. The problem with this approach is that the TFRC calculation can be inaccurate; for example, it fails to model BBR~\cite{bbr} flows. RCP estimates the number of flows in each queue using a data structure called a Zombie List~\cite{sred}, and then adapts the weights to equalize the average rate of RCP and TCP flows. This approach works well if all the flows are long-running, but it is not fair in the presence of short flows. When one queue has a large number of short flows (and hence a small average throughput), RCP increases the weight of that queue. However, the short flows cannot send faster, so the extra bandwidth is taken by long-running flows in the same queue, which get more throughput than long-running flows in the other queue. We demonstrate this unfairness experimentally in \S\ref{ss:flow_fairness}.

%problem is that instead of trying to match the throughput for backlogged (long-lived) flows, RCP is matching the average throughput for each queue. For instance, consider a scenario with long-lived RCP flows, and both long- and short-lived non-RCP flows. Since the non-RCP queue includes short flows, the throughput of long-lived non-RCP flows will be higher than the targeted average throughput for the entire non-RCP queue. Consequently, long-lived non-RCP flows will have higher throughput than long-lived RCP flows, resulting in unfairness. Section~\ref{ss:flow_fairness} compares ABC and RCP's strategy got coexistence and demonstrate this unfairness empirically.


%computes average congestion windows for XCP and non-XCP traffic; the former is computed using congestion window values in XCP packet headers, while the latter is estimated assuming equation based congestion control (EBCC)~\cite{ebcc}. XCP routers then assign queue weights to match the two congestion window values. XCP's use of EBCC to compute non-XCP congestion windows can lead to inaccurate measurements, both because drops (which EBCC relies on) are infrequent, and cross traffic does not necessarily follow an EBCC model (i.e., EBCC fails to model throughput of BBR flows).

%RCP estimates the number of flows in each queue (i.e., RCP and non-RCP) using Zombie Lists~\cite{sred}. RCP routers then computes the average aggregate throughput for the flows in each queue by dividing each queue's total capacity by the estimated number of flows in that queue. Weights are then assigned to match the queues' average throughputs. This approach works well if all flows are long-lived, but deviates from the desired max-min fairness property in the presence of short flows. \pg{The problem is that instead of trying to match the throughput for backlogged (long-lived) flows, RCP is matching the average throughput for each queue.} For instance, consider a scenario with long-lived RCP flows, and both long- and short-lived non-RCP flows. Since the non-RCP queue includes short flows, the throughput of long-lived non-RCP flows will be higher than the targeted average throughput for the entire non-RCP queue. Consequently, long-lived non-RCP flows will have higher throughput than long-lived RCP flows, resulting in unfairness. Section~\ref{ss:flow_fairness} compares ABC and RCP's strategy got coexistence and demonstrate this unfairness empirically.


To overcome these drawbacks, \name routers use a more robust strategy for assigning weights to each queue. The router measures the average rate of the $K$ largest flows in each queue.\footnote{There are many algorithms for top-$K$ rate measurement~\cite{estan2002new, sivaraman2017heavy}. Our implementation uses the Space Saving Algorithm~\cite{metwally2005efficient} which requires $\mathcal{O}(K)$ space.} It considers any remaining flow in either queue to be short, and it calculates the total rate of the short flows in each queue by subtracting the rate of the largest $K$ flows from the queue's aggregate throughput. \name uses these rate measurements to estimate the rate demands of the flows. Using these demands, \name periodically computes the max-min fair rate allocation for the flows, and it sets the weight of each queue to be equal to the total max-min rate allocation of its flows. This algorithm ensures that long-running flows in the two queues achieve the same average rate, while correctly accounting for demand-limited short flows. 

To estimate the demand of the flows, the \name router assumes two things: 1) the demand for the top $K$ flows in each queue is X\% higher than the current throughput of the flow, and 2) the aggregate demand for the short flows in each queue is same as the current aggregate throughput of the short flows. Notice that if a top-$K$ flow is unable to increase its sending rate by X\%, its queue's weight will be larger than necessary. However, any unfairness in weight assignment is bounded by X\%. Small values of $X$ limit unfairness but can slow down convergence to the fair throughput allocation; our experiments use $X=10\%$. 

%The max-min fair allocation also ensures that all UDP traffic will pass through without being limited.


%The router then computes the max-min throughput allocation and updates $w_{ABC}$ to be the ratio of the max-min throughput of \name and non-\name flows. 




%One approach for assigning weights is to calculate the throughput achieved by each flow, and then perform a max-min fair allocation to match the throughput for \name and non-\name backlogged (long-lived) flows. The problem with this approach is that it requires per-flow state. To remedy this, for each queue (i.e., \name and non-\name), the \name router estimates the average (EWMA) throughput of only the $K$ biggest flows using the Space Saving Algorithm~\cite{metwally2005efficient} which requires $\mathcal{O}(K)$ space. The \name router calculates the aggregate throughput of the remaining flows (which are considered to be short flows and include all UDP flows) by subtracting the observed throughput of the largest $K$ flows from the queues aggregate throughput.

%In case the number of backlogged flows for a given queue is much larger than $K$ (unlikely as wireless links are typically deployed at the edge), the biggest $K$ flows will serve as a representative sample for each queue. In this setting, if the current weights are inequitable, the unfairness will be reflected in the throughput of the biggest $K$ flows and our allocation strategy will readjust the weights to ultimately achieve fairness.
%This estimate is computed once per $\delta$, or the RTT normalization factor (~\Sec{abc-router}).


%o compute a throughput allocation, the \name router assumes two things: 1) the sending rate for all of the top $K$ flows in each queue \textit{can} increase by X\% in the next RTT, and 2) the aggregate throughput of the short flows in each queue \textit{will} remain same in the next RTT. The router then computes the max-min throughput allocation and updates $w_{ABC}$ to be the ratio of the max-min throughput of \name and non-\name flows. Importantly, this strategy can result in unfairness if either of the aforementioned conditions are unmet. In particular, if a flow in a given queue is unable to increase its sending rate by X\%, that queue's weight can become unfairly high. However, such unfairness in weight assignment is bounded by X\%. Smaller values of $X$ limit unfairness but can slow down convergence to the fair throughput allocation; our experiments use $X=10\%$.

\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/coexist_explanation.pdf}
     \vspace{-5mm}
     \caption{\small {\bf Coexistence with non-\name flows ---} \name flows compete fairly with non-\name flows.}
     \label{fig:coexist_explanation}
     \vspace{-4mm}
\end{figure}

\Fig{coexist_explanation} illustrates \name's fairness with non-\name flows. In this experiment, first two \name flows and then two Cubic flows arrive one after another. \name flows compete fairly with each other and with non-\name flows, and they achieve a low queuing delay despite the large Cubic queue.
% One challenge: how do we even classify ABC and non-ABC traffic?


%\textbf{Comparison to prior schemes:} Prior explicit flow control schemes have also proposed assigning competing traffic to separate queues to help with fairness. However, these approaches have several shortcomings in comparison to \name. For example, XCP~\cite{xcp} computes average congestion windows for XCP and non-XCP traffic; the former is computed using congestion window values in XCP packet headers, while the latter is estimated assuming equation based congestion control (EBCC)~\cite{ebcc}. XCP routers then assign queue weights to match the two congestion window values. XCP's use of EBCC to compute non-XCP congestion windows can lead to inaccurate measurements, both because drops (which EBCC relies on) are infrequent, and cross traffic does not necessarily follow an EBCC model (i.e., EBCC fails to model throughput of BBR flows).

%\textbf{Comparison to prior schemes:} Prior explicit flow control schemes have also proposed assigning competing traffic to separate queues to help with fairness. However, these approaches have several shortcomings. For example, XCP~\cite{xcp} computes average congestion windows for XCP and non-XCP traffic; the former is computed using congestion window values in XCP packet headers, while the latter is estimated assuming equation based congestion control (EBCC)~\cite{ebcc}. XCP routers then assign queue weights to match the two congestion window values. Unfortunately, this solution cannot be generalized to \name as \name packets do not explicitly list congestion window values. Additionally, XCP's use of EBCC to compute non-XCP congestion windows can lead to inaccurate measurements, both because drops (which EBCC relies on) are infrequent, and cross traffic does not necessarily follow an EBCC model (i.e., XCP assumes a throughput-versus-loss-rate function of $1/\sqrt{p}$ which means that it cannot correctly support a scheme like Cubic, or a mix of different competing protocols).

%RCP estimates the number of flows in each queue (i.e., RCP and non-RCP) using Zombie Lists~\cite{sred}. RCP routers then computes the average aggregate throughput for the flows in each queue by dividing each queue's total capacity by the estimated number of flows in that queue. Weights are then assigned to match the queues' average throughputs. This approach works well if all flows are long-lived, but deviates from the desired max-min fairness property in the presence of short flows. \pg{The problem is that instead of trying to match the throughput for backlogged (long-lived) flows, RCP is matching the average throughput for each queue.} For instance, consider a scenario with long-lived RCP flows, and both long- and short-lived non-RCP flows. Since the non-RCP queue includes short flows, the throughput of long-lived non-RCP flows will be higher than the targeted average throughput for the entire non-RCP queue. Consequently, long-lived non-RCP flows will have higher throughput than long-lived RCP flows, resulting in unfairness. Section~\ref{ss:flow_fairness} compares ABC and RCP's strategy got coexistence and demonstrate this unfairness empirically.

\cut{

\subsection{Practical Deployment with ECN}
\label{ss:deployment}

In this section, we describe how ECN~\cite{ecn-rfc} can be repurposed to signal accel-brake marks. The \name sender must be able to distinguish accel-brake marks from \name routers and congestion signals (drops and legacy ECN markings) from non-\name routers (\S\ref{s:multiple-bottleneck}). Our deployment solution requires simple modifications to TCP receivers. We start with an overview of standard ECN, and then present our practical deployment solution. 

\textbf{ECN Overview:} IP packets have two ECN-related bits: ECT and CE. These two bits are traditionally interpreted as follows:
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & ECN-Capable Transport ECT(1)\\
 1 & 0 & ECN-Capable Transport ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
Routers interpret both (01) and (10) to indicate that a connection is ECN capable, and routers change those bits to (11) to mark a packet with ECN. Upon receiving an ECN mark (11), a receiver sets the {\em ECN Echo (ECE)} flag in {\em all} subsequent ACKs until it receives a {\em Congestion Window Reduced (CWR)} notification from the sender, \ie a packet with the CWR flag in the TCP header set to 1. Thus receivers echo ECN marks for a full round-trip worth of ACKs.

%Upon receiving an ECN mark (11), a receiver sets the {\em ECN Echo (ECE)} flag in {\em all} subsequent ACKs until it receives a {\em Congestion Window Reduced (CWR)} notification from the sender, \ie a packet with the CWR flag in the TCP header set to 1. Thus receivers echo ECN marks for a full round-trip worth of ACKs.


\textbf{Deployment:} \name can coexist with non-\name  routers (using ECN for signalling congestion) by reinterpreting the ECT and CE ECN bits as follow:
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & \textit{accelerate} ECT(1)\\
 1 & 0 & \textit{brake} ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
\name senders can mark accelerates using (01), and \name routers can signal brakes by flipping the bits to (10). Both (01) and (10) equivalently indicate ECN capable transport to legacy routers, which can continue to use (11) to signal congestion.

With this design, receivers must be able to convey both standard ECN signals and accelerates/brakes for \name. ECN feedback can be signaled using the ECE flag. For \name feedback, we repurpose the NS (nonce sum) bit, which was originally proposed to ensure ECN feedback integrity~\cite{nonce} but has been reclassified as historic~\cite{accurate-ecn} due to lack of deployment.


\textbf{Deployment in Cellular Networks:} Cellular networks commonly split TCP connections and deploy proxy at the edge~\cite{wang2011untold,ravindranath2013timecard}. In such a network, it is unlikely that any non-\name router will act as the bottleneck and interfere with the accel-brake markings from the \name router. In this case where non-\name routers do not use ECN, deploying \name is relatively straightforward and doesn't require any receiver modifications. \name senders can simply use either (01) or (10) ECN markings to signal an accelerate, and routers can use (11) to indicate a brake. However, a challenge with such deployment is that ECN receivers, by default, will echo an ECN bit in all ACKs in an RTT (i.e., until they receive a CWR from the sender). An \name sender that responds to all marked ACKs will incorrectly be throttled. To ensure that the receiver conveys accelerate/brake signals accurately, the sender sets the CWR flag on {\em every} packet. This ensures that the receiver echoes a brake exactly once (instead of for a full RTT). The proxy can be modified to run custom \name senders, and the base station can be modified to act as a \name router.

We note that any internal encryption used by cellular network providers does not hinder a \name{} router's ability to modify ECN bits. The reason is that the \name{} router is typically positioned in a place where any form of in-network encryption is removed (e.g., at an LTE eNodeB).

\textbf{Security:} It is possible for a malicious router to convert a brake to an accelerate, causing congestion at other routers on the path. However, an \name sender can easily detect this by periodically transmitting packets that are marked with brake; if any of these packets return with accelerate, there exist malicious entities on the path.
}

\if 0

\subsection{Practical Deployment with ECN}
\label{ss:deployment}

\pg{In this section, we describe two potential deployment options for \name that build upon re purposing ECN~\cite{ecn-rfc} to signal accel-brake marks. The \name sender must be able to distinguish accel-brake marks from \name routers and congestion signals (drops or legacy ECN markings) from non-\name routers (\S\ref{s:multiple-bottleneck}).} First, we discuss how \name can be deployed on \pg{paths with non-\name bottleneck routers} which do not use ECN to signal congestion, but instead rely on packet drops; we refer to these routers as ``no legacy ECN routers.'' In this case, \name can be deployed without any modifications to TCP receivers, though sender transport stacks must be modified to use \name for uploading traffic. \pg{This scenario is common in cellular networks, which split TCP connections and deploy proxy at the edge~\cite{wang2011untold,ravindranath2013timecard}. In such an environment, the proxy can be modified to run \name senders, and the base station can be modified to marks packets. In such a network, it is unlikely that any non-\name router will act as the bottleneck, interfering with the accel-brake markings from the base station.}. Second, we present a way to deploy \name in scenarios where \pg{non-\name bottleneck routers} already use ECN to signal congestion (i.e., ``legacy ECN routers''). In this scenario, our deployment solution requires simple modifications to TCP receivers. We start with an overview of standard ECN, and then present our practical deployment solutions in more detail. 

\textbf{ECN Overview:} IP packets have two ECN-related bits: ECT and CE. These two bits are traditionally interpreted as follows:
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & ECN-Capable Transport ECT(1)\\
 1 & 0 & ECN-Capable Transport ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
Routers interpret both (01) and (10) to indicate that a connection is ECN capable, and routers change those bits to (11) to mark a packet with ECN. Upon receiving an ECN mark (11), a receiver sets the {\em ECN Echo (ECE)} flag in {\em all} subsequent ACKs until it receives a {\em Congestion Window Reduced (CWR)} notification from the sender, \ie a packet with the CWR flag in the TCP header set to 1. Thus receivers echo ECN marks for a full round-trip worth of ACKs.

We note that any internal encryption used by cellular network providers does not hinder a \name{} router's ability to modify ECN bits. The reason is that the \name{} router is typically positioned in a place where any form of in-network encryption is removed (e.g., at an LTE eNodeB).

\textbf{Deployment with no legacy ECN routers:} In the case where non-\name routers do not use ECN to signal congestion, deploying \name is relatively straightforward. \name senders can simply use either (01) or (10) ECN markings to signal an accelerate, and routers can use (11) to indicate a brake. However, a challenge with such deployment is that ECN receivers, by default, will echo an ECN bit in all ACKs in an RTT (i.e., until they receive a CWR from the sender). An \name sender that responds to all marked ACKs will incorrectly be throttled. We present and evaluate two solutions for overcoming this, one with receiver modifications and one without. Both solutions ensure that receivers only echo each ECN mark once, in a single ACK. We implemented both solutions in Linux as a kernel module using the pluggable TCP API.
% add something about TCP proxies in cell networks

\textit{With receiver modification:} Using the pluggable TCP API, we modified the receiver such that it simply echoes back an ECN bit once and doesn't wait for a CWR from the sender. This receiver behaviour is identical to that of DCTCP~\cite{dctcp}. We use this version of TCP in all of the experiments in this paper.

\textit{Without receiver modification:} To ensure that the receiver conveys accelerate/brake signals accurately, we modified the kernel such that the sender sets the CWR flag on {\em every} packet. This ensures that the receiver echoes a brake exactly once (instead of for a full RTT).

% I dont think we need to say this
%, assuming all packets are acknowledged and ACKs are not lost. \name can also leverage proposed ECN feedback mechanisms that are more accurate in the presence of delayed or lost ACKs~\cite{accurate-ecn}.

Appendix~\ref{app:cwr} compares the throughput and $95^{th}\%$ile per-packet delay of the two TCP variants using a backlogged iperf flow running on eight different emulated cellular network traces. Our results show that both TCP variants achieve similar throughput and delay (within 1\% of each other) averaged across the traces.

\textbf{Deployment with legacy ECN routers:} In the case where non-\name routers use ECN to signal congestion, \name can coexist with legacy ECN routers by reinterpreting the ECT and CE ECN bits as follow:
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & \textit{accelerate} ECT(1)\\
 1 & 0 & \textit{brake} ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
\name senders can mark accelerates using (01), and \name routers can signal brakes by flipping the bits to (10). Both (01) and (10) equivalently indicate ECN capable transport to legacy routers, which can continue to use (11) to signal congestion.

With this design, receivers must be able to convey both standard ECN signals and accelerates/brakes for \name. ECN feedback can be signaled using the ECE flag. For \name feedback, we can repurpose the NS (nonce sum) bit, which was originally proposed to ensure ECN feedback integrity~\cite{nonce} but has been reclassified as historic~\cite{accurate-ecn} due to lack of deployment.

\pg{Note that, \name{} routers do not interfere with the proper operation of ECN for standard TCP flows as they classify \name and non-\name flows into separate queues. The non-\name queue uses ECN as specified in the standard~\cite{ecn-rfc}.} It is possible for a malicious router to convert a brake to an accelerate, causing congestion at other routers on the path. However, an \name sender can easily detect this by periodically transmitting packets that are marked with brake; if any of these packets return with accelerate, there exist malicious entities on the path. 

\fi 
%\name{} routers do not interfere with the proper operation of ECN for standard TCP flows. All TCP implementations transmit packets with ECT/CE set to (10)  to indicate ECN-capable transport. Since \name{} only converts accelerates (01) to brakes (10), it will ignore any packet marked with (10). It is possible for a malicious router to convert a brake to an accelerate. However, senders can easily detect this by periodically transmitting packets that are marked with brake; if any of these packets return with accelerate, there exist malicious entities on the path. 

%As a result, there is no need for senders to convey \name{} capability in packet headers.

==> eval-trace.tex <==
\subsection{Does \name Achieve Low Delays\\and High Throughput?}
\label{s:abc-throughput-delay}

\begin{figure*}[tbh]
    \centering
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/single_downlink.pdf}
        \caption{Downlink}
        \label{fig:througput-delay:down}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/single_uplink.pdf}
        \caption{Uplink}
        \label{fig:througput-delay:up}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/weinstein_multi.pdf}
        \caption{Uplink+Downlink}
        \label{fig:througput-delay:up+down}
    \end{subfigure}
    \caption{\small {\bf ABC vs. previous schemes on three Verizon cellular network traces ---} In each case, ABC outperforms all other schemes and sits well outside the Pareto frontier of previous schemes. }
    \label{fig:througput-delay}
\end{figure*}

\begin{figure}[tbh]
     \centering
     \begin{subfigure}[tbh]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/new_aggregate_utilization.png}
    \subcaption{Utilization}
    \end{subfigure}
    \begin{subfigure}[tbh]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/new_aggregate_mean_delay.png}
    \subcaption{Mean per-packet delay}
    \end{subfigure}
    \caption{\small {\bf Utilization and mean per-packet delay across 8 different cellular network traces ---} On average, \name achieves 38\% more utilization than Copa and Cubic+Codel for similar delays. BBR, PCC and Cubic achieve slithtly higher throughput than \name, but incur significantly higher packet delays.}
    \label{fig:aggregate-statistics}
 \end{figure}


We evaluate throughput and delay benefits of \name{} by emulating real cellular link traces using Mahimahi, a network emulation tool~\cite{mahimahi}. We compare \name to end-to-end protocols for cellular networks, Sprout~\cite{sprout} and Verus~\cite{verus}; AQM schemes, Cubic+Codel~\cite{codelID} and Cubic+PIE~\cite{pie}; delay sensitive end-to-end protocols, BBR~\cite{bbr}, Copa~\cite{copa}, PCC Vivace-Latency~\cite{vivace} and Vegas~\cite{vegas}; and the default protocol in linux, Cubic~\cite{cubic}.

For \name{}, BBR, Cubic, PCC Vivace-Latency and Vegas, we used the TCP kernel-module. For Copa, Sprout and Verus, we used author's UDP implementation. For schemes with TCP kernel-module we used iperf~\cite{iperf} to create a backlogged flow, for other schemes we used application provided by authors. We used existing implementation of Cubic and Pie in Mahimahi. \name uses $\eta=0.98, \beta=0.75, \delta=100$ms and $d_{t}=50$ms. In our experiments, one way propagation delay was 50 ms and buffer size was 250 packets. Note that the reverse path (receiver to sender) is also emulating a cellular link trace. Until specified otherwise, we use the same setup in all following experiments in this paper.

Figure~\ref{fig:througput-delay:down} and ~\ref{fig:througput-delay:up} show utilization and 95$^{th}$ percentile per packet delay achieved by a single backlogged flow on two cellular link traces. \name exhibits a better throughput/delay trade off than all previous schemes. The dashed line in each figure shows the ``Pareto frontier'' for previous approaches; each scheme on this frontier achieves higher throughput or lower delay than the others. ABC sits well outside the best previous Pareto frontier.

Cubic+Codel, Cubic+PIE, Copa and Sprout achieve low delays (comparable to \name) but heavily under utilize the link. These schemes lack a way to infer the degree of under-utilization of the bottleneck link, when the cellular link capacity opens up, these schemes fail to utilize the network. In contrast, BBR, Cubic and PCC achieve high utilization by filling up buffers, causing ``bufferbloat''.

Figure~\ref{fig:aggregate-statistics} summarizes Utilization and mean per-packet delay across 8 different cellular traces from 3 major cellular network providers, ATT, TMobile and Verizon. \name achieves both higher throughput and lower delay compared to Sprout, Vegas and Verus. \name achieves 38\% more throughput than Cubic+Codel and Copa, with only 13\% higher mean per-packet delay. While BBR, PCC and Cubic achieve slightly higher utilization than \name{} (BBR 9\%, PCC 12\%, Cubic 18\%), they incur significantly higher delays (BBR 75\%, PCC 240\%, Cubic 232\%). Appendix~\ref{app:abc-throughput-delay} shows 95$^{th}$ percentile per-packet-delay on these traces. The trend is similar to that of mean delay.

\textbf{Perfect Knowledge} In this experiment we consider a variant of \name, PK-\name that knows the entire trace in advance. Instead of using the current link rate, PK-\name uses the link rate at time 1 propagation delay from current time to calculate target rate. Compared to \name, PK-\name reduces the queuing delay from 97ms to only 28ms on a link with 100ms propagation delay, while achieving same utilization (90\%). In cellular networks, predicting resource allocation in near future can allow \name to further reduce queuing delays.

 \textbf{WiFi Evaluation}
 %\label{s:wifi-eval}
 
 We evaluate performance of \name on a WiFi link in single user and multiple user scenario. We compare \name against a number of end-to-end scheme BBR, Cubic, PCC Vivace-latency and Vegas; and an AQM scheme, Cubic+Codel. We evaluate \name at three delay threshold ($d_{t}$) values, 20ms, 60ms and 100ms. A moving receiver (e.g., mobile phone) can create variations in signal-to-noise ratio, leading to changes in bit rate of users. To emulate effect of movement in a reproducible manner, we change the bit rate at the router by varying the MCS index using the iw utility in linux. In our experiment, we vary the MCS index between 2 values, 1 and 7, every 4 seconds. Figure ~\ref{fig:wifi} shows throughput and average RTT of these schemes, measured using the trace route utility. For 2 user scenario, we report the sum of throughput achieved by two users, and the average of average RTT observed by them. To reduce variation from devices contending for the channel, we report average values across 3, 30 second runs.
 
 In both the scenarios, \name outperforms all other schemes, achieving better throughput/delay tradeoff. \name is outside the pareto frontier forme by previous schemes. In the single user scenario, increasing delay threshold increases both throughput and RTT. Compared to Cubic+Codel and Vegas, \name{}\_100 ($d_{t}=100$ms) achieves upto 32\% higher throughput for similar RTTs. Compared to \name{}\_100, Cubic and BBR achieve slightly higher throughput (~4\%), but have singnificantly higher average RTTs (40\%). PCC achieves the highest throughput, but has 3X the average RTT compared to other schemes.
 
 In the 2 user scenario, all the variants of \name achieve similar throughput and RTT. Compared to Cubic+Codel and Vegas, \name achieves 43\% and 32\% throughput respectively, \name's RTT is 25\% higher than that of Cubic+Codel and Vegas. BBR achieves 5\% more throughput than \name, has 65\% higher average RTT than \name.
 
 \begin{figure}[tbh]
     \centering
     \begin{subfigure}[tbh]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/wifi_single.pdf}
    \subcaption{Single User}
    \label{fig:wifi:single}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/wifi_multiple.pdf}
    \subcaption{Two Users}
    \label{fig:wifi:multiple}
    \end{subfigure}
    \caption{\small {\bf Throughout and average RTT on WiFi ---} For 2 user scenario, we report the sum of throughput achieved by 2 users, and average of averahe RTT of the two users. \name outperforms all other schemes and sits outside the pareto frontier.}
    \label{fig:wifi}
 \end{figure}
 
 In Appendix~\ref{fig:app:wifi_brownian}, we consider a variant of the above experiment for the single user scenario. We model the changes in MCS index as a brownian motion. Our results in Figure~\ref{fig:app:wifi_brownian} are similar to the experiment above.

\subsection{Can Multiple \name Bottlenecks Coexist?}
\label{s:multi-bottleneck}

Figure~\ref{fig:ts_multilink} shows throughput and queuing delay of a \name{} flow traversing two cellular links running \name{}. At any given time, one of the two links is the bottleneck. The dashed line in top graphs shows bottleneck link rate of the two cellular links. \name{} tracks the bottleneck closely, sending traffic just below the bottleneck link capacity to maintain low queuing delays.

Figure~\ref{fig:througput-delay:up+down} shows throughput and delay of various schemes on a path with two cellular links. \name{} achieves better throughput/delay tradeoff and sits well outside the pareto frontier of previous schemes.

\begin{figure}[tbh]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/ts_multi.pdf}
     \caption{\small {\bf Coexistence of multiple \name bottlenecks ---} \name{}'s rate tracks the bottleneck closely.}
     \label{fig:ts_multilink}
\end{figure}


\subsection{Can \name Bottlenecks Coexist With Non-\name Bottlenecks?}
\label{s:non-abc-bottleneck}

Figure~\ref{fig:ts_droptail_cell} shows throughput and queuing delay of a \name flow on a path with a cellular and a wired link (4 Mbit/sec). The cellular link is running \name and the wired link has a droptail buffer. When the droptail link is the bottleneck, \name behaves like a Cubic flow. The queuing delays in this case, exhibit the characteristics Cubic shape. When the cellular link becomes the bottleneck, \name starts reacting to accelerates/brakes, reducing the queuing delay while maintaining high link utilization.

 \begin{figure}[tbh]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/abccubic.pdf}
     \caption{\small {\bf Coexistence with non-\name bottlenecks ---} \name behaves like Cubic when wired link becomes the bottleneck.}
     \label{fig:ts_droptail_cell}
\end{figure}


 \subsection{Can \name Flows Coexist With Each Other?}
 \label{s:fairness}
 
 In this experiment we consider 5 \name{} flows competing on a 24 Mbit/sec link. In the first half of the experiment a new \name{} is added every 30 seconds. In the remaining half, 1 \name{} flow leaves every 30 seconds. Figure~\ref{fig:fairness} shows throughput and queuing delay for the \name flows. We observe that \name flows quickly adapt to both arrival and departure of flows, achieving inter-flow fairness throughout the entire duration. The queuing delays remain close to 0 during the entire duration of the experiment. There is a slight increase in queuing delay, when the no of flows increase (90-180 ms). This increase can be attributed to the extra packets sent by flows for additive increase in \name{}.
 
\begin{figure}[tbh]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/fairness.pdf}
     \caption{\small {\bf Fairness ---} \name flows compete fairly with each other while maintaining low queuing delays. When cellular link become the bottleneck \name sender adjusts window based on accelerate/brake signals achieving close to 0 queuing delays.}
     \label{fig:fairness}
\end{figure}


\subsection{Can \name Flows Coexist With Non-\name Flows?}
\label{s:non-abc-flow}

We now evaluate coexistence of \name and non-\name flows on a \name router. We create 3 \name and 3 cubic flows sharing the same bottleneck link. Besides long lived flows, we also create non-\name short flows sharing the bottleneck link. We vary the load of short flows and compare \name and RCP's Zombie list based coexistence strategy. Figure~\ref{fig:non-abc-flow} shows the mean and standard deviation of throughput achieved by \name and Cubic flows across 10 runs each lasting 40 seconds.

Figure~\ref{fig:non-abc-flow:abc} shows \name{}'s strategy allows \name and Cubic flows to coexist fairly across all load values. The difference in average throughput between \name and cubic flows is within 1 standard deviation of each other. 
%This unfairness is because \name assigns $X=10\%$ additional throughput to non-\name short flows, non-\name class this has higher weight than its fair share. Note that the weights are within $X\%$ of max-min fair allocation (~\Sec{fairness}).

In contrast, RCP's strategy gives more preference to non-\name flows (~\Fig{non-abc-flow:rcp}), the disparity in throughput increases with load of short flows. This is because long lived non-\name flows have higher throughput than average throughput of non-\name flows calculated by RCP, and RCP tries to match the average throughput in each class leading to unfairness as discussed in ~\Sec{fairness}. 

In both the scenarios, compared to Cubic, \name on average has 50\% smaller standard deviation. This implies that \name flows compete more fairly with each other than Cubic.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/coexist_ABC.pdf}
        \caption{ABC}
        \label{fig:non-abc-flow:abc}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/coexist_RCP.pdf}
        \caption{RCP's Zombie List}
        \label{fig:non-abc-flow:rcp}
    \end{subfigure}
    \caption{\small{\bf Coexistence with non-\name flows ---} Compared to RCP's Zombie List strategy, \name's max-min allocation provides better fairness between \name and non-\name flows. In \name, the average throughput of flows in the two categories in within 1 standard deviation of each other.}
    \label{fig:non-abc-flow}
\end{figure}


\subsection{How Does \name Perform In Presence Of Application Limited Flows?}
\label{s:traffic-char}

In this experiment, we evaluate the impact of application limited flows on performance. We create 1 long lived flow along with 200 application limited flows sending traffic at 1 Mbit/sec in aggregate. Figure~\ref{fig:traffic-char} shows aggregate throughput and queuing delay achieved by \name flows on a cellular link. While the application limited flows don't react to feedback, the long lived flow does, achieving low queuing delays and high link utilization.

\begin{figure}
    \centering
        \includegraphics[width=0.8\columnwidth]{images/short_flow.pdf}
    \caption{\small{\bf \name's robustness to flow size ---} In aggregate \name achieves high utilization and low queuing delays in presence of applicated limited flows.}
    \label{fig:traffic-char}
\end{figure}

\subsection{How does \name Compare Against Explicit Flow Control Schemes?}
\label{s:explicit}

We evaluate \name against two explicit flow control schemes, RCP~\cite{rcp} and XCP~\cite{xcp}; and a ECN based scheme, VCP~\cite{vcp}. For RCP we use $\alpha=0.5$ and $\beta=0.25$, as specified by the authors. For XCP we use $\alpha=0.55$, $\beta=0.4$, the highest permissible stable values for fastest convergence to link rate. For VCP we use the default parameter values in the original paper. Figure~\ref{fig:explicit} shows utilization and mean per packet delay achieved by these schemes on 8 cellular traces. 

\name's achieves similar throughput and delay as XCP without using multibit per packet feedback. Compared to RCP, \name achieves 20\% more utilization. RCP is a rate based protocol as a result its slower in reacting to congestion when link rate drops. In such a situation, compared to window based protocols, \name and XCP, RCP experiences congestion longer and over reduces its rate, causing under utilization. Appendix~\ref{app:explicit} demonstrates this behaviour via a simple experiment.

\name also outperforms VCP, a previous scheme with succinct feedback to signal multiplicative increase or decrease. Unlike \name, VCP can only signal a fixed multiplicative increase (1.0625) and decrease (0.875). As a result \name achieves 20\% higher throughput than VCP, while incurring only a 10\% increase in 95th percentile per packet delay. 
 
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/explicit_utilization.png}
        \caption{Utilization}
        \label{fig:explicit:utilization}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/explicit_delay.png}
        \caption{Delay}
        \label{fig:explicit:delay}
    \end{subfigure}
    \caption{\small{\bf \name vs explicit flow control ---} \name achieves the same utilization and mean delay as XCP across all traces. Compared to RCP and VCP, \name achieves 20\% more utilization.}
    \label{fig:explicit}
\end{figure}


\subsection{Does \name Improve Performance Of\\Applications?}
\label{s:application}

\subsection{Does \name Perform Well Across Network Conditions?}
\label{s:network-condition}
In this experiment we test the impact of propagation delay on performance, we use the same setup used in ~\Fig{aggregate-statistics}. Figure~\ref{fig:rtt} shows utilization and mean queuing delay on a cellular trace across a number of propagation delays (referred to as RTT in the figure). For all schemes, increasing propagation delay increases utilization and reduces queuing delay. For all the propagation delay values, \name outperforms all other schemes, achieving a better throughput latency trade-off on average similar to ~\Fig{aggregate-statistics}.

For Cubic+Codel and Cubic+PIE, reducing the propagation delay reduce the bandwidth delay product, increasing the additive increase of Cubic. As result, compared to other schemes, Cubic+Codel and Cubic+PIE see a greater improvement in utilization with reduction in propagation delay. Sprout exhibits this behaviour as well.


\begin{figure}[tbh]
     \centering
     \begin{subfigure}[tbh]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/rtt_utilization.png}
    \subcaption{Utilization}
    \end{subfigure}
    \begin{subfigure}[tbh]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/rtt_delay.png}
    \subcaption{Mean per-packet queuing delay}
    \end{subfigure}
    \caption{\small {\bf Impact of propagation delay on performance ---} On a cellular trace \name outperforms all other schemes across all propagation delay values.}
    \label{fig:rtt}
 \end{figure}




==> evaluation.tex <==
\section{Evaluation}
\label{s:eval}

In this section, we evaluate \name using both our Wi-Fi implementation and trace-driven emulation of cellular networks. We evaluate the following metrics:
\begin{CompactEnumerate}
\item \textbf{Performance:} We measure \name's ability to achieve low delay and high throughput and compare \name to end-to-end schemes, AQM schemes, and explicit control     schemes (\S\ref{ss:performance}).
\item \textbf{Multiple Bottlenecks:} We test \name in scenarios with multiple \name bottlenecks and mixtures of \name and non-\name bottlenecks (\S\ref{ss:coexistence}).
\item \textbf{Coexistence:} We evaluate \name's fairness mechanisms both in competition with other \name flows and with non-\name flows (\S\ref{ss:flow_fairness}).
\item \textbf{Additional Considerations:} We evaluate how \name performs with application-limited flows and different network delays. We conclude with a demonstration of \name's impact on a real application's performance (\S\ref{ss:other_results}).
\end{CompactEnumerate}


\subsection{Experimental Setup}
\label{ss:setup}

Experiments performed over a live Wi-Fi network used the \name router described in Section~\ref{s:wifi}. We also evaluated \name using  Mahimahi~\cite{mahimahi} emulating multiple cellular networks (Verizon LTE, AT\&T, and TMobile) using packet delivery traces that were captured directly on those networks. We used separate traces to emulate the cellular uplinks and downlinks. We note that these traces include outages, highlighting \name's ability to handle ACK losses.

We compare \name to end-to-end protocols designed for cellular networks (Sprout~\cite{sprout} and Verus~\cite{verus}), loss-based end-to-end protocols both with and without AQM (Cubic protocol~\cite{cubic}, Cubic+Codel~\cite{codel}, and Cubic+PIE~\cite{pie}), recently-proposed end-to-end protocols (BBR~\cite{bbr}, Copa~\cite{copa}, PCC Vivace-Latency aka PCC)~\cite{vivace}), TCP Vegas~\cite{vegas}), and explicit control protocols (XCP~\cite{xcp} and RCP~\cite{rcp}). We used TCP kernel modules to evaluate \name, BBR, Cubic, PCC, and Vegas; for these schemes, we generated traffic by using iperf~\cite{iperf} to create a backlogged flow. For the schemes that are not implemented as a TCP kernel module (Copa, Sprout, Verus), we used the UDP implementations and traffic generation applications provided by the protocol authors. We used Mahimahi's support of Cubic and Pie to evaluate AQM. \name's target rate calculation (Equation~\ref{eq:abctargetrule}) used $\eta=0.98$, $\beta=2$, and $\delta=133$ ms. Unless otherwise noted, our emulated cellular  experiments used a minimum RTT of 100 ms and a buffer size of 250 packets.

\subsection{Performance: \name achieves low delay, high throughput, and outperforms existing schemes}
\label{ss:performance}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/single_downlink_v2.pdf}
        \vspace{-5mm}
        \caption{Downlink}
        \label{fig:througput-delay:down}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/single_uplink_v2.pdf}
        \vspace{-5mm}
        \caption{Uplink}
        \label{fig:througput-delay:up}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/weinstein_multi_v2.pdf}
        \vspace{-5mm}
        \caption{Uplink+Downlink}
        \label{fig:througput-delay:up+down}
    \end{subfigure}
    \caption{\small {\bf ABC vs. previous schemes on three Verizon cellular network traces ---} In each case, ABC outperforms all other schemes and sits well outside the Pareto frontier of previous schemes (denoted by the dashed lines). }
    \label{fig:througput-delay}
\end{figure*}

\begin{figure}[tbh]
     \centering
     \begin{subfigure}[tbh]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/new_aggregate_utilization.pdf}
    \vspace{-7mm}
    \subcaption{Utilization}
    \label{fig:aggregate-statistics:utilization}
    \end{subfigure}
    \begin{subfigure}[tbh]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/new_aggregate_mean_delay.pdf}
    \vspace{-7mm}
    \subcaption{Mean per-packet delay}
    \label{fig:aggregate-statistics:delay}
    \end{subfigure}
    \caption{\small {\bf Utilization and mean per-packet delay across 8 different cellular network traces ---} On average, \name achieves similar delays and 38\% higher utilization than Copa and Cubic+Codel. BBR, PCC, and Cubic achieve slightly higher throughput than \name, but incur 70-240\% higher mean per-packet delays.}
    \label{fig:aggregate-statistics}
 \end{figure}

Figures~\ref{fig:througput-delay:down} and~\ref{fig:througput-delay:up} show the utilization and 95$^{th}$ percentile per packet delay that a single backlogged flow achieves using each aforementioned congestion control protocol on two Verizon LTE cellular link traces. As shown, \name exhibits a better (i.e., higher) throughput/delay tradeoff than all prior schemes. In particular, \name sits well outside the Pareto frontier of the existing schemes, which houses the prior schemes that achieve higher throughput or lower delay than any other prior schemes.

Further analysis of Figures~\ref{fig:througput-delay:down} and~\ref{fig:througput-delay:up} reveals that Cubic+Codel, Cubic+PIE, Copa, and Sprout are all able to achieve low delays (comparable to \name). However, these schemes heavily underutilize the link. The reason is that, though these schemes are able to infer queue buildups and can react to them to reduce delays, they lack a way of quickly inferring increases in link capacity (a common occurrence on time-varying wireless links), leading to underutilization. In contrast, schemes like BBR, Cubic, and PCC are able to rapidly saturate the network (achieving high utilization), but these schemes also quickly fill buffers and thus suffer from high queuing delays. Unlike prior schemes, \name is able to quickly react to \textit{both} increases and decreases in available link capacity, enabling high throughput and low delays.

We observed similar trends across a larger set of 8 different cellular network traces. Figure~\ref{fig:aggregate-statistics} summarizes the link utilization and mean per-packet delays for each scheme across these scenarios. As shown, \name is able to achieve high throughput and lower delay than Sprout, Vegas, and Verus. \name also achieves 38\% higher throughput than Cubic+Codel and Copa, while only incurring 13\% higher mean per-packet delays. Finally, though BBR, PCC, and Cubic achieve slightly higher link utilization values than \name (9\%, 12\%, and 18\%, respectively), they each incur significantly higher per-packet delays than \name (75\%, 240\%, and 232\%, respectively). Appendix~\ref{app:abc-throughput-delay} compares these schemes on 95$^{th}$ percentile per-packet delay over the same conditions, and shows the same trends.

 \begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/wifi_single.pdf}
    \vspace{-7mm}
    \subcaption{Single user}
    \label{fig:wifi:single}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/wifi_multiple.pdf}
    \vspace{-7mm}
    \subcaption{Two users, shared queue}
    \label{fig:wifi:multiple}
    \end{subfigure}
    \caption{\small {\bf Throughout and mean delay on Wi-Fi ---} For the multi-user scenario, we report the sum of achieved throughputs and the average observed delay across both users. We consider three versions of \name (denoted \name\_*) for different delay thresholds. All versions of \name outperform all prior schemes and sit outside the pareto frontier.}
    \label{fig:wifi}
 \end{figure}

We performed similar evaluations on a live Wi-Fi link, considering both single and multi-user scenarios. In this experiment, we only considered schemes which include a TCP kernel module. To mimic common Wi-Fi usage scenarios where endpoints can move to create variations in signal-to-noise ratios (and thus bitrates), we varied the Wi-Fi router's bitrate selections by varying the MCS index using the Linux \texttt{iw} utility; we alternated the MCS index between values of 1 and 7 every 4 seconds. In Appendix~\ref{fig:app:wifi_brownian}, we also list results for an experiment where we model MCS index variations as Brownian motion--results show the same trends as described below. The experiment was performed in a crowded computer lab. Thus, to reduce variations from channel contention, we report average performance values across three, 45 second runs. We considered three different \name delay threshold ($d_{t}$) values of 20 ms, 60 ms, and 100 ms; increasing \name's delay threshold will increase both observed throughput and RTT values.

Figure~\ref{fig:wifi} shows throughput and mean per packet delay for each considered protocol, as measured using the \texttt{tcptrace} Linux utility. For the multi-user scenario, we report the sum of achieved throughputs and the average observed mean delay across both users. As shown, in both the single and multi-user scenarios, \name achieves a better throughput/delay tradeoff than all prior schemes, and falls well outside the Pareto frontier for those schemes. For example, in the single user scenario, the \name configuration with $d_{t}=100$ ms achieves up to 32\% higher throughput than Cubic+Codel and Vegas. Though Cubic and BBR achieve slightly higher throughput (4\%) than this \name configuration, their average RTT values are considerably higher (40\%). The multi-user scenario showed similar results. For instance, \name achieves 43\% and 32\% higher average throughput than Cubic+Codel and Vegas, respectively, though \name's average RTT values are 25\% higher. BBR achieves 5\% higher throughput than \name, but also incurs 65\% higher average RTT values.

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/explicit_utilization.pdf}
        \caption{Utilization}
        \label{fig:explicit:utilization}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/explicit_delay.pdf}
        \caption{Delay}
        \label{fig:explicit:delay}
    \end{subfigure}
    \caption{\small{\bf \name vs explicit flow control ---} \name achieves similar utilization and mean delay as XCP across all traces. Compared to RCP and VCP, \name achieves 20\% more utilization.}
    \label{fig:explicit}
\end{figure}


\textbf{Comparing \name with existing explicit flow control schemes:} We evaluate \name against two traditional explicit flow control schemes, XCP~\cite{xcp} and RCP~\cite{rcp}, as well as another in-network signaling scheme, VCP~\cite{vcp} which uses succinct feedback to only signal  a fixed multiplicative/additive increase or multiplicative decrease. We implemented each scheme as a Mahimahi qdisc~\cite{mahimahi}.

For XCP, we used constant values of $\alpha=0.55$ and $\beta=0.4$, which the authors note are the highest permissible stable values that achieve the fastest possible link rate convergence. We initially began using an unedited version of XCP in our experiments. However, we quickly observed that this version of XCP (XCP\_Original) performed significantly worse than \name, achieving far higher delay (Figure~\ref{fig:xcp} in Appendix~\ref{app:xcp} presents this comparison). The reason is that XCP computes aggregate feedback values ($\phi$) once per RTT, which it uses to calculate per-packet feedback. In scenarios where link capacity suddenly drops, it may take XCP a complete RTT before it recomputes the aggregate feedback to reduce the window. To improve XCP's performance, we modified XCP\_Original to recompute aggregate feedback \textit{on each packet} based on the rate and delay measurements from the past RTT; we refer to this version as XCP throughout the paper. This modification improves reactivity and helps control delays in the presence of rapid drops in link rate. We discuss and evaluate other potential modifications of XCP in Appendix~\ref{app:xcp}. For RCP and VCP, we used the author-specified parameter values of $\alpha=0.5$ and $\beta=0.25$, and $\alpha=1$, $\beta=0.875$ and $\kappa=0.25$, respectively. 

Figure~\ref{fig:explicit} shows utilizations and mean per packet delays achieved by each of these schemes over eight different cellular link traces. As shown, \name is able to achieve similar throughput and mean delay to the best performing explicit flow control scheme, XCP, without using multibit per-packet feedback. We note that XCP's 95$^{th}$ percentile per-packet delays are 40\% higher than \name's (Appendix~\ref{app:xcp}).
\name is also able to outperform RCP and VCP. Specifically, \name achieves 20\% higher utilization than RCP. This improvement stems from the fact that RCP is a rate based protocol (not a window based protocol)---by signaling rates, RCP is slower to react to link rate fluctuations (Appendix~\ref{app:explicit} illustrates this behavior). \name also achieves 20\% higher throughput than VCP, while incurring only a 10\% higher mean per-packet-delay.

\subsection{Coexistence with Various Bottlenecks: \name is able to properly coexist with different combinations of \name and non-\name bottlenecks}
\label{ss:coexistence}

\if 0
\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/ts_multi.pdf}
     \caption{\small {\bf Coexistence of multiple \name bottlenecks ---} \name{}'s rate tracks the bottleneck closely.}
     \label{fig:ts_multilink}
\end{figure}
\fi
\textbf{Coexistence with \name bottlenecks:} 
\pg{Figure~\ref{fig:througput-delay:up+down}, evaluates \name and prior protocols on a network path with two cellular links. In this scenario, \name{} tracks the bottleneck link rate and achieves a better throughput/delay tradeoff than prior schemes, and again sits well outside the Pareto frontier for those schemes.}
\if 0
Figure~\ref{fig:ts_multilink} lists throughput and queuing delay values for an \name{} flow traversing two different emulated cellular links, each running \name{}. At any given time, either one of the two links can be the bottleneck link. The dashed line in the Figure's top graph shows the bottleneck link rate across the two cellular links. As shown, \name{} is able to closely track the bottleneck link rate, and sends traffic just below that rate to maintain low queuing delays. This behavior is also highlighted in Figure~\ref{fig:througput-delay:up+down}, which evaluates \name and prior protocols on a network path with two cellular links. In this scenario, \name{} achieves a better throughput/delay tradeoff than prior schemes, and again sits well outside the Pareto frontier for those schemes.
 \begin{figure}[tbh]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/abccubic.pdf}
     \vspace{-3mm}
     \caption{\small {\bf Coexistence with non-\name bottlenecks ---} \name behaves like Cubic when the wired link is the bottleneck. When the cellular link is the bottleneck, \name follows accelerates and brakes to achieve low delays and high utilization.}
     \label{fig:ts_droptail_cell}
\end{figure}
\fi


\textbf{Coexistence with non-\name bottlenecks:} 
 
 \begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/abccubic_visualization_v3.pdf}
     \vspace{-3mm}
     \caption{\small \pg{{\bf Coexistence with non-\name bottlenecks ---}} \name tracks the ideal rate closely (fairshare) and reduces queuing delays in absence of cross traffic (white region). }
     \label{fig:ts_droptail_cell_visualization}
\end{figure}

\pg{Figure~\ref{fig:ts_droptail_cell_visualization} lists throughput and queuing delay values for an \name flow traversing a network path with an emulated wireless link and an emulated 12 Mbits/s fixed rate (wired) link. The wireless link is configured to run \name, while the wired link operates a droptail buffer. On-off cubic cross traffic shares the wired link with \name. In the absence of cross traffic (white region), the wireless link is the bottleneck. In the presence of cross traffic (yellow and grey regions), due to contention, the wired link can become the bottleneck. In this case, the fairshare of \name flow on the wired link is half the capacity of the wired link (6 Mbit/s). If the wireless link rate is lesser than the fairshare (yellow region), then the wireless link is the bottleneck. Otherwise (grey region), the wired link is the bottleneck. }

\pg{The black dashed line in the top graph represents ideal throughput for \name flow. When the wireless link is the bottleneck (white and yellow regions), the ideal rate for \name is the wireless link rate. When the wired link is the bottleneck (grey region), the ideal rate is the fairshare rate of 6 Mbit/s. In all the regions, \name tracks the ideal rate closely. In the absence of any cross traffic (white region), \name achieves low delays while maintaining high link utilization. In the yellow region, \name tracks the wireless link rate, the increase in queuing delays is due to congestion cause by cubic flow on the wired link. When the wired link is the bottleneck (grey region), \name behaves like Cubic and is able to achieve its fairshare of rate. }

\subsection{Coexistence: \name competes fairly with both \name flows and non-\name flows}
\label{ss:flow_fairness}

\if 0
\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/fairness.pdf}
     \vspace{-3mm}
     \caption{\small pg{{\bf Coexistence with non-\name flows ---}} \name flows compete fairly with each other while maintaining low aggregate queuing delays.}
     \label{fig:fairness}
\end{figure}
\fi

\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/jain.pdf}
     \vspace{-3mm}
     \caption{\small \pg{\bf Fairness ---} Jain Index captures fairness for competing flows. Ideal Jain Index is 1. \name and Cubic's Jain Index is close to 1 in all the cases. BBR's fairness decreases with increase in the number of flows.}
     \label{fig:jain}
\end{figure}

\pg{\textbf{Coexistence among \name flows:} To illustrate intra-flow fairness for different protocols (\name, Cubic and BBR), we simultaneously run multiple flows of the same protocol. We use a fixed 24 Mbits/s bottleneck link and the duration of each run is 60s. \Fig{jain} lists Jain Fairness Index ~\cite{jain1999throughput} for different number of competing flows. Jain Index for \name and Cubic remains close to the ideal value of 1 in all cases. The additive increase in \name ensures fairness among \name flows. In contrast, BBR's jain index decreases with increase in flows.}

%\textbf{Coexistence among \name flows:} We consider a scenario in which five \name flows are competing on a fixed 24 Mbits/s link. At the beginning of the experiment, a new \name flow is introduced every 30 seconds, and at the end of the experiment, an \name flow is terminated every 30 seconds. Figure~\ref{fig:fairness} illustrates that the \name flows are able to quickly adapt to both arrivals and departures of other \name flows, achieving inter-flow fairness throughout the entire experiment. The queuing delays remain close to 0 during the entire duration of the experiment. There is a slight $\sim$5 ms increase in queuing delay between the 90--180 second experiment time frame, which includes the maximum of five concurrent \name flows. This delay can be attributed to extra packets in the network that result from the additive increase mechanism used by each of the five \name flows.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/coexist_ABC.pdf}
        \vspace{-6mm}
        \caption{ABC}
        \label{fig:non-abc-flow:abc}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/coexist_RCP.pdf}
        \vspace{-6mm}
        \caption{RCP's Zombie List}
        \label{fig:non-abc-flow:rcp}
    \end{subfigure}
    \caption{\small{\bf Coexistence with non-\name flows ---} Across all scenarios, the standard deviation for \name flows is small and the flows are fair to each other. Compared to RCP's Zombie List strategy, \name's max-min allocation provides better fairness between \name and non-\name flows. With \name's strategy, the difference in average throughput of \name and Cubic flows is under 5\%.}
    \label{fig:non-abc-flow}
\end{figure}

\textbf{Coexistence with non-\name flows:} We consider a scenario where three \name and three non-\name (in this case, Cubic) long-lived flows share the same bottleneck link. In addition, we create varying numbers of short flows (each of size 10 KB) with flow arrival times generated by a Poisson process to offer fixed average loads. We consider several different total offered load values. Our results summarize 10 runs, each of 40 seconds. To evaluate \name's ability to fairly coexist with non-\name flows, we compare \name's coexistence strategy with RPC's Zombie list approach (\S\ref{s:fairness}). Figure~\ref{fig:non-abc-flow} shows the mean and standard deviation throughput values achieved by the \name and Cubic flows. As shown in Figure~\ref{fig:non-abc-flow:abc}, \name's coexistence strategy allows \name and Cubic flows to fairly share the bottleneck link across all offered load values. Specifically, the difference in average throughput between the \name and Cubic flows is under 5\%. In contrast, Figure~\ref{fig:non-abc-flow:rcp} shows that RCP's coexistence strategy gives higher priority to Cubic flows. This discrepancy increases as the offered load increases, with Cubic flows achieving 17-165\% higher throughput than \name flows. The reason, as discussed in ~\Sec{fairness}, is that long-lived Cubic flows receive higher throughput than the average throughput that RCP intends for Cubic flows. This triggers unfairness because RCP attempts to match average throughput values for each scheme. \pg{Moreover, ~\ref{fig:non-abc-flow} also shows that the standard deviation of \name flows is small (under 10\%) across all scenarios. A small standard deviation implies that in each run of the experiment, throughput of the three concurrent \name flow is close to each other and \name flows are fair to each other. The standard deviation for \name is smaller than Cubic, thus, \name flows converge to fairness faster than Cubic flows.}

\if 0
\textbf{Coexistence with non-\name flows:} To evaluate \name's ability to fairly coexist with non-\name flows, we compare \name's coexistence strategy with RPC's Zombie list approach (\S\ref{s:fairness}). We consider a scenario where three \name and three non-\name (in this case, Cubic) long-lived flows share the same bottleneck link. In addition, we create varying numbers of short flows (each of size 10 KB) with flow arrival times generated by a Poisson process to offer fixed average loads. We consider several different total offered load values. Our results summarize 10 runs, each of 40 seconds. Figure~\ref{fig:non-abc-flow} shows the mean and standard deviation throughput values achieved by the \name and Cubic flows. As shown in Figure~\ref{fig:non-abc-flow:abc}, \name's coexistence strategy allows \name and Cubic flows to fairly share the bottleneck link across all offered load values. Specifically, the difference in average throughput between the \name and Cubic flows is under 5\%. In contrast, Figure~\ref{fig:non-abc-flow:rcp} shows that RCP's coexistence strategy gives higher priority to Cubic flows. This discrepancy increases as the offered load increases, with Cubic flows achieving 17-165\% higher throughput than \name flows. The reason, as discussed in ~\Sec{fairness}, is that long-lived Cubic flows receive higher throughput than the average throughput that RCP intends for Cubic flows. This triggers unfairness because RCP attempts to match average throughput values for each scheme.
\fi

\subsection{Additional Results: \name improves real applications, and its benefits persist across different workloads and network latencies}
\label{ss:other_results}


\begin{figure}
    \centering
        \includegraphics[width=0.8\columnwidth]{images/short_flow.pdf}
        \vspace{-3mm}
    \caption{\small{\bf \name's robustness to flow size ---} With a single backlogged \name flow and multiple concurrent application-limited \name flows, all flows achieve high utilization and low queuing delays.}
    \label{fig:traffic-char}
\end{figure}

\textbf{Application-limited flows:} We created a single long-lived \name flow that shared a cellular link with 200 application-limited \name flows that send traffic at an aggregate of 1 Mbit/s. Figure~\ref{fig:traffic-char} shows that, despite the fact that the application-limited flows do not have traffic to properly respond to \name's feedback, the \name flows (in aggregate) are still able to achieve low queuing delays and high link utilization.

\begin{figure}[t]
     \centering
     \begin{subfigure}[t]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/rtt_utilization_v2.pdf}
    \vspace{-5mm}
    \subcaption{Utilization}
    \end{subfigure}
    \begin{subfigure}[t]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/rtt_delay_v2.pdf} \vspace{-5mm}
    \subcaption{ per-packet queuing delay}
    \end{subfigure}
    \caption{\small {\bf Impact of propagation delay on performance ---} On a Verizon cellular network trace with different propagation delays, \name achieves a better throughput/delay tradeoff than all other schemes.}
    \label{fig:rtt}
 \end{figure}

\textbf{\name's sensitivity to network latency:} Thus far, our emulation experiments have considered fixed minimum RTT values of 100 ms. To evaluate the impact that propagation delay has on \name's performance, we used a modified version of the experimental setup from Figure~\ref{fig:aggregate-statistics}. In particular, we consider RTT values of 20 ms, 50 ms, 100 ms, and 200 ms. Figure~\ref{fig:rtt} shows that, across all propagation delays, \name is still able to outperform all prior schemes, again achieving a more desirable throughput/latency trade off. \name's benefits persist even though schemes like Cubic+Codel and Cubic+PIE actually improve with increasing propagation delays. Performance with these schemes improves because bandwidth delay products increase, making Cubic's additive increase more aggressive (thereby improving link utilization).

\textbf{\name's improvement on real applications:} We evaluated \name's ability to improve performance for real user-facing applications by considering a multiplayer interactive game, Slither.io~\cite{slither}. We loaded Slither.io using a Google Chrome browser which ran inside an emulated cellular link with a background backlogged flow (generated with iperf). We considered three different congestion control protocols for the backlogged flow: Cubic, Cubic+Codel, and \name. As expected, Cubic is able to fully utilize the link, but adds excessive queuing delays which hinder gameplay. In contrast, Cubic+Codel reduces queuing delays (improving user experience in the game), but underutilizes the link. Only \name is able to achieve both high link utilization for the backlogged flow and low queuing delays for the game. A video demo of this experiment can be viewed at \url{https://youtu.be/Dauq-tfJmyU}.

\textbf{Perfect future capacity knowledge:} We considered a variant of \name, PK-\name, which knows an entire emulated link trace in advance. This experiment reflects the possibility of resource allocation predictions at cellular network base stations. Rather than using an estimate of the current link rate to compute a target rate (as \name does), PK-\name uses the exact link rate that is expected 1 RTT value in the future. Using the same setup as in Figure~\ref{fig:througput-delay:up}, PK-\name is able to reduce 95$^{th}$ percentile per-packet-delays from 97 ms to 28 ms, compared to \name, while achieving the same link utilization (\sim90\%).

==> evaluation_new.tex <==
\section{Evaluation}
\label{s:eval}

We evaluate \name using both our concrete Wi-Fi implementation (\S\ref{s:prototype implementation}) and trace-driven emulation of cellular networks. Our evaluation considers the following properties of \name:
\begin{CompactEnumerate}
\item \textbf{Performance:} We measure \name's ability to achieve low delay and high throughput and compare \name to end-to-end schemes, AQM schemes, and explicit control     schemes (\S\ref{ss:performance}). \rn{better label than performance?}
\item \textbf{Multiple Bottlenecks:} We test \name in scenarios with multiple \name bottlenecks and mixtures of \name and non-\name bottlenecks (\S\ref{ss:coexistence}).
\item \textbf{Coexistence:} We evaluate \name's fairness mechanisms both in competition with other \name flows and with non-\name flows (\S\ref{ss:flow_fairness}).
\item \textbf{Additional Considerations:} We evaluate how \name performs with application-limited flows and different network delays. We conclude with a demonstration of \name's impact on a real application's performance (\S\ref{ss:other_results}).
\end{CompactEnumerate}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/single_downlink_v3.pdf}
        \vspace{-7mm}
        \caption{Downlink}
        \label{fig:througput-delay:down}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/single_uplink_v3.pdf}
        \vspace{-7mm}
        \caption{Uplink}
        \label{fig:througput-delay:up}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/weinstein_multi_v3.pdf}
        \vspace{-7mm}
        \caption{Uplink+Downlink}
        \label{fig:througput-delay:up+down}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf ABC vs. previous schemes on three Verizon cellular network traces ---} In each case, ABC outperforms all other schemes and sits well outside the Pareto frontier of previous schemes (denoted by the dashed lines). }
    \label{fig:througput-delay}
    \vspace{-4mm}
\end{figure*}



\subsection{Experimental Setup}
\label{ss:setup}

We evaluated \name in both Wi-Fi and cellular network settings. For Wi-Fi, experiments were run over a live Wi-Fi network and used the \name router described in Section~\ref{s:prototype implementation}. For cellular settings, we use Mahimahi~\cite{mahimahi} to emulate multiple cellular networks (Verizon LTE, AT\&T, and TMobile). Mahimahi's emulation uses packet delivery traces (separate for uplink and downlink) that were captured directly on those networks, and thus include outages (highlighting \name's ability to handle ACK losses).


%Experiments performed over a live Wi-Fi network used the \name router described in Section~\ref{s:prototype implementation}. We also use Mahimahi~\cite{mahimahi} to evaluate \name over multiple emulated cellular networks (Verizon LTE, AT\&T, and TMobile). Mahimahi's emulation uses packet delivery traces that were captured directly on those networks. We used separate traces to emulate the cellular uplinks and downlinks. We note that these traces include outages, highlighting \name's ability to handle ACK losses.

We compare \name to end-to-end protocols designed for cellular networks (Sprout~\cite{sprout} and Verus~\cite{verus}), loss-based end-to-end protocols both with and without AQM (Cubic~\cite{cubic}, Cubic+Codel~\cite{codel}, and Cubic+PIE~\cite{pie}), recently-proposed end-to-end protocols (BBR~\cite{bbr}, Copa~\cite{copa}, PCC Vivace-Latency (which we refer to as PCC))~\cite{vivace}), and TCP Vegas~\cite{vegas}), and explicit control protocols (XCP~\cite{xcp}, RCP~\cite{rcp} and VCP~\cite{VCP}). We used TCP kernel modules to evaluate \name, BBR, Cubic, PCC, and Vegas; for these schemes, we generated traffic by using iperf~\cite{iperf} to create a backlogged flow. For the end-to-end schemes that are not implemented as TCP kernel modules (i.e., Copa, Sprout, Verus), we used the UDP implementations and traffic generation applications provided by the protocol authors. Lastly, for the explicit control protocols (i.e., XCP, RCP, and VCP), we used our own implementations as qdiscs with Mahimahi to ensure compatibility with our emulation setup. We used Mahimahi's support of Cubic and Pie to evaluate AQM.


%We compare \name to end-to-end protocols designed for cellular networks (Sprout~\cite{sprout} and Verus~\cite{verus}), loss-based end-to-end protocols both with and without AQM (Cubic~\cite{cubic}, Cubic+Codel~\cite{codel}, and Cubic+PIE~\cite{pie}), recently-proposed end-to-end protocols (BBR~\cite{bbr}, Copa~\cite{copa}, PCC Vivace-Latency (i.e., PCC))~\cite{vivace}), and TCP Vegas~\cite{vegas}), and explicit control protocols (XCP~\cite{xcp}, RCP~\cite{rcp} and VCP~\cite{VCP}). We used TCP kernel modules to evaluate \name, BBR, Cubic, PCC, and Vegas; for these schemes, we generated traffic by using iperf~\cite{iperf} to create a backlogged flow. For the schemes that are not implemented as TCP kernel modules (i.e., Copa, Sprout, Verus), we used the UDP implementations and traffic generation applications provided by the protocol authors. \pg{For evaluation over traces, we used our own implementation of XCP, RCP and VCP (implemented as a qdisc in mahimahi)}. We used Mahimahi's support of Cubic and Pie to evaluate AQM.

Unless otherwise noted, our emulated cellular network experiments used a minimum RTT of 100 ms and a buffer size of 250 MTU-sized packets. Additionally, in all experiments, \name's target rate calculation (Equation~\ref{eq:abctargetrule}) used $\eta=0.98$ and $\delta=133$ ms. Our Wi-Fi implementation uses the link rate estimation described in \S\ref{s:linkrate}, while our emulated cellular network setup assumes the realistic scenario that \name's router has knowledge of the underlying link capacity~\cite{3GPP}.

\subsection{Performance: \name achieves low delay, high throughput, and outperforms existing schemes}
\label{ss:performance}


\begin{figure}[t]
     \centering
     \begin{subfigure}[tbh]{\columnwidth}
     %\includegraphics[width=1.0\columnwidth]{images/wifi_single_v2.pdf}
     \includegraphics[width=1.0\columnwidth]{images/new_aggregare_utilization_v2.pdf}
    \vspace{-7mm}
    \subcaption{Utilization}
    \label{fig:aggregate-statistics:utilization}
    \end{subfigure}
    \vspace{-1mm}
    \begin{subfigure}[tbh]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/new_aggregare_95delay_v2.pdf}
    \vspace{-6mm}
    \subcaption{$95^{th}$ percentile per-packet delay}
    \label{fig:aggregate-statistics:delay}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small {\bf 95$^{th}$ percentile per-packet delay across 8 cellular link traces ---} On average, ABC achieves similar  delays  and  38\%  higher  utilization  than  Copa  and Cubic+Codel.  BBR,  PCC,  and  Cubic  achieve  slightly  higher throughput   than   ABC,   but   incur 180-400\% higher  95$^{th}$ percentile  delay than \name.}
    \label{fig:aggregate-statistics}
    \vspace{-4mm}
 \end{figure}
 
\Fig{througput-delay:down} and~\ref{fig:througput-delay:up} show the utilization and 95$^{th}$ percentile per packet delay that a single backlogged flow achieves using each aforementioned congestion control protocol on two Verizon LTE cellular link traces. As shown, \name exhibits a better (i.e., higher) throughput/delay tradeoff than all prior schemes. In particular, \name sits well outside the Pareto frontier of the existing schemes, which represents the prior schemes that achieve higher throughput or lower delay than any other prior schemes.

Further analysis of \Fig{througput-delay:down}~and~\ref{fig:througput-delay:up} reveals that Cubic+Codel, Cubic+PIE, Copa, and Sprout are all able to achieve low delays that are comparable to \name. However, these schemes heavily underutilize the link. The reason is that, though these schemes are able to infer and react to queue buildups in a way that reduces delays, they lack a way of quickly inferring increases in link capacity (a common occurrence on time-varying wireless links), leading to underutilization. In contrast, schemes like BBR, Cubic, and PCC are able to rapidly saturate the network (achieving high utilization), but these schemes also quickly fill buffers and thus suffer from high queuing delays. Unlike these prior schemes, \name is able to quickly react to \textit{both} increases and decreases in available link capacity, enabling high throughput and low delays.

We observed similar trends across a larger set of 8 different cellular network traces (\Fig{aggregate-statistics}). \name is able to achieve higher throughput and lower delay than Sprout, Vegas, and Verus. \name also achieves 38\% higher throughput than Cubic+Codel and Copa, while only incurring 17\% higher $95^{th}$ percentile per-packet delays. Finally, though BBR, PCC, and Cubic achieve slightly higher link utilization values than \name (9\%, 12\%, and 18\%, respectively), they each incur significantly higher per-packet delays than \name (183\%, 394\%, and 382\%, respectively). Appendix~\ref{app:abc-throughput-delay} compares these schemes on mean per-packet delay over the same conditions, and shows the same trends.

\textbf{Comparison with Explicit Protocols:} \Fig{througput-delay} and~\ref{fig:aggregate-statistics} also show that \name outperforms the explicit control protocol, XCP, despite not using multi-bit per-packet feedback as XCP does. In these experiments, XCP used constant values of $\alpha=0.55$ and $\beta=0.4$, which the authors note are the highest permissible stable values that achieve the fastest possible link rate convergence. XCP achieves similar average throughput to \name, but with 105\% higher 95$^{th}$ percentile delays. This performance discrepancy can be attributed to the fact that \name's control rule is better suited for the link rate variations in wireless networks. In particular, unlike \name which updates its feedback on every packet, XCP computes aggregate feedback values ($\phi$) only once per RTT and may thus take an entire RTT to inform a sender to reduce its window. To overcome this, we also considered an improved version of XCP that recomputes aggregate feedback on each packet based on the rate and delay measurements from the past RTT; we refer to this version as XCP$_{w}$ (short for XCP wireless). As shown in \Fig{througput-delay} and~\ref{fig:aggregate-statistics}, XCP$_{w}$ reduces delay compared to XCP, but still incurs 40\% higher 95$^{th}$ percentile delays than \name.
 We also compared with two other explicit schemes, RCP and VCP, and found that \name consistently outperformed both (Appendix~\ref{app:explicit}). 


%\textbf{Comparison with Explicit Protocols:} \pg{For XCP, we used constant values of $\alpha=0.55$ and $\beta=0.4$, which the authors note are the highest permissible stable values that achieve the fastest possible link rate convergence. \name outperform XCP without using multi bit per-packet feedback. XCP achieves similar average throughput as \name but incurs 105\% higher delays. The performance difference can be attributed to the fact that \name's control rule is designed for variations in wireless links. Moreover, unlike \name which updates its feedback every packet, XCP computes aggregate feedback values ($\phi$) only once per RTT, which it uses to calculate per-packet feedback. In scenarios where link capacity suddenly drops, it may take XCP a complete RTT before it recomputes the aggregate feedback to reduce the window. To improve XCP's performance, we modified XCP to recompute aggregate feedback \textit{on each packet} based on the rate and delay measurements from the past RTT; we refer to this version as XCP$_{w}$ (short for XCP Wireless). This modification helps reduce delays, but the average 95\%ile per-packet delay is still 40\% higher than \name (\Fig{aggregate-statistics}). We also compared \name against two other explicit congestion control schemes , RCP and VCP.  \name outperforms both RCP and VCP, Appendix~\ref{app:explicit} summarizes their performance over 8 different cellular traces.}

 \begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/wifi_single_v2.pdf}
    \vspace{-7mm}
    \subcaption{Single user}
    \label{fig:wifi:single}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/wifi_multiple_v3.pdf}
    \vspace{-7mm}
    \subcaption{Two users, shared queue}
    \label{fig:wifi:multiple}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf Throughout and mean delay on Wi-Fi ---} For the multi-user scenario, we report the sum of achieved throughputs and the average of observed $95^{th}$ percentile delay across both users. We consider three versions of \name (denoted \name\_*) for different delay thresholds. All versions of \name outperform all prior schemes and sit outside the pareto frontier.}
    \label{fig:wifi}
    \vspace{-4mm}
 \end{figure}

\textbf{Wi-Fi:} We performed similar evaluations on a live Wi-Fi link, considering both single and multi-user scenarios. In this experiment, we excluded Verus and Sprout as they are designed specifically for cellular networks. \cut{schemes which include a TCP kernel module. \pg{For Copa, we used an experimental implementation over CCP~\cite{ccp-sigcomm18}.}} To mimic common Wi-Fi usage scenarios where endpoints can move and create variations in signal-to-noise ratios (and thus bitrates), we varied the Wi-Fi router's bitrate selections by varying the MCS index using the Linux \texttt{iw} utility; we alternated the MCS index between values of 1 and 7 every 2 seconds. In Appendix~\ref{fig:app:wifi_brownian}, we also list results for an experiment where we model MCS index variations as Brownian motion---results show the same trends as described below. This experiment was performed in a crowded computer lab. Thus, to reduce variations from channel contention, we report average performance values across three, 45 second runs. We considered three different \name delay threshold ($d_{t}$) values of 20 ms, 60 ms, and 100 ms; note that increasing \name's delay threshold will increase both observed throughput and RTT values.

%We performed similar evaluations on a live Wi-Fi link, considering both single and multi-user scenarios. In this experiment, we only considered schemes which include a TCP kernel module. \pg{For Copa, we used an experimental implementation over CCP~\cite{ccp-sigcomm18}.} To mimic common Wi-Fi usage scenarios where endpoints can move to create variations in signal-to-noise ratios (and thus bitrates), we varied the Wi-Fi router's bitrate selections by varying the MCS index using the Linux \texttt{iw} utility; we alternated the MCS index between values of 1 and 7 \pg{every 2} seconds. In Appendix~\ref{fig:app:wifi_brownian}, we also list results for an experiment where we model MCS index variations as Brownian motion--results show the same trends as described below. The experiment was performed in a crowded computer lab. Thus, to reduce variations from channel contention, we report average performance values across three, 45 second runs. We considered three different \name delay threshold ($d_{t}$) values of 20 ms, 60 ms, and 100 ms; increasing \name's delay threshold will increase both observed throughput and RTT values.

\Fig{wifi} shows the throughput and $95^{th}$ percentile per-packet delay for each considered protocol, as measured using the \texttt{tcptrace} Linux utility. For the multi-user scenario, we report the sum of achieved throughputs and the average observed $95^{th}$ percentile across all users. As shown, in both the single and multi-user scenarios, \name achieves a better throughput/delay tradeoff than all prior schemes, and falls well outside the Pareto frontier for those schemes. For example, in the single user scenario, the \name configuration with $d_{t}=100$ ms achieves up to 29\% higher throughput than Cubic+Codel, Copa and Vegas. Though PCC-Vivace, Cubic and BBR achieve slightly higher throughput (4\%) than this \name configuration, their delay values are considerably higher (67\%-6$\times$). The multi-user scenario showed similar results. For instance, \name achieves 38\%, 41\% and 31\% higher average throughput than Cubic+Codel, Copa and Vegas, respectively, with delay values up to 29\% lower.

%BBR achieves 5\% higher throughput than \name, but also incurs 120\% higher delay values.

\if 0
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/explicit_utilization.pdf}
        \caption{Utilization}
        \label{fig:explicit:utilization}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/explicit_delay.pdf}
        \caption{Delay}
        \label{fig:explicit:delay}
    \end{subfigure}
    \caption{\small{\bf \name vs explicit flow control ---} \name achieves similar utilization and mean delay as XCP across all traces. Compared to RCP and VCP, \name achieves 20\% more utilization.}
    \label{fig:explicit}
\end{figure}



\textbf{Comparing \name with existing explicit flow control schemes:} We evaluate \name against two traditional explicit flow control schemes, XCP~\cite{xcp} and RCP~\cite{rcp}, as well as another in-network signaling scheme, VCP~\cite{VCP} which uses succinct feedback to only signal  a fixed multiplicative/additive increase or multiplicative decrease. We implemented each scheme as a Mahimahi qdisc~\cite{mahimahi}.

For XCP, we used constant values of $\alpha=0.55$ and $\beta=0.4$, which the authors note are the highest permissible stable values that achieve the fastest possible link rate convergence. We initially began using an unedited version of XCP in our experiments. However, we quickly observed that this version of XCP (XCP\_Original) performed significantly worse than \name, achieving far higher delay (\Fig{xcp} in Appendix~\ref{app:xcp} presents this comparison). The reason is that XCP computes aggregate feedback values ($\phi$) once per RTT, which it uses to calculate per-packet feedback. In scenarios where link capacity suddenly drops, it may take XCP a complete RTT before it recomputes the aggregate feedback to reduce the window. To improve XCP's performance, we modified XCP\_Original to recompute aggregate feedback \textit{on each packet} based on the rate and delay measurements from the past RTT; we refer to this version as XCP throughout the paper. This modification improves reactivity and helps control delays in the presence of rapid drops in link rate. We discuss and evaluate other potential modifications of XCP in Appendix~\ref{app:xcp}. For RCP and VCP, we used the author-specified parameter values of $\alpha=0.5$ and $\beta=0.25$, and $\alpha=1$, $\beta=0.875$ and $\kappa=0.25$, respectively. 

\Fig{explicit} shows utilizations and mean per packet delays achieved by each of these schemes over eight different cellular link traces. As shown, \name is able to achieve similar throughput and mean delay to the best performing explicit flow control scheme, XCP, without using multibit per-packet feedback. We note that XCP's 95$^{th}$ percentile per-packet delays are 40\% higher than \name's (Appendix~\ref{app:xcp}).
\name is also able to outperform RCP and VCP. Specifically, \name achieves 20\% higher utilization than RCP. This improvement stems from the fact that RCP is a rate based protocol (not a window based protocol)---by signaling rates, RCP is slower to react to link rate fluctuations (Appendix~\ref{app:explicit} illustrates this behavior). \name also achieves 20\% higher throughput than VCP, while incurring only a 10\% higher mean per-packet-delay.
\fi

\subsection{Coexistence with Various Bottlenecks: \name is able to properly coexist with different combinations of \name and non-\name bottlenecks}
\label{ss:coexistence}

\if 0
\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/ts_multi.pdf}
     \caption{\small {\bf Coexistence of multiple \name bottlenecks ---} \name{}'s rate tracks the bottleneck closely.}
     \label{fig:ts_multilink}
\end{figure}
\fi

\textbf{Coexistence with \name bottlenecks:} 
\Fig{througput-delay:up+down} compares \name and prior protocols on a network path with two cellular links. In this scenario, \name{} tracks the bottleneck link rate and achieves a better throughput/delay tradeoff than prior schemes, and again sits well outside the Pareto frontier for those schemes.

\if 0
\Fig{ts_multilink} lists throughput and queuing delay values for an \name{} flow traversing two different emulated cellular links, each running \name{}. At any given time, either one of the two links can be the bottleneck link. The dashed line in the Figure's top graph shows the bottleneck link rate across the two cellular links. As shown, \name{} is able to closely track the bottleneck link rate, and sends traffic just below that rate to maintain low queuing delays. This behavior is also highlighted in \Fig{througput-delay:up+down}, which evaluates \name and prior protocols on a network path with two cellular links. In this scenario, \name{} achieves a better throughput/delay tradeoff than prior schemes, and again sits well outside the Pareto frontier for those schemes.
 \begin{figure}[tbh]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/abccubic.pdf}
     \vspace{-3mm}
     \caption{\small {\bf Coexistence with non-\name bottlenecks ---} \name behaves like Cubic when the wired link is the bottleneck. When the cellular link is the bottleneck, \name follows accelerates and brakes to achieve low delays and high utilization.}
     \label{fig:ts_droptail_cell}
\end{figure}
\fi


 
 \begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/abccubic_visualization_v3.pdf}
     \vspace{-5mm}
     \caption{\small {\bf Coexistence with non-\name bottlenecks ---} \name tracks the ideal rate closely (fair share) and reduces queuing delays in the absence of cross traffic (white region). }
     \label{fig:ts_droptail_cell_visualization}
     \vspace{-4mm}
\end{figure}

\textbf{Coexistence with non-\name bottlenecks:} 
\Fig{ts_droptail_cell_visualization} illustrates throughput and queuing delay values for an \name flow traversing a network path with both an emulated wireless link and an emulated 12 Mbits/s fixed rate (wired) link. The wireless link is configured to run \name, while the wired link operates a droptail buffer. \name shares the wired link with on-off cubic cross traffic. In the absence of cross traffic (white region), the wireless link is always the bottleneck. However, with cross traffic (yellow and grey regions), due to contention, the wired link can become the bottleneck. In this case, \name's fair share on the wired link is half of the link's capacity (i.e., 6 Mbit/s).
If the wireless link rate is lower than the fair share (yellow region), the wireless link remains the bottleneck; otherwise, the wired link becomes the bottleneck (grey region).

The black dashed line in the top graph represents the ideal throughput (i.e., that of the bottleneck link) for the \name flow throughout the experiment. As shown, in all regions, \name is able to track the ideal rate closely, even as the bottleneck shifts. In particular, in the absence of cross traffic, \name continually achieves low delays while maintaining high link utilization. Similarly, with cross traffic, \name appropriately tracks the wireless link rate (yellow region) or achieves its fair share of the wired link (grey region) like Cubic. In the former cross traffic scenario, increased queuing delays are due to congestion caused by the Cubic flow on the wired link. Further, deviations from the ideal rate in the latter cross traffic scenario can be attributed to the fact that an \name flow (while running as Cubic) takes time to converge to its fair share.


%When the wireless link is the bottleneck (white and yellow regions), the ideal rate for \name is the wireless link rate. When the wired link is the bottleneck (grey region), the ideal rate is the fairshare rate of 6 Mbit/s. In all the regions, \name tracks the ideal rate closely. In the absence of any cross traffic (white region), \name achieves low delays while maintaining high link utilization. In the yellow region, \name tracks the wireless link rate, the increase in queuing delays is due to congestion cause by cubic flow on the wired link. When the wired link is the bottleneck (grey region), \name behaves like Cubic and is able to achieve its fairshare of rate. Note that, deviation from ideal rate in this region can attributed to the fact that an \name (while running as Cubic) takes time to converge to its fairshare.

\subsection{Coexistence: \name competes fairly with both \name flows and non-\name flows}
\label{ss:flow_fairness}

\if 0
\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/fairness.pdf}
     \vspace{-8mm}
     \caption{\small pg{{\bf Coexistence with non-\name flows ---}} \name flows compete fairly with each other while maintaining low aggregate queuing delays.}
     \label{fig:fairness}
\end{figure}
\fi

\if 0
\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/jain.pdf}
     \vspace{-4mm}
     \caption{\small \pg{\bf Fairness ---} Jain Index captures fairness for competing flows. Ideal Jain Index is 1. \name and Cubic's Jain Index is close to 1 in all the cases.}
     \label{fig:jain}
     \vspace{-4mm}
\end{figure}
\fi

\textbf{Coexistence among \name flows:} We simultaneously run multiple \name flows on a fixed 24 Mbits/s wired bottleneck link. We varied the number of competing flows from 2 to 32, and the duration of each run was 60 s. In each case, the Jain Fairness Index(~\cite{jain1999throughput}) was within 5\% from the ideal fairness value of 1, highlighting \name's ability to ensure fairness.

%\pg{\textbf{Coexistence among \name flows:} To illustrate intra-flow fairness for \name, we simultaneously run multiple flows \name on a fixed 24 Mbits/s bottleneck link. For comparison we also include results for Cubic, the duration of each experiment was 60s. \Fig{jain} lists Jain Fairness Index ~\cite{jain1999throughput} for different number of competing flows. Jain Index for \name and Cubic remains close to the ideal value of 1 in all cases. The additive increase in \name ensures fairness among \name flows.}

%\textbf{Coexistence among \name flows:} We consider a scenario in which five \name flows are competing on a fixed 24 Mbits/s link. At the beginning of the experiment, a new \name flow is introduced every 30 seconds, and at the end of the experiment, an \name flow is terminated every 30 seconds. \Fig{fairness} illustrates that the \name flows are able to quickly adapt to both arrivals and departures of other \name flows, achieving inter-flow fairness throughout the entire experiment. The queuing delays remain close to 0 during the entire duration of the experiment. There is a slight $\sim$5 ms increase in queuing delay between the 90--180 second experiment time frame, which includes the maximum of five concurrent \name flows. This delay can be attributed to extra packets in the network that result from the additive increase mechanism used by each of the five \name flows.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/coexist_ABC.pdf}
        \vspace{-7mm}
        \caption{ABC}
        \label{fig:non-abc-flow:abc}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/coexist_RCP.pdf}
        \vspace{-7mm}
        \caption{RCP's Zombie List}
        \label{fig:non-abc-flow:rcp}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small{\bf Coexistence with non-\name flows ---} Across all scenarios, the standard deviation for \name flows is small and the flows are fair to each other. Compared to RCP's Zombie List strategy, \name's max-min allocation provides better fairness between \name and non-\name flows. With \name's strategy, the difference in average throughput of \name and Cubic flows is under 5\%.}
    \label{fig:non-abc-flow}
    \vspace{-4mm}
\end{figure}

\textbf{Coexistence with non-\name flows:} We consider a scenario where three \name and three non-\name (in this case, Cubic) long-lived flows share the same 96 Mbits/s bottleneck link. In addition, we create varying numbers of short flows (each of size 10 KB) with flow arrival times generated by a Poisson process to offer fixed average loads. We consider several different total offered load values. Our results summarize 10 runs, each of 40 seconds. We compare \name's strategy to coexist with non-\name flows to RPC's Zombie list approach (\S\ref{s:fairness}).

\Fig{non-abc-flow} shows the mean and standard deviation throughput values achieved by the \name and Cubic flows. As shown in \Fig{non-abc-flow:abc}, \name's coexistence strategy allows \name and Cubic flows to fairly share the bottleneck link across all offered load values. Specifically, the difference in average throughput between the \name and Cubic flows is under 5\%. In contrast, \Fig{non-abc-flow:rcp} shows that RCP's coexistence strategy gives higher priority to Cubic flows. This discrepancy increases as the offered load increases, with Cubic flows achieving 17-165\% higher throughput than \name flows. The reason, as discussed in ~\Sec{fairness}, is that long-lived Cubic flows receive higher throughput than the average throughput that RCP intends for Cubic flows. This leads to unfairness because RCP attempts to match average throughput values for each scheme.\Fig{non-abc-flow} also shows that the standard deviation of \name flows is small (under 10\%) across all scenarios. A small standard deviation implies that in each run of the experiment, the throughput values for each of the three concurrent \name flows are close to each other, implying fairness across \name flows. Importantly, the standard deviation values for \name are smaller than those for Cubic. Thus, \name flows converge to fairness faster than Cubic flows do.

\if 0
\textbf{Coexistence with non-\name flows:} To evaluate \name's ability to fairly coexist with non-\name flows, we compare \name's coexistence strategy with RPC's Zombie list approach (\S\ref{s:fairness}). We consider a scenario where three \name and three non-\name (in this case, Cubic) long-lived flows share the same bottleneck link. In addition, we create varying numbers of short flows (each of size 10 KB) with flow arrival times generated by a Poisson process to offer fixed average loads. We consider several different total offered load values. Our results summarize 10 runs, each of 40 seconds. \Fig{non-abc-flow} shows the mean and standard deviation throughput values achieved by the \name and Cubic flows. As shown in \Fig{non-abc-flow:abc}, \name's coexistence strategy allows \name and Cubic flows to fairly share the bottleneck link across all offered load values. Specifically, the difference in average throughput between the \name and Cubic flows is under 5\%. In contrast, \Fig{non-abc-flow:rcp} shows that RCP's coexistence strategy gives higher priority to Cubic flows. This discrepancy increases as the offered load increases, with Cubic flows achieving 17-165\% higher throughput than \name flows. The reason, as discussed in ~\Sec{fairness}, is that long-lived Cubic flows receive higher throughput than the average throughput that RCP intends for Cubic flows. This triggers unfairness because RCP attempts to match average throughput values for each scheme.
\fi

\subsection{Additional Results: \name improves real applications, and its benefits persist across different workloads and network latencies}
\label{ss:other_results}


\begin{figure}
    \centering
        \includegraphics[width=0.8\columnwidth,height=1.5in]{images/short_flow.pdf}
        \vspace{-5mm}
    \caption{\small{\bf \name's robustness to flow size ---} With a single backlogged \name flow and multiple concurrent application-limited \name flows, all flows achieve high utilization and low queuing delays.}
    \label{fig:traffic-char}
    \vspace{-4mm}
\end{figure}

\textbf{Application-limited flows:} We created a single long-lived \name flow that shared a cellular link with 200 application-limited \name flows that send traffic at an aggregate of 1 Mbit/s. \Fig{traffic-char} shows that, despite the fact that the application-limited flows do not have traffic to properly respond to \name's feedback, the \name flows (in aggregate) are still able to achieve low queuing delays and high link utilization.

\begin{figure}[t]
     \centering
     \begin{subfigure}[t]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/rtt_utilization_v4.pdf}
    \vspace{-6mm}
    \subcaption{Utilization}
    \end{subfigure}
    \begin{subfigure}[t]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/rtt_delay_v4.pdf} \vspace{-6mm}
    \subcaption{ per-packet queuing delay}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf Impact of propagation delay on performance ---} On a Verizon cellular network trace with different propagation delays, \name achieves a better throughput/delay tradeoff than all other schemes.}
    \label{fig:rtt}
    \vspace{-4mm}
 \end{figure}

\textbf{\name's sensitivity to network latency:} Thus far, our emulation experiments have considered fixed minimum RTT values of 100 ms. To evaluate the impact that propagation delay has on \name's performance, we used a modified version of the experimental setup from \Fig{aggregate-statistics}. In particular, we consider RTT values of 20 ms, 50 ms, 100 ms, and 200 ms. \Fig{rtt} shows that, across all propagation delays, \name is still able to outperform all prior schemes, again achieving a more desirable throughput/latency trade off. \name's benefits persist even though schemes like Cubic+Codel and Cubic+PIE actually improve with increasing propagation delays. Performance with these schemes improves because bandwidth delay products increase, making Cubic's additive increase more aggressive (improving link utilization).

\textbf{\name's improvement on real applications:} We evaluated \name's ability to improve performance for real user-facing applications by considering a multiplayer interactive game, Slither.io~\cite{slither}. We loaded Slither.io using a Google Chrome browser which ran inside an emulated cellular link with a background backlogged flow (generated with iperf). We considered three different congestion control protocols for the backlogged flow: Cubic, Cubic+Codel, and \name. As expected, Cubic is able to fully utilize the link, but adds excessive queuing delays which hinder gameplay. In contrast, Cubic+Codel reduces queuing delays (improving user experience in the game), but underutilizes the link. Only \name is able to achieve both high link utilization for the backlogged flow and low queuing delays for the game. A video demo of this experiment can be viewed at \url{https://youtu.be/Dauq-tfJmyU}.

\textbf{Perfect future capacity knowledge:} We considered a variant of \name, PK-\name, which knows an entire emulated link trace in advance. This experiment reflects the possibility of resource allocation predictions at cellular network base stations. Rather than using an estimate of the current link rate to compute a target rate (as \name does), PK-\name uses the exact link rate that is expected 1 RTT value in the future. Using the same setup as in \Fig{througput-delay:up}, PK-\name is able to reduce 95$^{th}$ percentile per-packet-delays from 97 ms to 28 ms, compared to \name, while achieving the same link utilization ($\sim$90\%).

==> hari_coexistence_wired.tex <==
\section{Coexistence with wired bottlenecks}
\label{s:multiple-bottleneck}
An \name{} flow can encounter both \name and non-\name bottleneck routers. For example, a Wi-Fi user's traffic will traverse both a Wi-Fi router (running \name{}) and an ISP router (not running \name{}); either router could be the bottleneck at any given time. To handle such situations, \name flows must be able to detect and react to traditional congestion signals (e.g., drops or ECN marks), and they must determine when to ignore accelerate feedback from \name routers. First, we describe how can \name senders incorporate feedback from  non-\name routers for coexistence. Then, we show how we can repurpose ECN for \name feedback, without compromising the \name sender's ability to infer congestion based on ECN markings from non-\name routers. 

\subsection{Incorporating feedback from non-\name Routers}
\label{ss:multiple-bottleneck}

\name senders maintain two congestion windows, one for tracking the available rate on \name routers ($w_{abc}$), and one for tracking the rate on non-\name{} routers ($w_{cubic}$). $w_{abc}$ obeys accelerates/brakes using Eq.~\eqref{eq:abc_cwnd_rule}, while $w_{cubic}$ follows Cubic's standard window update rule~\cite{cubic} and responds to drop and ECN signals.\footnote{We discuss how \name senders can distinguish between accelerate/brake and ECN marks in \S\ref{ss:deployment}.} An \name sender must send packets to match the minimum of the two available rates. Thus, \name uses min($w_{abc}$, $w_{cubic}$) as its congestion window. 
Although we chose to behave as Cubic on non-\name routers, the same technique can be used to emulate other protocols.

With this approach, the window that is not the bottleneck could grow very large. For example, when a non-\name router is the bottleneck, the \name router will continually send accelerates. These accelerates do not cause the sender to transmit new packets, but they do cause $w_{abc}$ to grow. Thus if the \name router becomes the bottleneck, it will (temporarily) incur very large queues. To prevent this problem, \name senders cap both $w_{abc}$ and $w_{cubic}$ to twice the number of in-flight packets.

 \begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/abccubic_cwnd.pdf}
     \vspace{-5mm}
     \caption{\small {\bf Coexistence with non-\name bottlenecks ---} When the wired link is the bottleneck, \name becomes limited by $w_{cubic}$ and behaves like a cubic flow. When the wireless link is the bottleneck, \name uses $w_{abc}$ to achieve low delays and high utilization.}
     \label{fig:ts_droptail_cell}
     \vspace{-4mm}
\end{figure}

\Fig{ts_droptail_cell} shows the throughput and aggregate queuing delay for an \name flow traversing a path with an \name-capable wireless link and a wired link with a droptail queue. For illustration, we vary the capacity of the wireless link in a series of steps every 5 seconds. Over the experiment, the bottleneck switches between the wired and wireless links several times. \name is able to adapt its behavior both quickly and accurately. Depending on which link is the bottleneck, either $w_{cubic}$ or $w_{abc}$ becomes smaller and controls the rate of the flow. When the wireless link is the bottleneck, \name maintains low queuing delay, whereas the queuing delay exhibits standard Cubic behavior when the wired link is the bottleneck. In either case, the larger window grows to the upper limit of 2$\times$ the smaller window. Notice that $w_{cubic}$ does not limit \name's ability to increase its rate when the wireless link is the bottleneck. At these times (e.g., around the 70~s mark), as soon on $w_{abc}$ increases, the inflight packets  and the cap on $w_{cubic}$ increases, and $w_{cubic}$ rises immediately.

\subsection{Deployment with ECN}
\label{ss:deployment}

%In this section, we describe how ECN can be repurposed to signal accel-brake marks. 

%This distinction between feedback from \name and non-\name routers is critical for coexistence with non-\name bottleneck (\S\ref{s:multiple-bottleneck}). 
We start with an overview of standard ECN, and then present our practical deployment solution. 

\textbf{ECN Overview:} IP packets have two ECN-related bits: ECT and CE. These two bits are traditionally interpreted as follows:
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & ECN-Capable Transport ECT(1)\\
 1 & 0 & ECN-Capable Transport ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
Routers interpret both (01) and (10) to indicate that a connection is ECN capable, and routers change those bits to (11) to mark a packet with ECN. Upon receiving an ECN mark (11), a receiver sets the sets the {\em ECN Echo (ECE)} flag to signal congestion to the sender.

%, a receiver sets the {\em ECN Echo (ECE)} flag in {\em all} subsequent ACKs until it receives a {\em Congestion Window Reduced (CWR)} notification from the sender, \ie a packet with the CWR flag in the TCP header set to 1. Thus receivers echo ECN marks for a full round-trip worth of ACKs.

\textbf{Deployment:} \name reinterprets the ECT and CE ECN bits as follow:

%\name can coexist with non-\name  routers (using ECN for signalling congestion) by reinterpreting the ECT and CE ECN bits as follow:
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & \textit{accelerate} ECT(1)\\
 1 & 0 & \textit{brake} ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
\name senders can mark accelerates using (01), and \name routers can signal brakes by flipping the bits to (10). Both (01) and (10) equivalently indicate ECN capable transport to legacy routers, which can continue to use (11) to signal congestion.

With this design, receivers must be able to convey both standard ECN signals and accelerates/brakes for \name. ECN feedback can be signaled using the ECE flag. For \name feedback, we repurpose the NS (nonce sum) bit, which was originally proposed to ensure ECN feedback integrity~\cite{nonce} but has been reclassified as historic~\cite{accurate-ecn} due to lack of deployment. Thus, our deployment solution only requires simple modifications to TCP receivers.


\textbf{Deployment in Cellular Networks:} Cellular networks commonly split TCP connections and deploy proxy at the edge~\cite{wang2011untold,ravindranath2013timecard}. In such a network, it is unlikely that any non-\name router will act as the bottleneck and interfere with the accel-brake markings from the \name router. In this case where non-\name routers do not use ECN, deploying \name is relatively straightforward and doesn't require any receiver modifications. \name senders can simply use either (01) or (10) ECN markings to signal an accelerate, and routers can use (11) to indicate a brake.  The unmodified receiver can echo this feedback using the ECE flag. The proxy can be modified to run custom \name senders, and the base station can be modified to act as a \name router.


==> hari_evaluation.tex <==
\section{Evaluation}
\label{s:eval}

In this section, we evaluate \name using both our Wi-Fi implementation and trace-driven emulation of cellular networks. We evaluate the following metrics:
\begin{CompactEnumerate}
\item \textbf{Performance:} We measure \name's ability to achieve low delay and high throughput and compare \name to end-to-end schemes, AQM schemes, and explicit control     schemes (\S\ref{ss:performance}).
\item \textbf{Multiple Bottlenecks:} We test \name in scenarios with multiple \name bottlenecks and mixtures of \name and non-\name bottlenecks (\S\ref{ss:coexistence}).
\item \textbf{Coexistence:} We evaluate \name's fairness mechanisms both in competition with other \name flows and with non-\name flows (\S\ref{ss:flow_fairness}).
\item \textbf{Additional Considerations:} We evaluate how \name performs with application-limited flows and different network delays. We conclude with a demonstration of \name's impact on a real application's performance (\S\ref{ss:other_results}).
\end{CompactEnumerate}

\begin{figure*}[t]
    \centering
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/single_downlink_v3.pdf}
        \vspace{-7mm}
        \caption{Downlink}
        \label{fig:througput-delay:down}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/single_uplink_v3.pdf}
        \vspace{-7mm}
        \caption{Uplink}
        \label{fig:througput-delay:up}
    \end{subfigure}
    \begin{subfigure}[tbh]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/weinstein_multi_v3.pdf}
        \vspace{-7mm}
        \caption{Uplink+Downlink}
        \label{fig:througput-delay:up+down}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf ABC vs. previous schemes on three Verizon cellular network traces ---} In each case, ABC outperforms all other schemes and sits well outside the Pareto frontier of previous schemes (denoted by the dashed lines). }
    \label{fig:througput-delay}
    \vspace{-4mm}
\end{figure*}

\subsection{Prototype Implementation}
\label{s:prototype implementation}
\noindent {\bf \name transport:} We implemented \name endpoints in Linux as kernel modules using the pluggable TCP API. 

\noindent{\bf \name router:} We implemented \name as a Linux queuing discipline (qdisc) kernel module using OpenWrt, an open source operating system for embedded networked devices~\cite{openwrt}. We used a NETGEAR WNDR 3800 router configured to 802.11n. However, we note that our implementation is portable as OpenWrt is supported on numerous other commodity Wi-Fi routers.

%An \name router must be able to estimate link capacities, compute target rates, and mark packets as accelerates or brakes. 
\name's WiFi link rate prediction strategy exploits the inner workings of the MAC 802.11n protocol, and thus requires fine-grained values at this layer. In particular, the \name qdisc must know A-MPDU sizes, Block ACK receive times, and packet transmission bitrates. Unfortunately, these values are not natively exposed to Linux router qdiscs, and instead are only available at the network driver. To bridge this gap, we modified the router to log the relevant MAC layer data in the cross-layer socket buffer data structure (skb) that it already maintains per packet. 


\subsection{Experimental Setup}
\label{ss:setup}

Experiments performed over a live Wi-Fi network used the \name router described in Section~\ref{s:prototype implementation}. We also evaluated \name using  Mahimahi~\cite{mahimahi} emulating multiple cellular networks (Verizon LTE, AT\&T, and TMobile) using packet delivery traces that were captured directly on those networks. We used separate traces to emulate the cellular uplinks and downlinks. We note that these traces include outages, highlighting \name's ability to handle ACK losses.

We compare \name to end-to-end protocols designed for cellular networks (Sprout~\cite{sprout} and Verus~\cite{verus}), loss-based end-to-end protocols both with and without AQM (Cubic protocol~\cite{cubic}, Cubic+Codel~\cite{codel}, and Cubic+PIE~\cite{pie}), recently-proposed end-to-end protocols (BBR~\cite{bbr}, Copa~\cite{copa}, PCC Vivace-Latency aka PCC)~\cite{vivace}), TCP Vegas~\cite{vegas}), and explicit control protocols (XCP~\cite{xcp}, RCP~\cite{rcp} and VCP~\cite{VCP}). We used TCP kernel modules to evaluate \name, BBR, Cubic, PCC, and Vegas; for these schemes, we generated traffic by using iperf~\cite{iperf} to create a backlogged flow. For the schemes that are not implemented as a TCP kernel module (Copa, Sprout, Verus), we used the UDP implementations and traffic generation applications provided by the protocol authors. \pg{For evaluation over traces, we used our own implementation of XCP, RCP and VCP (implemented as a qdisc in mahimahi)}. We used Mahimahi's support of Cubic and Pie to evaluate AQM. \name's target rate calculation (Equation~\ref{eq:abctargetrule}) used $\eta=0.98$, and $\delta=133$ ms. Unless otherwise noted, our emulated cellular  experiments used a minimum RTT of 100 ms and a buffer size of 250 packets. \pg{For cellular traces, we assumed that the link rate is known at the \name router (~\cite{3GPP}).} 


\subsection{Performance: \name achieves low delay, high throughput, and outperforms existing schemes}
\label{ss:performance}


\begin{figure}[t]
     \centering
     \begin{subfigure}[tbh]{\columnwidth}
     %\includegraphics[width=1.0\columnwidth]{images/wifi_single_v2.pdf}
     \includegraphics[width=1.0\columnwidth]{images/new_aggregare_utilization_v2.pdf}
    \vspace{-7mm}
    \subcaption{Utilization}
    \label{fig:aggregate-statistics:utilization}
    \end{subfigure}
    \vspace{-1mm}
    \begin{subfigure}[tbh]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/new_aggregare_95delay_v2.pdf}
    \vspace{-6mm}
    \subcaption{$95^{th}$ percentile per-packet delay}
    \label{fig:aggregate-statistics:delay}
    \end{subfigure}
    \vspace{-4mm}
    \caption{\small {\bf 95$^{th}$ percentile per-packet delay across 8 cellular link traces ---} On average, ABC achieves similar  delays  and  38\%  higher  utilization  than  Copa  and Cubic+Codel.  BBR,  PCC,  and  Cubic  achieve  slightly  higher throughput   than   ABC,   but   incur 180-400\% higher  95$^{th}$ percentile  delay than \name.}
    \label{fig:aggregate-statistics}
    \vspace{-4mm}
 \end{figure}
\Fig{througput-delay:down} and~\ref{fig:througput-delay:up} show the utilization and 95$^{th}$ percentile per packet delay that a single backlogged flow achieves using each aforementioned congestion control protocol on two Verizon LTE cellular link traces. As shown, \name exhibits a better (i.e., higher) throughput/delay tradeoff than all prior schemes. In particular, \name sits well outside the Pareto frontier of the existing schemes, which houses the prior schemes that achieve higher throughput or lower delay than any other prior schemes.

Further analysis of Figures~\ref{fig:througput-delay:down} and~\ref{fig:througput-delay:up} reveals that Cubic+Codel, Cubic+PIE, Copa, and Sprout are all able to achieve low delays (comparable to \name). However, these schemes heavily underutilize the link. The reason is that, though these schemes are able to infer queue buildups and can react to them to reduce delays, they lack a way of quickly inferring increases in link capacity (a common occurrence on time-varying wireless links), leading to underutilization. In contrast, schemes like BBR, Cubic, and PCC are able to rapidly saturate the network (achieving high utilization), but these schemes also quickly fill buffers and thus suffer from high queuing delays. Unlike prior schemes, \name is able to quickly react to \textit{both} increases and decreases in available link capacity, enabling high throughput and low delays.

We observed similar trends across a larger set of 8 different cellular network traces. \Fig{aggregate-statistics} summarizes the link utilization and $95^{th}$ percentile per-packet delays for each scheme across these scenarios. As shown, \name is able to achieve high throughput and lower delay than Sprout, Vegas, and Verus. \name also achieves 38\% higher throughput than Cubic+Codel and Copa, while only incurring 17\% higher $95^{th}$ percentile per-packet delays. Finally, though BBR, PCC, and Cubic achieve slightly higher link utilization values than \name (9\%, 12\%, and 18\%, respectively), they each incur significantly higher per-packet delays than \name (183\%, 394\%, and 382\%, respectively). Appendix~\ref{app:abc-throughput-delay} compares these schemes on mean per-packet delay over the same conditions, and shows the same trends.

\textbf{Comparison with Explicit Protocols:} \pg{For XCP, we used constant values of $\alpha=0.55$ and $\beta=0.4$, which the authors note are the highest permissible stable values that achieve the fastest possible link rate convergence. \name outperform XCP without using multi bit per-packet feedback. XCP achieves similar average throughput as \name but incurs 105\% higher delays. The performance difference can be attributed to the fact that \name's control rule is designed for variations in wireless links. Moreover, unlike \name which updates its feedback every packet, XCP computes aggregate feedback values ($\phi$) only once per RTT, which it uses to calculate per-packet feedback. In scenarios where link capacity suddenly drops, it may take XCP a complete RTT before it recomputes the aggregate feedback to reduce the window. To improve XCP's performance, we modified XCP to recompute aggregate feedback \textit{on each packet} based on the rate and delay measurements from the past RTT; we refer to this version as XCP$_{w}$ (short for XCP Wireless). This modification helps reduce delays, but the average 95\%ile per-packet delay is still 40\% higher than \name (\Fig{aggregate-statistics}). We also compared \name against two other explicit congestion control schemes , RCP and VCP.  \name outperforms both RCP and VCP, Appendix~\ref{app:explicit} summarizes their performance over 8 different cellular traces.}

 \begin{figure}[t]
     \centering
     \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/wifi_single_v2.pdf}
    \vspace{-7mm}
    \subcaption{Single user}
    \label{fig:wifi:single}
    \end{subfigure}
    \begin{subfigure}[t]{0.8\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/wifi_multiple_v3.pdf}
    \vspace{-7mm}
    \subcaption{Two users, shared queue}
    \label{fig:wifi:multiple}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf Throughout and mean delay on Wi-Fi ---} For the multi-user scenario, we report the sum of achieved throughputs and the average of observed \pg{$95^{th}$ percentile} delay across both users. We consider three versions of \name (denoted \name\_*) for different delay thresholds. All versions of \name outperform all prior schemes and sit outside the pareto frontier.}
    \label{fig:wifi}
    \vspace{-4mm}
 \end{figure}

\textbf{Wi-Fi:} We performed similar evaluations on a live Wi-Fi link, considering both single and multi-user scenarios. In this experiment, we excluded Verus and Sprout as they are designed specifically for cellular networks. \cut{schemes which include a TCP kernel module. \pg{For Copa, we used an experimental implementation over CCP~\cite{ccp-sigcomm18}.}} To mimic common Wi-Fi usage scenarios where endpoints can move to create variations in signal-to-noise ratios (and thus bitrates), we varied the Wi-Fi router's bitrate selections by varying the MCS index using the Linux \texttt{iw} utility; we alternated the MCS index between values of 1 and 7 every 2 seconds. In Appendix~\ref{fig:app:wifi_brownian}, we also list results for an experiment where we model MCS index variations as Brownian motion--results show the same trends as described below. The experiment was performed in a crowded computer lab. Thus, to reduce variations from channel contention, we report average performance values across three, 45 second runs. We considered three different \name delay threshold ($d_{t}$) values of 20 ms, 60 ms, and 100 ms; increasing \name's delay threshold will increase both observed throughput and RTT values.

%We performed similar evaluations on a live Wi-Fi link, considering both single and multi-user scenarios. In this experiment, we only considered schemes which include a TCP kernel module. \pg{For Copa, we used an experimental implementation over CCP~\cite{ccp-sigcomm18}.} To mimic common Wi-Fi usage scenarios where endpoints can move to create variations in signal-to-noise ratios (and thus bitrates), we varied the Wi-Fi router's bitrate selections by varying the MCS index using the Linux \texttt{iw} utility; we alternated the MCS index between values of 1 and 7 \pg{every 2} seconds. In Appendix~\ref{fig:app:wifi_brownian}, we also list results for an experiment where we model MCS index variations as Brownian motion--results show the same trends as described below. The experiment was performed in a crowded computer lab. Thus, to reduce variations from channel contention, we report average performance values across three, 45 second runs. We considered three different \name delay threshold ($d_{t}$) values of 20 ms, 60 ms, and 100 ms; increasing \name's delay threshold will increase both observed throughput and RTT values.

\pg{\Fig{wifi} shows throughput and \pg{$95^{th}$ percentile per packet delay }for each considered protocol, as measured using the \texttt{tcptrace} Linux utility. For the multi-user scenario, we report the sum of achieved throughputs and the average of observed $95^{th}$ percentile across both users. As shown, in both the single and multi-user scenarios, \name achieves a better throughput/delay tradeoff than all prior schemes, and falls well outside the Pareto frontier for those schemes. For example, in the single user scenario, the \name configuration with $d_{t}=100$ ms achieves up to 29\% higher throughput than Cubic+Codel, Copa and Vegas. Though PCC-Vivace, Cubic and BBR achieve slightly higher throughput (4\%) than this \name configuration, their delay values are considerably higher (67\%-6$\times$). The multi-user scenario showed similar results. For instance, \name achieves 38\%, 41\% and 31\% higher average throughput than Cubic+Codel, Copa and Vegas, respectively, though the delay values are upto 29\% lower. BBR achieves 5\% higher throughput than \name, but also incurs 120\% higher delay values.}

\if 0
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/explicit_utilization.pdf}
        \caption{Utilization}
        \label{fig:explicit:utilization}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/explicit_delay.pdf}
        \caption{Delay}
        \label{fig:explicit:delay}
    \end{subfigure}
    \caption{\small{\bf \name vs explicit flow control ---} \name achieves similar utilization and mean delay as XCP across all traces. Compared to RCP and VCP, \name achieves 20\% more utilization.}
    \label{fig:explicit}
\end{figure}



\textbf{Comparing \name with existing explicit flow control schemes:} We evaluate \name against two traditional explicit flow control schemes, XCP~\cite{xcp} and RCP~\cite{rcp}, as well as another in-network signaling scheme, VCP~\cite{VCP} which uses succinct feedback to only signal  a fixed multiplicative/additive increase or multiplicative decrease. We implemented each scheme as a Mahimahi qdisc~\cite{mahimahi}.

For XCP, we used constant values of $\alpha=0.55$ and $\beta=0.4$, which the authors note are the highest permissible stable values that achieve the fastest possible link rate convergence. We initially began using an unedited version of XCP in our experiments. However, we quickly observed that this version of XCP (XCP\_Original) performed significantly worse than \name, achieving far higher delay (\Fig{xcp} in Appendix~\ref{app:xcp} presents this comparison). The reason is that XCP computes aggregate feedback values ($\phi$) once per RTT, which it uses to calculate per-packet feedback. In scenarios where link capacity suddenly drops, it may take XCP a complete RTT before it recomputes the aggregate feedback to reduce the window. To improve XCP's performance, we modified XCP\_Original to recompute aggregate feedback \textit{on each packet} based on the rate and delay measurements from the past RTT; we refer to this version as XCP throughout the paper. This modification improves reactivity and helps control delays in the presence of rapid drops in link rate. We discuss and evaluate other potential modifications of XCP in Appendix~\ref{app:xcp}. For RCP and VCP, we used the author-specified parameter values of $\alpha=0.5$ and $\beta=0.25$, and $\alpha=1$, $\beta=0.875$ and $\kappa=0.25$, respectively. 

\Fig{explicit} shows utilizations and mean per packet delays achieved by each of these schemes over eight different cellular link traces. As shown, \name is able to achieve similar throughput and mean delay to the best performing explicit flow control scheme, XCP, without using multibit per-packet feedback. We note that XCP's 95$^{th}$ percentile per-packet delays are 40\% higher than \name's (Appendix~\ref{app:xcp}).
\name is also able to outperform RCP and VCP. Specifically, \name achieves 20\% higher utilization than RCP. This improvement stems from the fact that RCP is a rate based protocol (not a window based protocol)---by signaling rates, RCP is slower to react to link rate fluctuations (Appendix~\ref{app:explicit} illustrates this behavior). \name also achieves 20\% higher throughput than VCP, while incurring only a 10\% higher mean per-packet-delay.
\fi

\subsection{Coexistence with Various Bottlenecks: \name is able to properly coexist with different combinations of \name and non-\name bottlenecks}
\label{ss:coexistence}

\if 0
\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/ts_multi.pdf}
     \caption{\small {\bf Coexistence of multiple \name bottlenecks ---} \name{}'s rate tracks the bottleneck closely.}
     \label{fig:ts_multilink}
\end{figure}
\fi
\textbf{Coexistence with \name bottlenecks:} 
\pg{\Fig{througput-delay:up+down}, evaluates \name and prior protocols on a network path with two cellular links. In this scenario, \name{} tracks the bottleneck link rate and achieves a better throughput/delay tradeoff than prior schemes, and again sits well outside the Pareto frontier for those schemes.}
\if 0
\Fig{ts_multilink} lists throughput and queuing delay values for an \name{} flow traversing two different emulated cellular links, each running \name{}. At any given time, either one of the two links can be the bottleneck link. The dashed line in the Figure's top graph shows the bottleneck link rate across the two cellular links. As shown, \name{} is able to closely track the bottleneck link rate, and sends traffic just below that rate to maintain low queuing delays. This behavior is also highlighted in \Fig{througput-delay:up+down}, which evaluates \name and prior protocols on a network path with two cellular links. In this scenario, \name{} achieves a better throughput/delay tradeoff than prior schemes, and again sits well outside the Pareto frontier for those schemes.
 \begin{figure}[tbh]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/abccubic.pdf}
     \vspace{-3mm}
     \caption{\small {\bf Coexistence with non-\name bottlenecks ---} \name behaves like Cubic when the wired link is the bottleneck. When the cellular link is the bottleneck, \name follows accelerates and brakes to achieve low delays and high utilization.}
     \label{fig:ts_droptail_cell}
\end{figure}
\fi


\textbf{Coexistence with non-\name bottlenecks:} 
 
 \begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/abccubic_visualization_v3.pdf}
     \vspace{-5mm}
     \caption{\small \pg{{\bf Coexistence with non-\name bottlenecks ---}} \name tracks the ideal rate closely (fairshare) and reduces queuing delays in absence of cross traffic (white region). }
     \label{fig:ts_droptail_cell_visualization}
     \vspace{-4mm}
\end{figure}

\pg{\Fig{ts_droptail_cell_visualization} lists throughput and queuing delay values for an \name flow traversing a network path with an emulated wireless link and an emulated 12 Mbits/s fixed rate (wired) link. The wireless link is configured to run \name, while the wired link operates a droptail buffer. On-off cubic cross traffic shares the wired link with \name. In the absence of cross traffic (white region), the wireless link is the bottleneck. In the presence of cross traffic (yellow and grey regions), due to contention, the wired link can become the bottleneck. In this case, the fairshare of \name flow on the wired link is half the capacity of the wired link (6 Mbit/s). If the wireless link rate is lesser than the fairshare (yellow region), then the wireless link is the bottleneck. Otherwise (grey region), the wired link is the bottleneck. }

\pg{The black dashed line in the top graph represents ideal throughput for \name flow. When the wireless link is the bottleneck (white and yellow regions), the ideal rate for \name is the wireless link rate. When the wired link is the bottleneck (grey region), the ideal rate is the fairshare rate of 6 Mbit/s. In all the regions, \name tracks the ideal rate closely. In the absence of any cross traffic (white region), \name achieves low delays while maintaining high link utilization. In the yellow region, \name tracks the wireless link rate, the increase in queuing delays is due to congestion cause by cubic flow on the wired link. When the wired link is the bottleneck (grey region), \name behaves like Cubic and is able to achieve its fairshare of rate. Note that, deviation from ideal rate in this region can attributed to the fact that an \name (while running as Cubic) takes time to converge to its fairshare.}

\subsection{Coexistence: \name competes fairly with both \name flows and non-\name flows}
\label{ss:flow_fairness}

\if 0
\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/fairness.pdf}
     \vspace{-8mm}
     \caption{\small pg{{\bf Coexistence with non-\name flows ---}} \name flows compete fairly with each other while maintaining low aggregate queuing delays.}
     \label{fig:fairness}
\end{figure}
\fi

\if 0
\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/jain.pdf}
     \vspace{-4mm}
     \caption{\small \pg{\bf Fairness ---} Jain Index captures fairness for competing flows. Ideal Jain Index is 1. \name and Cubic's Jain Index is close to 1 in all the cases.}
     \label{fig:jain}
     \vspace{-4mm}
\end{figure}
\fi

\pg{\textbf{Coexistence among \name flows:} We simultaneously run multiple flows \name on a fixed 24 Mbits/s bottleneck link. We varied the number of competing flows from 2 to 32, the duration of each run was 60s. In each case, Jain Fairness Index(~\cite{jain1999throughput}) was within 5\% from the ideal fairness value of 1. Thus, \name ensures fairness.}

%\pg{\textbf{Coexistence among \name flows:} To illustrate intra-flow fairness for \name, we simultaneously run multiple flows \name on a fixed 24 Mbits/s bottleneck link. For comparison we also include results for Cubic, the duration of each experiment was 60s. \Fig{jain} lists Jain Fairness Index ~\cite{jain1999throughput} for different number of competing flows. Jain Index for \name and Cubic remains close to the ideal value of 1 in all cases. The additive increase in \name ensures fairness among \name flows.}

%\textbf{Coexistence among \name flows:} We consider a scenario in which five \name flows are competing on a fixed 24 Mbits/s link. At the beginning of the experiment, a new \name flow is introduced every 30 seconds, and at the end of the experiment, an \name flow is terminated every 30 seconds. \Fig{fairness} illustrates that the \name flows are able to quickly adapt to both arrivals and departures of other \name flows, achieving inter-flow fairness throughout the entire experiment. The queuing delays remain close to 0 during the entire duration of the experiment. There is a slight $\sim$5 ms increase in queuing delay between the 90--180 second experiment time frame, which includes the maximum of five concurrent \name flows. This delay can be attributed to extra packets in the network that result from the additive increase mechanism used by each of the five \name flows.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/coexist_ABC.pdf}
        \vspace{-7mm}
        \caption{ABC}
        \label{fig:non-abc-flow:abc}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/coexist_RCP.pdf}
        \vspace{-7mm}
        \caption{RCP's Zombie List}
        \label{fig:non-abc-flow:rcp}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small{\bf Coexistence with non-\name flows ---} Across all scenarios, the standard deviation for \name flows is small and the flows are fair to each other. Compared to RCP's Zombie List strategy, \name's max-min allocation provides better fairness between \name and non-\name flows. With \name's strategy, the difference in average throughput of \name and Cubic flows is under 5\%.}
    \label{fig:non-abc-flow}
    \vspace{-4mm}
\end{figure}

\textbf{Coexistence with non-\name flows:} We consider a scenario where three \name and three non-\name (in this case, Cubic) long-lived flows share the same bottleneck link. In addition, we create varying numbers of short flows (each of size 10 KB) with flow arrival times generated by a Poisson process to offer fixed average loads. We consider several different total offered load values. Our results summarize 10 runs, each of 40 seconds. To evaluate \name's ability to fairly coexist with non-\name flows, we compare \name's coexistence strategy with RPC's Zombie list approach (\S\ref{s:fairness}). \Fig{non-abc-flow} shows the mean and standard deviation throughput values achieved by the \name and Cubic flows. As shown in \Fig{non-abc-flow:abc}, \name's coexistence strategy allows \name and Cubic flows to fairly share the bottleneck link across all offered load values. Specifically, the difference in average throughput between the \name and Cubic flows is under 5\%. In contrast, \Fig{non-abc-flow:rcp} shows that RCP's coexistence strategy gives higher priority to Cubic flows. This discrepancy increases as the offered load increases, with Cubic flows achieving 17-165\% higher throughput than \name flows. The reason, as discussed in ~\Sec{fairness}, is that long-lived Cubic flows receive higher throughput than the average throughput that RCP intends for Cubic flows. This triggers unfairness because RCP attempts to match average throughput values for each scheme. \pg{Moreover, ~\ref{fig:non-abc-flow} also shows that the standard deviation of \name flows is small (under 10\%) across all scenarios. A small standard deviation implies that in each run of the experiment, throughput of the three concurrent \name flow is close to each other and \name flows are fair to each other. The standard deviation for \name is smaller than Cubic, thus, \name flows converge to fairness faster than Cubic flows.}

\if 0
\textbf{Coexistence with non-\name flows:} To evaluate \name's ability to fairly coexist with non-\name flows, we compare \name's coexistence strategy with RPC's Zombie list approach (\S\ref{s:fairness}). We consider a scenario where three \name and three non-\name (in this case, Cubic) long-lived flows share the same bottleneck link. In addition, we create varying numbers of short flows (each of size 10 KB) with flow arrival times generated by a Poisson process to offer fixed average loads. We consider several different total offered load values. Our results summarize 10 runs, each of 40 seconds. \Fig{non-abc-flow} shows the mean and standard deviation throughput values achieved by the \name and Cubic flows. As shown in \Fig{non-abc-flow:abc}, \name's coexistence strategy allows \name and Cubic flows to fairly share the bottleneck link across all offered load values. Specifically, the difference in average throughput between the \name and Cubic flows is under 5\%. In contrast, \Fig{non-abc-flow:rcp} shows that RCP's coexistence strategy gives higher priority to Cubic flows. This discrepancy increases as the offered load increases, with Cubic flows achieving 17-165\% higher throughput than \name flows. The reason, as discussed in ~\Sec{fairness}, is that long-lived Cubic flows receive higher throughput than the average throughput that RCP intends for Cubic flows. This triggers unfairness because RCP attempts to match average throughput values for each scheme.
\fi

\subsection{Additional Results: \name improves real applications, and its benefits persist across different workloads and network latencies}
\label{ss:other_results}


\begin{figure}
    \centering
        \includegraphics[width=0.8\columnwidth,height=1.5in]{images/short_flow.pdf}
        \vspace{-5mm}
    \caption{\small{\bf \name's robustness to flow size ---} With a single backlogged \name flow and multiple concurrent application-limited \name flows, all flows achieve high utilization and low queuing delays.}
    \label{fig:traffic-char}
    \vspace{-4mm}
\end{figure}

\textbf{Application-limited flows:} We created a single long-lived \name flow that shared a cellular link with 200 application-limited \name flows that send traffic at an aggregate of 1 Mbit/s. \Fig{traffic-char} shows that, despite the fact that the application-limited flows do not have traffic to properly respond to \name's feedback, the \name flows (in aggregate) are still able to achieve low queuing delays and high link utilization.

\begin{figure}[t]
     \centering
     \begin{subfigure}[t]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/rtt_utilization_v4.pdf}
    \vspace{-6mm}
    \subcaption{Utilization}
    \end{subfigure}
    \begin{subfigure}[t]{\columnwidth}
    \includegraphics[width=1.0\columnwidth]{images/rtt_delay_v4.pdf} \vspace{-6mm}
    \subcaption{ per-packet queuing delay}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf Impact of propagation delay on performance ---} On a Verizon cellular network trace with different propagation delays, \name achieves a better throughput/delay tradeoff than all other schemes.}
    \label{fig:rtt}
    \vspace{-4mm}
 \end{figure}

\textbf{\name's sensitivity to network latency:} Thus far, our emulation experiments have considered fixed minimum RTT values of 100 ms. To evaluate the impact that propagation delay has on \name's performance, we used a modified version of the experimental setup from \Fig{aggregate-statistics}. In particular, we consider RTT values of 20 ms, 50 ms, 100 ms, and 200 ms. \Fig{rtt} shows that, across all propagation delays, \name is still able to outperform all prior schemes, again achieving a more desirable throughput/latency trade off. \name's benefits persist even though schemes like Cubic+Codel and Cubic+PIE actually improve with increasing propagation delays. Performance with these schemes improves because bandwidth delay products increase, making Cubic's additive increase more aggressive (thereby improving link utilization).

\textbf{\name's improvement on real applications:} We evaluated \name's ability to improve performance for real user-facing applications by considering a multiplayer interactive game, Slither.io~\cite{slither}. We loaded Slither.io using a Google Chrome browser which ran inside an emulated cellular link with a background backlogged flow (generated with iperf). We considered three different congestion control protocols for the backlogged flow: Cubic, Cubic+Codel, and \name. As expected, Cubic is able to fully utilize the link, but adds excessive queuing delays which hinder gameplay. In contrast, Cubic+Codel reduces queuing delays (improving user experience in the game), but underutilizes the link. Only \name is able to achieve both high link utilization for the backlogged flow and low queuing delays for the game. A video demo of this experiment can be viewed at \url{https://youtu.be/Dauq-tfJmyU}.

\textbf{Perfect future capacity knowledge:} We considered a variant of \name, PK-\name, which knows an entire emulated link trace in advance. This experiment reflects the possibility of resource allocation predictions at cellular network base stations. Rather than using an estimate of the current link rate to compute a target rate (as \name does), PK-\name uses the exact link rate that is expected 1 RTT value in the future. Using the same setup as in \Fig{througput-delay:up}, PK-\name is able to reduce 95$^{th}$ percentile per-packet-delays from 97 ms to 28 ms, compared to \name, while achieving the same link utilization ($\sim$90\%).

==> hari_fairness.tex <==
\section{Fairness\\}
This section, presents how an \name flow can coexist fairly with both \name and non-\name flows.

\subsection{Coexistence with \name flows}
\label{s:coexist_abc_flow}
Multiple \name flows sharing the same bottleneck link should be able to compete fairly with one another. However, the basic window update rule described in ~\Sec{abc-sender} effectively employs a multiplicative-increase / multiplicative-decrease (MIMD) strategy,\footnote{All the competing \name senders will observe the same accelerate fraction, $f$, on average. Therefore, each flow will update its congestion window, $w$, in a multiplicative manner, to $2fw$, in the next RTT.} which does not provide fairness among contending flows (see \Fig{fairness:no_ai} for an illustration). To achieve fairness, we add an additive-increase (AI) component to the basic window update rule. Specifically,  \name senders adjust their congestion window on each ACK as follows:
\begin{equation}
w \leftarrow 
\begin{cases}
      w + 1 + 1/w & \text{if accelerate} \\
      w - 1 + 1/w & \text{if brake}
    \end{cases}
    \label{eq:abc_cwnd_rule}
\end{equation}
This rule increases the congestion window by 1 packet each RTT, in addition to reacting to received accelerate and brake ACKs. This additive increase, coupled with \name's MIMD response, makes \name a multiplicative-and-additive-increase / multiplicative-decrease (MAIMD) scheme. Chiu and Jain~\cite{chiujain} proved that MAIMD schemes converge to fairness (see also~\cite{akella2002exploring}).

To give intuition, we provide a simple informal argument for why including additive-increase gives \name fairness. Consider $N$ \name flows sharing a link, and suppose that in steady state, the router marks a fraction $f$ of the packets accelerate, and the window size of flow $i$ is $w_i$. To be in steady state, each flow must send 1 packet on average for each ACK that it receives. Now consider flow $i$. It will send $2f+1/w_i$ packets on average for each ACK: $2f$ for the two packets it sends on an accelerate (with probability $f$), and $1/w_i$ for the extra packet it sends every $w_i$ ACKs. Therefore, to be in steady state, we must have: $2f + 1/w_i = 1 \implies w_i = 1 / (1-2f)$. This shows that the steady-state window size for all flows must be the same, since they all observe the same fraction $f$ of accelerates! Hence, with equal RTTs, the flows will have the same throughput, and otherwise their throughput will be inversely proportional to their RTT. 

\Fig{fairness:ai} shows how with an AI component, competing \name flows achieve fairness. 

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/fairness_complicated_no_ai.pdf}
        \vspace{-7mm}
        \caption{\name w/o AI}
        \label{fig:fairness:no_ai}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{images/fairness_complicated_ai.pdf}
        \vspace{-7mm}
        \caption{\name with AI}
        \label{fig:fairness:ai}
    \end{subfigure}
    \vspace{-3mm}
    \caption{\small {\bf Fairness among competing \name flows ---} 5 flows with the same RTT start and depart one-by-one on a 24~Mbit/s link. The additive-increase (AI) component leads to fairness.}
    \label{fig:fairness}
    \vspace{-4mm}
\end{figure}


\subsubsection{Stability Analysis\\}
\label{s:stability_analysis}
\name's stability depends on the values of $\eta$ and $\delta$. $\eta$ determines the target link utilization, while $\delta$ controls how long it will take for a queue buildup to drain. In Appendix~\ref{app:stability} we prove the following result for a fluid model of the \name control loop.
\begin{theorem}
Consider a single \name link, traversed by $N$ \name flows. Let $\tau$ be the maximum round-trip propagation delay of the flows. \name is globally asymptotically stable if
\begin{align}
    \delta > \frac{2}{3} \cdot \tau.
\end{align}
Specifically, if $\mu(t) = \mu$ for $t > t_0$ (i.e., the link capacity stops changing after some time $t_0$), the enqueue/dequeue rate and the queuing delay at the \name router will converge to certain values $r^*$ and $x^*$ that depend on the system parameters and the number of flows. In all cases: $\eta \mu < r^* \leq \mu$.
\label{thm:stablity}
\end{theorem}
This stability criterion is simple and intuitive. It states that $\delta$ should not be much smaller than the RTT (i.e, the feedback delay). If $\delta$ is very small, \name reacts too forcefully to queue build up, causing under-utilization and  oscillations.\footnote{Interestingly, if the sources do not perform additive increase or if the additive increase is sufficiently ``gentle,'' \name is stable for any value of $\delta$. See the proof in Appendix~\ref{app:stability} for details.} Increasing $\delta$ well beyond $2/3\tau$ improves the stability margins of the feedback loop, but hurts responsiveness. In our experiments, we used $\delta=133$ ms for a propagation RTT of $100$ ms. 




\subsection{Coexistence with non-\name flows}
\label{s:fairness}
\name flows are potentially at a disadvantage when they share an \name bottleneck link with non-\name flows.\footnote{\name and non-\name flows may also share a non-\name  link, but in such cases, \name flows will behave like Cubic and compete fairly with other traffic (\Sec{multiple-bottleneck}).} If the non-\name flows fill up queues and increase queuing delay, the \name router will reduce \name's target rate. To ensure fairness in such scenarios, \name routers isolate \name and non-\name packets in separate queues. Using separate queues allows \name flows to achieve low delays even if the non-\name flows build up a large queue.

We assume that \name routers can determine whether a packet belongs to an \name flow. In some deployment scenarios, this is relatively straightforward. For example, many cellular networks deploy TCP proxies at the edge of the network~\cite{wang2011untold,ravindranath2013timecard}. In such networks, the operator can deploy \name at the proxy, and configure the base station to assume that all traffic from the proxy's IP address uses \name. Other deployment scenarios may require \name senders to set a predefined value in a packet field like the IPv6 flow label. 

The \name router assigns weights of $w_{\name}$ and 1-$w_{\name}$ to the \name and non-\name queues, respectively, and it schedules packets from the queues in proportion to their weights. In addition, \name's target rate calculation considers only \name's share of the link capacity (which is governed by the weights). The challenge is how to set the weights to ensure that the average throughput of long-running \name and non-\name flows is the same, irrespective of the number of flows.

Prior explicit control schemes have considered two approaches. XCP estimates the average window size of competing TCP flows based on their packet loss rate, using a TCP-Friendly-Rate-Control-like~\cite{ebcc} calculation. XCP then dynamically adjusts the weights to equalize the average window size for XCP and TCP flows. The problem with this approach is that the TFRC calculation can be inaccurate; for example, it fails to model BBR~\cite{bbr} flows. RCP estimates the number of flows in each queue using a data structure called a Zombie List~\cite{sred}, and then adapts the weights to equalize the average rate of RCP and TCP flows. This approach works well if all the flows are long-running, but it is not fair in the presence of short flows. When one queue has a large number of short flows (and hence a small average throughput), RCP increases the weight of that queue. However, the short flows cannot send faster, so the extra bandwidth is taken by long-running flows in the same queue, which get more throughput than long-running flows in the other queue. We demonstrate this unfairness experimentally in \S\ref{ss:flow_fairness}.

To overcome these drawbacks, \name routers use a more robust strategy for assigning weights to each queue. The router measures the average rate of the $K$ largest flows in each queue.\footnote{There are many algorithms for top-$K$ rate measurement~\cite{estan2002new, sivaraman2017heavy}. Our implementation uses the Space Saving Algorithm~\cite{metwally2005efficient} which requires $\mathcal{O}(K)$ space.} It considers any remaining flow in either queue to be short, and it calculates the total rate of the short flows in each queue by subtracting the rate of the largest $K$ flows from the queue's aggregate throughput. \name uses these rate measurements to estimate the rate demands of the flows. Using these demands, \name periodically computes the max-min fair rate allocation for the flows, and it sets the weight of each queue to be equal to the total max-min rate allocation of its flows. This algorithm ensures that long-running flows in the two queues achieve the same average rate, while correctly accounting for demand-limited short flows. 

To estimate the demand of the flows, the \name router assumes two things: 1) the demand for the top $K$ flows in each queue is X\% higher than the current throughput of the flow, and 2) the aggregate demand for the short flows in each queue is same as the current aggregate throughput of the short flows. Notice that if a top-$K$ flow is unable to increase its sending rate by X\%, its queue's weight will be larger than necessary. However, any unfairness in weight assignment is bounded by X\%. Small values of $X$ limit unfairness but can slow down convergence to the fair throughput allocation; our experiments use $X=10\%$. 

\begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{images/coexist_explanation.pdf}
     \vspace{-5mm}
     \caption{\small {\bf Coexistence with non-\name flows ---} \name flows compete fairly with non-\name flows.}
     \label{fig:coexist_explanation}
     \vspace{-4mm}
\end{figure}

\Fig{coexist_explanation} illustrates \name's fairness with non-\name flows. In this experiment, first two \name flows and then two Cubic flows arrive one after another. \name flows compete fairly with each other and with non-\name flows, and they achieve a low queuing delay despite the large Cubic queue.

==> hari_protocol.tex <==
\section{\name Protocol}
\label{s:design}

\name is a window-based protocol: the sender limits the number of packets in flight to the current congestion window. Window-based protocols react faster to the sudden onset of congestion than rate-based schemes (which set a transmission rate). On a wireless link, when the capacity drops and the sender stops receiving ACKs, \name will stop sending packets immediately, avoiding further queue buildup. In contrast, a rate-based protocol would take time to reduce its rate and may queue up a large number of packets at the bottleneck link in the meantime.

\name senders adjust their window size based on explicit feedback from \name routers. An \name router uses its current estimate of the link capacity and queuing delay to compute a {\em target rate}. The router then sets one bit of feedback in each packet to guide the senders towards the target rate. Each bit is echoed to a sender by a receiver in an ACK, and it signals either a one-packet increase (``accelerate'') or a one-packet decrease (``brake'') to the sender's congestion window.

%\subsection{The ABC Protocol}
We now present \name's design in the most basic case where all routers are \name-capable and all flows use \name. We later discuss how to extend the design to handle non-ABC routers and scenarios with competing non-ABC flows.

\subsection{ABC Sender\\}
\label{s:abc-sender}

On receiving an ``accelerate'' ACK, an \name sender increases its congestion window by 1 packet. This increase results in two packets being sent, one in response to the ACK and one due to the window size increase. On receiving a ``brake,'' the sender reduces its congestion window by 1 packet, preventing the sender from transmitting a new packet in response to the received ACK. As we discuss in \S\ref{s:fairness}, the sender also performs an additive increase of 1 packet per RTT to achieve fairness. For ease of exposition, let us ignore this additive increase for now.

Though each bit of feedback translates to a small change in the congestion window, when aggregated over an RTT, the feedback can express a large dynamic range of window size adjustments. For example, suppose a sender's window size is $w$, and the router marks accelerates on a fraction $f$ of packets in that window. Over the next RTT, the sender will receive $w \cdot f$ accelerates and $w - w \cdot f$ brakes. Then, the sender's window size one RTT later will be $w + w f - (w - w f) = 2wf$ packets. Thus, in one RTT, an ABC router can vary the sender's window size between zero ($f$ = 0) to double its current value ($f = 1$). The set of achievable window changes for the next RTT depends on the number of packets in the current window $w$; the larger $w$, the higher the granularity of control.

%reduces the window to zero, $f$ = 1/2 maintains the current window, and $f$ = 1 doubles it. 

In practice, \name senders increase or decrease their congestion window by the number of newly acknowledged bytes covered by each ACK. Byte-based congestion window modification is a standard technique in many TCP implementations~\cite{allman2003tcp}, and it makes \name robust to variable packet sizes and delayed, lost, and partial ACKs. For simplicity, we describe the design with packet-based window modifications in this paper.

%\name senders take special care to react to all ACKed packets in the event of delayed ACKs, and support byte-level congestion window modifications to support varying packet sizes. \ma{this sentence isn't clear.}


%An alternate design, can interpret accelerate-brake differently (e.g., increase/decrease window by 2 instead of 1), allowing \name to increase its rate faster than slow start. Slow start is deemed safe in the internet, anything faster might lead to excessive congestion on non-\name links. 
%Thus, using only a single-bit of feedback, an \name router can vary a sender's rate from 0 ($f$ = 0) to double ($f$ = 1) the current congestion window within a single RTT.
%Thus, values of 0, 1/2, and 1 for $f$ correspond to throttling, maintaining, or doubling the sender's current window within 1 RTT, respectively.

\subsection{\name Router\\}

\label{s:abc-router}
\textbf{Calculating the target rate:} %\pg{The rate control rule used by existing explicit schemes such as XCP and RCP were designed for fixed capacity links and are not well suited for time varying links.} 
\name routers compute the target rate $tr(t)$ using the following rule:
\begin{equation}
tr(t) = \eta {\mu(t)} - \frac{\mu(t)}{\delta} (x(t) - d_{t})^{+},
\label{eq:abctargetrule}
\end{equation}
where $\mu(t)$ is the link capacity, $x(t)$ is the observed queuing delay, $d_{t}$ is a pre-configured delay threshold, $\eta$ is a constant less than 1,  $\delta$ is a positive constant (in units of time), and $y^{+}$ is $\max(y,0)$. This rule has the following interpretation. When queuing delay is low ($x(t) < d_t$), \name sets the target rate to $\eta \mu(t)$, for a value of $\eta$ slightly less than 1 (e.g., $\eta = 0.95$). By setting the target rate a little lower than the link capacity, \name aims to trade a small amount of bandwidth for large reductions in delay,  similar to prior work~\cite{jain1996congestion,hull,avq}. However, queues can still develop due to rapidly changing link capacity and the 1 RTT of delay it takes for senders to achieve the target rate. \name uses the second term in Eq.~\eqref{eq:abctargetrule} to drain queues. Whenever $x(t) > d_t$, this term reduces the target rate by an amount that causes the queuing delay to decrease to $d_t$ in at most $\delta$ seconds. 

The threshold $d_t$ ensures that the target rate does not react to small increases in queuing delay. This is important because wireless links often schedule packets in batches. Queuing delay caused by batch packet scheduling does not imply congestion, even though it occurs persistently. To prevent target rate reductions due to this delay, $d_{t}$ must be configured to be greater than the average inter-scheduling time at the router.

\name's target rate calculation requires an estimate of the underlying link capacity, $\mu(t)$. In \Sec{linkrate}, we discuss how to estimate the link capacity in cellular and WiFi networks, and we present an implementation for WiFi.


\smallskip
\noindent {\bf Packet marking:} To achieve a target rate, $tr(t)$, the router computes the fraction of packets, $f(t)$, that should be marked as accelerate. Assume that the current {\em dequeue rate}\,---\,the rate at which the router transmits packets\,---\,is $cr(t)$. If the accelerate fraction is $f(t)$, for each packet that is ACKed, the sender transmits $2f(t)$ packets on average. Therefore, after 1 RTT, the {\em enqueue rate}\,---\,the rate at which packets arrive to the router\,---\,will be $2cr(t)f(t)$. To achieve the target rate, $f(t)$ must be chosen such that $2cr(t)f(t)$ is equal to $tr(t)$. Thus, $f(t)$ is given by:
\begin{equation}
f(t) = \min\Big\{\frac{1}{2} \cdot \frac{tr(t)}{cr(t)}, 1 \Big\}.
\label{eq:f}
\end{equation}
An important consequence of the above calculation is that $f(t)$ is computed based on the {\em dequeue} rate. Most explicit protocols compare the enqueue rate to the link capacity to determine the feedback (e.g., see XCP~\cite{xcp}). 
%However, it is difficult to determine the appropriate feedback based on the enqueue rate when the link capacity fluctuates significantly over time. 
\name uses the dequeue rate instead to exploit the ACK-clocking property of its window-based protocol. Specifically, Eq.~\eqref{eq:f} accounts for the fact that when the link capacity changes (and hence the dequeue rate changes), the rate at the senders changes automatically within 1 RTT. As shown in Appendix~\ref{app:deque-vs-enque}, computing $f(t)$ based on the dequeue rate at the router enables \name to track the link capacity much more accurately than using the enqueue rate. 

\name recomputes $f(t)$ on every dequeued packet, using measurements of $cr(t)$ and $\mu(t)$ over a sliding time window of length $T$. Updating the feedback on every packet allows \name to react to link capacity changes more quickly than schemes that use periodic feedback updates (e.g., XCP and RCP).

Packet marking can be done deterministically or probabilistically. To limit burstiness, \name uses the deterministic method shown in Algorithm~\ref{alg:abc}. The variable {\tt token} implements a token bucket that is incremented by $f(t)$ on each outgoing packet (up to a maximum value {\tt tokenLimit}), and decremented when a packet is marked accelerate. To mark a packet accelerate, {\tt token} must exceed 1. This simple method ensures that no more than a fraction $f(t)$ of the packets are marked accelerate. 

%Notice that the router never changes the mark for a packet that was previously marked with brake 

%. If {\tt token} is greater than 1, the packet is marked accelerate and {\tt token} is decremented; otherwise it is marked brake. This simple method ensures that no more than a fraction $f(t)$ of the packets are marked accelerate. 

\begin{algorithm}[t]
\SetAlgoLined
\caption{Packet marking at an \name{} router.}% The exponential decay limits the burstiness of ``accelerate'' signals.}
token $=$ 0\;
\For{each outgoing packet}{
    calculate $f(t)$ using Eq.~(\ref{eq:f})\;
    token = min(token $+ f(t)$, tokenLimit)\;
    \If{packet marked with accelerate}{
        \eIf{token $>$ 1}{
            token = token $-$ 1\;
            mark accelerate\;
        }{
            mark brake\;
        }
    }
}
\label{alg:abc}
\end{algorithm}

\smallskip
\noindent{\bf Multiple bottlenecks:} An \name flow may encounter multiple ABC routers on its path. An example of such a scenario is when two smartphone users communicate over an \name-compliant cellular network. Traffic sent from one user to the other will traverse a cellular uplink and cellular downlink, both of which could be the bottleneck. To support such situations, \name endhosts should send traffic at the smallest of the router-computed target rates along their path.  To achieve this goal, each packet is initially marked accelerate by the sender. \name routers may change a packet marked accelerate to a brake, but not vice versa (see Algorithm~\ref{alg:abc}). This rule guarantees that an \name router can unilaterally reduce the fraction of packets marked accelerate to ensure that its target rate is not exceeded, but it cannot increase this fraction. Hence the fraction of packets marked accelerate will equal the minimum $f(t)$ along the path. 

\subsection{Estimating Link Rate}
In this section we describe, how can \name routers estimate the link capacity for computing the target rate (\S\ref{s:abc-router}). We present a technique for WiFi that leverages the inner workings of the WiFi MAC layer, and we discuss options for cellular networks.
\label{s:linkrate}


\subsubsection{Wi-Fi\\}
\label{s:wifi}
We present how an \name access point router can estimate the link rate in the 802.11n Wi-Fi protocol. We assume that users share a single queue at the access point (AP), which is the dominant queuing strategy for Wi-Fi routers today. The link rate is defined as the aggregate throughput that would be achieved across all users when the AP is backlogged (i.e., not empty). We first describe our solution assuming a single user and then extend it to multiple users.

\textbf{Challenges:} A strawman would be to estimate link rates based on the bitrates of transmitted packets. Unfortunately, this will overestimate the link rate as packet transmission times are governed not only by bitrates, but also by delays for additional tasks (e.g., channel contention) and retransmissions. An alternative approach would be to use the fraction of time that the router queue was backlogged as a proxy for link utilization\cut{and compute link rate as the ratio of current throughput and link utilization}. Unfortunately, the Wi-Fi MAC's packet batching confounds this idea. Wi-Fi routers transmit packets (frames) in batches, a new batch in transmitted only after receiving an ACK for the last batch. Routers may accumulate packets while waiting for an ACK; this queue buildup does not necessarily imply that the link is fully utilized. Thus, accurately measuring link rates on a Wi-Fi 802.11n router requires a detailed consideration of Wi-Fi's packet transmission protocols. 
\cut{The primary challenge lies in handling several protocol-specific properties of the Wi-Fi MAC layer.}

\textbf{Understanding Wi-Fi 802.11 n:} In 802.11n, data frames, also known as MAC Protocol Data Units (MPDUs), are transmitted in batches called A-MPDUs (Aggregated MPDUs). The maximum number of MPDUs that can be included in a single A-MPDU, $M$, is negotiated by each receiver and the router. When a given user is not backlogged, the router might not have enough data to send a full-sized A-MPDU of size $M$, but will instead use an A-MPDU size $x < M$. Upon receiving an A-MPDU, a receiver responds with a single Block ACK. Thus, at a time $t$, given an A-MPDU size of $x$ frames, a frame size of $S$,\footnote{For simplicity, we assume that all frames are of the same size, though our formulas can be generalized in a straightforward manner for varying frame sizes.} and an ACK inter-arrival time (i.e., the time between receptions of consecutive block ACKs) of $T_{IA}(x,t)$, the instantaneous throughput, $cr(t)$, may be estimated as
%that acknowledges each individual MPDU in the A-MPDU.
\begin{equation}
     cr(t) = \frac{x . S}{T_{IA}(x,t)}.
     \label{eq:inst_throughput}
\end{equation}

When the user is backlogged, the instantaneous throughput will be equal to the link capacity. However, if the user is not backlogged and A-MPDUs only include $x < M$ frames, how can the router estimate the link capacity? Our approach calculates $\hat{T}_{IA}(M,t)$, the estimated ACK inter-arrival time if the router could have included $M$ frames in the last A-MPDU (rather than only including the $x$ frames).\cut{that the user had provided).Using $\hat{T}_{IA}(M,t)$,.} Thus, we can estimate the link capacity, $\hat{\mu}(t)$, as
  \begin{align}
    \hat{\mu}(t) = \frac{M .  S}{\hat{T}_{IA}(M,t)}. 
         \label{eq:capacity_backlog}
  \end{align}


 \begin{figure}[t]
     \centering
     \includegraphics[width=\columnwidth]{images/ampdu.pdf}
     \vspace{-8mm}
     \caption{\small {\bf Inter-ACK time vs A-MPDU size ---} Inter-ACK for a given A-MPDU exhibits variation. The solid black line represents the average Inter-ACk time for  given A-MPDU. The slope of the line is $S/R$.}
     \label{fig:ampdu_burst}
     \vspace{-4mm}
\end{figure}

To accurately estimate $\hat{T}_{IA}(M,t)$, we turn to the relationship between A-MPDU size and ACK inter-arrival time. We can break down ACK interval time between transmission time and time spent in performing ``overhead'' tasks, including physically receiving an ACK, contending for the shared channel, and transmitting the physical layer preamble~\cite{ginzburg2007performance}. Each of these overhead tasks is independent of the A-MPDU size; as a result, we refer to the overhead time spent on these tasks using a separate term $h(t)$. If $R$ is the bitrate used for transmission, the router's ACK inter-arrival time is
 \begin{align}
     T_{IA}(x,t) \;&=\; \frac{x . S}{R} + h(t).
     \label{eq:inter_ack}
 \end{align}

\Fig{ampdu_burst} illustrates this independence. There are two key properties to note. First, for a given A-MPDU size, ACK inter-arrival times vary due to overhead tasks~\cite{ginzburg2007performance}. Second, because the overhead time and A-MPDU size are independent (Equation~\ref{eq:inter_ack}), connecting the average values of ACK inter-arrival times across all considered A-MPDU values will produce a line with slope $S/R$. Using this independence, we can estimate the ACK inter-arrival time for a backlogged user as

\vspace{-3mm}
 \begin{align}
    \hat{T_{IA}}(M,t) \;&=\;  \frac{MS}{R} + h(t)\nonumber\\
    \hat{T}_{IA}(M,t) \;&=\; T_{IA}(x,t) + \frac{(M - x) S}{R}.
    \label{eq:inter-ack-time}
 \end{align}
 \vspace{-3mm}

We can then use $\hat{T}_{IA}(M,t)$ to estimate the link capacity with Equation~\ref{eq:capacity_backlog}. This computation occurs for each A-MPDU transmission, and we compute a weighted moving average of link capacity over a sliding window of time $T$. $T$ must be greater than Inter-ACK Time (up to 20 ms in \Fig{ampdu_burst}), we use $T = 40$ ms. Additionally, since \name cannot increase its rate more than twice per RTT, we cap the predicted link rate to twice the current rate. 

\textbf{Multiple users:} When multiple users share the bottleneck router's queue, we compute an aggregate link rate across all users. In particular, we can use Eq. (~\ref{eq:inter-ack-time})~and~(\ref{eq:capacity_backlog}) to compute the link capacity for each A-MPDU transmission. Because the router transmits only one A-MPDU at a time, although users can negotiate different A-MPDU values with the router, link rate calculations can occur in a user-independent way by considering only the size of each A-MPDU transmission.

 \begin{figure}[t]
     \centering
     \includegraphics[width=\columnwidth]{images/prediction.pdf}
     \vspace{-8mm}
     \caption{\small {\bf Wi-Fi Link Rate Prediction ---} \name router link rate predictions for a user that was not backlogged and sent traffic at multiple different rates over 3 distinct Wi-Fi links. Horizontal lines represent the true link capacity, solid lines summarize the \name router's link capacity prediction (each point is an average over 30 seconds of predictions), and the dashed slanted line represents the prediction rate caps. \name's link rate predictions are within 5\% of the ground truth across all sending rates.}
     \label{fig:prediction}
     \vspace{-4mm}
\end{figure}

\textbf{Evaluating link rate estimates:} To evaluate the accuracy of our link rate estimates, we had a single user send traffic through our modified \name router (implementation described below) at multiple different fixed rates (i.e., offered loads) over three distinct Wi-Fi links. \Fig{prediction} summarizes the accuracy of the \name router's link rate estimates. With this method, the \name Wi-Fi router is able to predict link rates within 5\% of the observed link capacities.

\subsubsection{Cellular Networks}
\label{cellular_estimation}
Cellular Networks schedule users from separate queues to ensure inter-user fairness. Each user will observe a different link capacity and queuing delay. As a result, every user should run a separate instance of \name router. Prior work~\cite{3GPP} has shown how to use scheduling information at the cellular base station to calculate per-user link rates. The described method is able to estimate capacity accurately even if a given user is not backlogged.




==> introduction.tex <==
\section{Introduction}
\label{s:introduction}

We propose a new explicit congestion control protocol for network paths with wireless links. Congestion control on such paths is challenging because of the rapid time variations of the link rate. End-to-end schemes must infer the correct window size indirectly from receiver ACK feedback. In principle, active queue management~\cite{codel, pie} (AQM) should help by providing feedback from the bottleneck router, but these schemes often leave the underutilized ~\cite{goyal2017rethinking, sprout}.\cut{end-to-end schemes like Copa~\cite{copa} and Verus~\cite{verus} often outperform them. \pg{Not really.}} The reason is that AQM schemes can respond to reductions in the bottleneck rate, but have no way to signal increases when bandwidth increases~\cite{goyal2017rethinking}.

 % Traditional protocols may respond to reductions in the bottleneck rate using explicit congestion notification (ECN) signals, but are not able to quickly increase their congestion window (rate) when bandwidth increases.

% In principle, explicit congestion control protocols like XCP and RCP should work well in such networks. But how well? This is the first question we answer in this paper. 

By contrast, routers in explicit control protocols like XCP~\cite{xcp} and RCP~\cite{rcp} directly specify a target rate to the sender, signaling both rate increases and decreases. In principle, these schemes could substantially improve performance compared to both traditional protocols~\cite{copa, vegas, bbr, vivace, cubic} and recent algorithms designed for cellular networks~\cite{sprout, verus}. However, they have two limitations, one conceptual and the other practical. First, XCP and RCP are designed for fixed-capacity links; we find that they are sub-optimal on time-varying wireless links. Second, they have proven hard to deploy on the Internet.

%allowing flows to converge to the specified rate quickly. Unlike AQM schemes, they can signal rate increases as well as decreases. We show that explicit protocols could substantially improve performance compared to both traditional protocols~\cite{copa, vegas, bbr, vivace, cubic} and recent algorithms designed for cellular networks~\cite{sprout, verus}. For example, on cellular traces, XCP achieves similar delays with 38\% higher utilization than both Cubic+Codel~\cite{codelID} and Copa~\cite{copa}. Figure~\ref{fig:motivation} illustrates the cause of this performance difference.

%Our goal is to understand whether, and by how much, explicit information can help on wireless paths, and to develop a simple and deployable protocol that works in practice.

%The first contribution of this paper is an evaluation of explicit congestion control protocols compared to other approaches on a variety of emulated wireless network paths. 


%These advantages of schemes like XCP and RCP are of course well-known. But how much better would such schemes perform than simpler-to-deploy alternatives over actual wireless links?


% XCP and RCP are ``clean slate'' protocol designs that have proven hard, if not impossible, to deploy on the Internet. Is it possible to develop a  simpler protocol that achieves the same benefits, but which is deployable? This is the second question we answer.

%Despite their promise, prior explicit protocols like XCP and RCP have proven hard, if not impossible, to deploy on the Internet. Thus we ask: can we design a {\em simple} explicit protocol that can be deployed and used in practice?  

This paper presents the design and evaluation of {\bf Accel-Brake Control} (ABC)~\cite{goyal2017rethinking}, a simple and deployable explicit control protocol targeted for Internet paths with time-varying bottleneck links. 
%4, which builds on concepts previously presented in a position paper~\cite{goyal2017rethinking}. 
In \name{}, wireless routers mark each packet with one bit of feedback corresponding to either {\em accelerate} or {\em brake} based on a measured estimate of the current link rate. Upon receiving this feedback via an ACK from the receiver, the sender either accelerates its transmission by sending {\em two packets} (on accelerate), or decelerates by not sending any packet (on brake). This simple mechanism allows the router to signal a large dynamic range of window size changes: from throttling the window to 0, to doubling the window, all within one RTT.

\name's control algorithm has two unique features that help it perform well on fast-varying links. First, \name routers exploit the ACK-clocking property of a window-based protocol to accurately predict the incoming rate of packets one RTT into the future based on the {\em current dequeue rate of packets} at the router. By contrast, prior work compares the enqueue rate to the link rate to determine the feedback. \name's feedback is more accurate and tracks capacity changes better because it models the enqueue rate in the future. Second, \name adjusts its feedback continuously on a packet-by-packet basis to react immediately to any capacity fluctuations. We conduct a control-theoretic analysis of the algorithm and provide a simple criteria on its parameters that ensures its stability and convergence. 

To ease deployment, we show how \name{} can be implemented by reusing the existing ECN infrastructure. Additionally, we describe how \name can co-exist well with non-\name bottleneck routers running ECN, and share bandwidth fairly with non-\name{} flows traversing a bottleneck \name router.

%\name{} has three key ideas. First, the base station marks  each packet with one bit of feedback corresponding to either {\em accelerate} or {\em brake} using a measured estimate of the current rate for the user and a computed estimate of a desired target rate. Second, upon receiving this feedback via an ACK from the receiver (using the same concept as in ECN), the sender either accelerates its transmission by sending {\em two packets} (on accelerate), or decelerates by not sending any packet (on brake). This simple mechanism achieves a large dynamic rate range, allowing the congestion window to vary from double the current value down to 0 within one RTT.

%The third idea eases deployment. We show how to reuse the existing ECN infrastructure to implement \name{}, and describe how \name can co-exist well with bottleneck routers running ECN (and not \name) and share resources fairly with non-\name{} flows traversing a bottleneck \name router. 

\cut{presenting two deployment options for networks without and with legacy ECN routers. The first case applies to many cellular networks that split TCP connections at the network boundary~\cite{wang2011untold,
  ravindranath2013timecard}; here, we show how to deploy \name{}
without any changes to TCP receivers (\eg running on mobile
phones). In the second case, we show how \name{} can co-exist with
legacy ECN with simple changes to the receiver. }

\cut{ABC addresses three deployment challenges:

\begin{CompactEnumerate}
    \item Protocols like XCP and RCP require major changes to headers, endpoints, and routers. In principle, TCP options provide a way to convey information in the transport layer, but in practice new TCP options are problematic due to middleboxes~\cite{honda2011still} and IPSec encryption~\cite{seo2005security}. \name repurposes the existing explicit congestion notification (ECN) bit to enable wireless routers to signal not only decreases, but also increases to the sender's congestion window, to quickly achieve a desired target rate. \name can be implemented without any receiver modifications and can co-exist with legacy ECN routers. 
    
    %\ma{Co-existence with legacy ECN requires the NS bit. Not sure if this is worth pointing out or with "co-existence with legacy ECN" is an overclaim.} 

\item \name is robust to scenarios where the bottleneck link is not the wireless link but a non-ABC link elsewhere on the path. With increasing wireless link rates, situations where the wireless link is not always the bottleneck do arise. When that happens, ABC ensures that it sends no faster than the bottleneck rate using a simple mechanism: it runs a traditional algorithm like Cubic in parallel and uses its window size as an upper bound on its congestion window, reacting to traditional congestion signals like packet loss or delay.

\item \name can co-exist with non-\name flows sharing the same bottleneck wireless link. Here, the router must allocate only part of the bottleneck rate to ABC, proportional to the number of long-running ABC flows sharing the bottleneck with other long-running non-ABC flows. ABC achieves this by separating \name and non-\name traffic into two queues and scheduling packets from each queue according to dynamic weights. ABC determines these weights by observing the rates of a small number of flows in each queue. Unlike RCP~\cite{rcp}, our method is robust to the presence of short or application-limited flows, and unlike XCP, converges quicker and does not depend on the other long-running flows having a well-known throughput-versus-loss-rate function (e.g., XCP assumes $1/\sqrt{p}$, which means it cannot correctly handle a scheme like Cubic, or a mix of different competing protocols).

\end{CompactEnumerate}

}

%We make two principal contributions. First, we present results showing how well explicit congestion control protocols perform compared to other approaches on various wireless network paths. To obtain these results, we develop a simple and general method to estimate the wireless link's ``target rate''---a parameter used in explicit protocols in conjunction with the current queue occupancy or delay---to guide the sender's actions.  Second, we develop a simple and deployable explicit protocol, called {\bf Accel Brake Control} (ABC), which redefines the existing ECN bit with which the (wireless) bottleneck router can cause the sender to not only decrease, but also increase, its congestion window to quickly achieve a desired target rate.

%The simplicity and economy of mechanism is the most important property of ABC. In addition, we show how ABC tackles two key deployment challenges.
% \begin{enumerate}
%     \item Robustness: if at any point during the transfer, the bottleneck link is not be the wireless link but a non-ABC wired link elsewhere on the path, how can the sender ensure that it sends no faster than the wired bottleneck? It is important in this case to respond to traditional congestion signals like packet loss or delay, as well as to ECN feedback, without being confounded by ABC's use of the same ECN bits.
%     \item Co-existence with non-ABC flows sharing the same bottleneck wireless link. In this case, our goal is to allocate only part of the bottleneck rate to ABC, proportional to the number of long-running ABC flows sharing the bottleneck with other long-running non-ABC flows. 
%     \end{enumerate}

We have implemented \name on a commodity Wi-Fi router running the OpenWRT~\cite{openwrt}. Our implementation reveals another important challenge for implementing explicit protocols on wireless links: how to determine the link rate at a given time? On the surface, this would seem straightforward. However, the task is complicated by the intricacies of the way a modern Wi-Fi MAC schedules and transmits packets (e.g., batch scheduling and block acknowledgements). We develop a method to estimate the link rate that takes into account frame batching and block acknowledgements in Wi-Fi and experimentally demonstrate its high accuracy. Similar techniques can be applied to cellular links~\cite{3GPP}, though the details might differ. For cellular links, our evaluation uses trace-driven network link emulation with Mahimahi~\cite{mahimahi}.

%A final important challenge for implementing explicit protocols on wireless links is how to determine the link rate at a given time? On the surface, this would seem straightforward. However, the task is complicated by the intricacies of the way modern Wi-Fi and cellular base stations schedule and transmits packets (e.g., batch scheduling and block acknowledgements). We develop a method to estimate the link rate in Wi-Fi that takes into account frame batching and block acknowledgements, and we experimentally demonstrate its high accuracy on a commodity Wi-Fi router running the OpenWRT~\cite{openwrt}. We believe similar techniques can be applied to cellular links~\cite{3GPP}, though the details might differ. For cellular links, our evaluation uses trace-driven network link emulation with Mahimahi~\cite{mahimahi}.

%when the link is not fully utilized (e.g., if bandwidth suddenly increases), determining the true link rate is complicated because of MAC layer transmits and acknowledges packets in batches. We cannot simply use the bitrate itself to estimate the actual link rate because of frame retransmissions and MAC delays. We develop a method to estimate the link rate that takes into account frame batching and block acknowledgements in Wi-Fi and experimentally demonstrate its high accuracy. We believe that similar techniques can be applied to cellular links, though the details will likely differ. For cellular links, our evaluation uses trace-driven network link emulation with Mahimahi~\cite{mahimahi}.

We have tested ABC using both our Wi-Fi implementation and trace-driven experiments across a variety of wireless network settings. Our results are:
\begin{CompactEnumerate}
    \item In Wi-Fi settings, compared to Cubic+Codel and Vegas, \name achieves 30-40\% higher throughput for similar delays. Cubic, PCC Vivace-latency and BBR incur 70\%--6$\times$ higher 95$^{th}$ percentile per packet delay, while achieving throughput similar to \name.
    \item XCP achieves similar throughput as \name, but incurs 105\% higher 95$^{th}$ percentile per packet delay. \name outperforms both RCP and VCP, achieving 20\% more utilization on average.
    \item Over cellular traces, \name achieves 38\% higher utilization than schemes designed to reduce delay (Copa, Cubic+Codel, Cubic+PIE) for comparable delays. Cubic, PCC Vivace-latency, and BBR incur 80\%-4$\times$ higher 95$^{th}$ percentile per packet delay, while achieving only 9\% to 18\% higher throughput. Compared to Sprout \name achieves 80\% higher throughput for similar delays. Verus incurs 2$\times$ higher delays than \name.
    \item \name competes fairly with both \name and non-\name flows. Specifically, in scenarios with both \name and non-\name flows, the difference in average throughput of \name and non-\name flows is under 5\%. 
    \item \name bottlenecks can coexist with both \name and non-\name bottlenecks. \name flows achieve high utilization and low queuing delays if the bottleneck router is \name, while switching to Cubic when the bottleneck is a non-\name router.
\end{CompactEnumerate}




==> linkestimate.tex <==
\section{Estimating Link Rate}
\label{s:linkrate}
We describe how \name routers can estimate the link capacity for computing the target rate (\S\ref{s:abc-router}). We present a technique for Wi-Fi that leverages the inner workings of the Wi-Fi MAC layer, and we discuss options for cellular networks. 
%\ma{I'd call this section Wi-Fi implementation and move the cellular network stuff to the discussion section}

\subsection{Wi-Fi}
\label{s:Wi-Fi}
We describe how an 802.11n access point (AP) can estimate the average link rate. This method works for any work-conserving scheduler, whether or not the users' packets share a queue. {\color{blue} Assuming, none of the users run of packets at the AP, }the link rate is defined as the ratio $S/T$, where $S$ is the number of bits to be transmitted in sequence over the link and $T$ is the time taken to do so, starting from when the first bit is ready to be sent on the link (any delay in sending the first bit due to channel contention or retransmissions of previous frames is included in $T$)\footnote{{\color{blue} We only present a technique for 802.11 n, but the ideas could be extended to 802.11 ac. In this case, we anticipate that the AP will do a separate link rate calculation for each of the spatial channels.}}. 


\smallskip
\noindent{\it Challenges:} A strawman would be to estimate the link rate using the physical layer bit rate selected for each transmission, which would depend on the modulation and channel code used for the transmission. Unfortunately, this method will overestimate the link rate as packet transmission times are governed not only by bitrates, but also by delays for additional tasks (e.g., channel contention and retransmissions~\cite{samplerate}). An alternative approach would be to use the fraction of time that the router queue was backlogged as a proxy for link utilization\cut{and compute link rate as the ratio of current throughput and link utilization}. Unfortunately, the Wi-Fi MAC's packet batching confounds this approach. Wi-Fi routers transmit packets (frames) in batches; a new batch is transmitted only after receiving an ACK for the last batch. The AP may accumulate packets while waiting for a link-layer ACK; this queue buildup does not necessarily imply that the link is fully utilized. Thus, accurately measuring link rates requires a detailed consideration of Wi-Fi's packet transmission protocols. 
\cut{The primary challenge lies in handling several protocol-specific properties of the Wi-Fi MAC layer.}

\smallskip
\noindent{\bf Understanding batching:} In 802.11n, data frames, also known as MAC Protocol Data Units (MPDUs), are transmitted in batches called A-MPDUs (Aggregated MPDUs). The maximum number of frames that can be included in a single batch, $M$, is negotiated by each receiver and the router. When a given user is not backlogged, the router might not have enough data to send a full-sized batch of $M$ frames, but will instead use a smaller batch of size $b < M$. Upon receiving a batch, the receiver responds with a single Block ACK. Thus, at a time $t$, given a batch size of $b$ frames, a frame size of $S$ bits,\footnote{For simplicity, we assume that all frames are of the same size, though our formulas can be generalized easily for varying frame sizes.} and an ACK inter-arrival time (i.e., the time between receptions of consecutive block ACKs) of $T_{IA}(b,t)$, the current dequeue rate, $cr(t)$, may be estimated as
%\noindent{\bf Understanding batching:} In 802.11n, data frames, also known as MAC Protocol Data Units (MPDUs), are transmitted in batches called A-MPDUs (Aggregated MPDUs). The maximum number of frames that can be included in a single batch, $M$, is negotiated by each receiver and the router. \pg{When a given user is not backlogged, i.e. the router does not have enough data to send a full-sized batch of $M$ frames, the router will instead use a smaller batch of size $b < M$.} Upon receiving a batch, the receiver responds with a single Block ACK. Thus, at a time $t$, given a batch size of $b$ frames, a frame size of $S$ bits,\footnote{For simplicity, we assume that all frames are of the same size, though our formulas can be generalized in a straightforward manner for varying frame sizes.} and an ACK inter-arrival time (i.e., the time between receptions of consecutive block ACKs) of $T_{IA}(b,t)$, the current dequeue rate, $cr(t)$, may be estimated as
%that acknowledges each individual MPDU in the A-MPDU.
\vspace{-2mm}
\begin{equation}
     cr(t) = \frac{b . S}{T_{IA}(b,t)}.
     \label{eq:inst_throughput}
\end{equation}
\vspace{-4mm}

When the user is backlogged and $b=M$, then $cr(t)$ above will be equal to the link capacity. However, if the user is not backlogged and $b < M$, how can the AP estimate the link capacity? Our approach calculates $\hat{T}_{IA}(M,t)$, the estimated ACK inter-arrival time {\em if the user was backlogged and had sent $M$ frames in the last batch.}
%(rather than only including the $x$ frames).\cut{that the user had provided).Using $\hat{T}_{IA}(M,t)$,.} 

We estimate the link capacity, $\hat{\mu}(t)$, as
\vspace{-2mm}
  \begin{align}
    \hat{\mu}(t) = \frac{M .  S}{\hat{T}_{IA}(M,t)}. 
         \label{eq:capacity_backlog}
  \end{align}
\vspace{-4mm}

 \begin{figure}[t]
     \centering
     \includegraphics[width=0.9\columnwidth]{images/ampdu.pdf}
     \vspace{-4mm}
     \caption{\small {\bf Inter-ACK time v. batch (A-MPDU) size ---} Inter-ACK times for a given batch size exhibits variation. The solid black line represents the average Inter-ACK time. The slope of the line is $S/R$, where $S$ is the frame size in bits and $R$ is the link rate in bits per second.}
     \label{fig:ampdu_burst}
     \vspace{-3mm}
\end{figure}

To accurately estimate $\hat{T}_{IA}(M,t)$, we turn to the relationship between the batch size and ACK inter-arrival time. We can decompose the ACK interval time into the batch transmission time and ``overhead'' time, the latter including physically receiving an ACK, contending for the shared channel, and transmitting the physical layer preamble~\cite{ginzburg2007performance}. Each of these overhead components is independent of the batch size, modeled as $h(t)$. If $R$ is the bitrate used for transmission,\footnote{Different users can have different transmission rates.} the router's ACK inter-arrival time is
\vspace{-1mm}
 \begin{align}
     T_{IA}(b,t) \;&=\; \frac{b . S}{R} + h(t).
     \label{eq:inter_ack}
 \end{align}
 \vspace{-4mm}

\Fig{ampdu_burst} illustrates this relationship empirically. There are two key properties to note. First, for a given batch size, the ACK inter-arrival times vary due to overhead tasks. Second, because the overhead time and batch size are independent, connecting the average values of ACK inter-arrival times across all considered batch sizes will produce a line with slope $S/R$. Using this property, we can estimate the ACK inter-arrival time for a backlogged user as

\vspace{-6mm}
 \begin{align*}
    \hat{T_{IA}}(M,t) \;&=\;  \frac{MS}{R} + h(t)\nonumber\\
\end{align*}
\vspace{-15mm}
\begin{align}
    \hat{T}_{IA}(M,t) \;&=\; T_{IA}(b,t) + \frac{(M - b) S}{R}.
    \label{eq:inter-ack-time}
 \end{align}
 \vspace{-6mm}

We can then use $\hat{T}_{IA}(M,t)$ to estimate the link capacity with Equation~\ref{eq:capacity_backlog}. This computation is performed for each batch transmission when the batch ACK arrives, and passed through a weighted moving average filter over a sliding window of time $T$ to estimate the smoothed time-varying link rate. $T$ must be greater than the inter-ACK time (up to 20 ms in \Fig{ampdu_burst}); we use $T = 40$ ms. Because \name cannot exceed a rate-doubling per RTT, we cap the predicted link rate to double the current rate (dashed slanted line in \Fig{ampdu_burst}). 

%\pg{Note that, the method presented here estimates the aggregate link capacity on the router. \name's additive-increase will ensure fairness among multiple user sharing the Wi-Fi link.}
%\noindent{\bf Multiple users:} When multiple users share the bottleneck router's queue, we compute an aggregate link rate across all users. In particular, we can use Eq. (~\ref{eq:inter-ack-time})~and~(\ref{eq:capacity_backlog}) to compute the link capacity for each A-MPDU transmission. Because the router transmits only one A-MPDU at a time, although users can negotiate different A-MPDU values with the router, link rate calculations can occur in a user-independent way by considering only the size of each A-MPDU transmission.

 \begin{figure}[t]
     \centering
     \includegraphics[width=0.9\columnwidth]{images/prediction.pdf}
     \vspace{-3mm}
     \caption{\small {\bf Wi-Fi Link Rate Prediction ---} \name router link rate predictions for a user that was not backlogged and sent traffic at multiple different rates over three different Wi-Fi links. Horizontal lines represent the true link capacity, solid lines summarize the \name router's link capacity prediction (each point is an average over 30 seconds of predictions), and the dashed slanted line represents the prediction rate caps. \name's link rate predictions are within 5\% of the ground truth across all sending rates.}
     \label{fig:prediction}
     \vspace{-5mm}
\end{figure}

%\smallskip
\smallskip
\noindent{\bf Evaluation:} To evaluate the accuracy of our link rate estimates, we transmit data to a single client through our modified \name router (\Sec{prototype implementation}) at multiple different rates over three Wi-Fi links (with different modulation and coding schemes). \Fig{prediction} summarizes the accuracy of the \name router's link rate estimates. With this method, the \name Wi-Fi router is able to predict link rates within 5\% of the true link capacities.

\subsection{Cellular Networks}
\label{cellular_estimation}

Cellular networks schedule users from separate queues to ensure inter-user fairness. Each user will observe a different link capacity and queuing delay. As a result, every user requires a separate target rate calculation at the \name router. The 3GPP cellular standard~\cite{3GPP} (page 13) describes how scheduling information at the cellular base station can be used to calculate per-user link rates. This method is able to estimate capacity accurately even if a given user is not backlogged at the base station, a key property for the target rate estimation in Eq.~(\ref{eq:abctargetrule}).

==> motivation_old.tex <==
\section{Motivation}
\label{s:related}

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/motivation_cubic.pdf}
        \caption{Cubic}
        \label{fig:motivation:cubic}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/motivation_codel.pdf}
        \caption{Cubic+Codel}
        \label{fig:motivation:codel}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/motivation_xcp.pdf}
        \caption{XCP}
        \label{fig:motivation:xcp}
    \end{subfigure}
    \caption{\small {\bf Performance on a emulated cellular trace ---} The dashed blue in the top graph represents link capacity, the solid orange line represents the achieved throughput. Cubic has high utilization but has very high delays (up to 1500 milliseconds). Cubic+Codel reduces queuing delays by 1 to 2 orders of magnitude, but leaves the link underutilized. XCP achieves close to 100\% utilization while maintaining low queuing delays (similar to that of Cubic+Codel). Please note, the Y-axis for queuing delay has a log scale.}
    \label{fig:motivation}
\end{figure*}

Traditional end-to-end protocols like TCP Cubic~\cite{cubic} and NewReno~\cite{Jacobson88,newreno} are unable to track time-varying wireless link capacities well. To achieve high throughput for these protocols, wireless/cellular networks often use deep buffers, which leads to significant bufferbloat.

Bufferbloat can be reduced using AQM schemes like CoDel~\cite{codel} or PIE~\cite{pie}. Although these schemes are able to achieve low packet delays, they suffer from under-utilization because of the conservative increase rules in Cubic and NewReno---when link capacity increases, the sender is unable to increase its rates quickly enough. Perhaps for this reason, we see little evidence of cellular networks using AQM schemes.

Without AQM, Cubic and NewReno rely only on packet drops to infer congestion, but (especially with deep packet buffers) this signal is too infrequent for efficient adaptation to changing link conditions. Recent end-to-end proposals like Copa~\cite{copa} , BBR~\cite{bbr} and PCC Vivace-latency~\cite{vivace} overcome the spareness of packet drops by using information about the RTT and the send/receive rate, and combining this information with prediction strategies to deduce available capacity. There also have been end to end proposals aimed at reducing delays in cellular networks, Sprout~\cite{sprout} and Verus~\cite{verus}.

These schemes face a trade-off between utilization (throughput) and packet delay because estimating the available capacity by end-to-end means requires some queue build up. These schemes have no information about available capacity when the queue is empty; during such periods, the best they can do is to increase the rate in ``blind'' fashion. This approach is problematic in networks with a large dynamic range of rates: if the increase is slow, throughput is low, but making the increase too fast inevitably causes overshoots and large queuing delays. Thus, we conclude that, end-to-end schemes will find it difficult to track the available capacity accurately. Router assistance using methods deployed at the base station (or the mobile device's network layer) are therefore important to consider.  

A natural solution ...\pg{TODO: Hari}


\todo{summary
explicit schemes outperform on time varying link
however they haven't seen deployment
cause challenges:
bullet
bullet
bullet
we describe our implementation next which solves challenges while maintaining benefits of other schemes
}


==> practical_challenges.tex <==
\section{Implementation Challenges}
\label{s:practical_challenges}
This section discusses two challenges for implementing and deploying \name in practice. First, we describe how we can repurpose ECN~\cite{ecn-rfc} to signal accel-brake marks. Second, how can \name routers estimate the link capacity for computing the target rate (\S\ref{s:abc-router}). We present a technique for WiFi that leverages the inner workings of the WiFi MAC layer, and we discuss options for cellular networks. Finally, we describe our prototype \name implementation.

\subsection{Deployment with ECN}
\label{ss:deployment}

%In this section, we describe how ECN can be repurposed to signal accel-brake marks. 
We show how we can repurpose ECN for \name feedback, without compromising the \name sender's ability to infer congestion based on ECN markings from non-\name routers. This distinction between feedback from \name and non-\name routers is critical for coexistence with non-\name bottleneck (\S\ref{s:multiple-bottleneck}). We start with an overview of standard ECN, and then present our practical deployment solution. 

\textbf{ECN Overview:} IP packets have two ECN-related bits: ECT and CE. These two bits are traditionally interpreted as follows:
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & ECN-Capable Transport ECT(1)\\
 1 & 0 & ECN-Capable Transport ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
Routers interpret both (01) and (10) to indicate that a connection is ECN capable, and routers change those bits to (11) to mark a packet with ECN. Upon receiving an ECN mark (11), a receiver sets the sets the {\em ECN Echo (ECE)} flag to signal congestion to the sender.

%, a receiver sets the {\em ECN Echo (ECE)} flag in {\em all} subsequent ACKs until it receives a {\em Congestion Window Reduced (CWR)} notification from the sender, \ie a packet with the CWR flag in the TCP header set to 1. Thus receivers echo ECN marks for a full round-trip worth of ACKs.

\textbf{Deployment:} \name reinterprets the ECT and CE ECN bits as follow:

%\name can coexist with non-\name  routers (using ECN for signalling congestion) by reinterpreting the ECT and CE ECN bits as follow:
\begin{center}
\begin{tabular}{ c c c }
 ECT & CE & Interpretation \\ 
 0 & 0 & Non ECN-Capable Transport\\  
 0 & 1 & \textit{accelerate} ECT(1)\\
 1 & 0 & \textit{brake} ECT(0)\\  
 1 & 1 & ECN set 
\end{tabular}
\end{center}
\name senders can mark accelerates using (01), and \name routers can signal brakes by flipping the bits to (10). Both (01) and (10) equivalently indicate ECN capable transport to legacy routers, which can continue to use (11) to signal congestion.

With this design, receivers must be able to convey both standard ECN signals and accelerates/brakes for \name. ECN feedback can be signaled using the ECE flag. For \name feedback, we repurpose the NS (nonce sum) bit, which was originally proposed to ensure ECN feedback integrity~\cite{nonce} but has been reclassified as historic~\cite{accurate-ecn} due to lack of deployment. Thus, our deployment solution only requires simple modifications to TCP receivers.


\textbf{Deployment in Cellular Networks:} Cellular networks commonly split TCP connections and deploy proxy at the edge~\cite{wang2011untold,ravindranath2013timecard}. In such a network, it is unlikely that any non-\name router will act as the bottleneck and interfere with the accel-brake markings from the \name router. In this case where non-\name routers do not use ECN, deploying \name is relatively straightforward and doesn't require any receiver modifications. \name senders can simply use either (01) or (10) ECN markings to signal an accelerate, and routers can use (11) to indicate a brake.  The unmodified receiver can echo this feedback using the ECE flag. The proxy can be modified to run custom \name senders, and the base station can be modified to act as a \name router.

%However, a challenge with such deployment is that ECN receivers, by default, will echo an ECN bit in all ACKs in an RTT (i.e., until they receive a CWR from the sender). An \name sender that responds to all marked ACKs will incorrectly be throttled. To ensure that the receiver conveys accelerate/brake signals accurately, the sender sets the CWR flag on {\em every} packet. This ensures that the receiver echoes a brake exactly once (instead of for a full RTT).

%We note that any internal encryption used by cellular network providers does not hinder a \name{} router's ability to modify ECN bits. The reason is that the \name{} router is typically positioned in a place where any form of in-network encryption is removed (e.g., at an LTE eNodeB).

%\textbf{Security:} It is possible for a malicious router to convert a brake to an accelerate, causing congestion at other routers on the path. However, an \name sender can easily detect this by periodically transmitting packets that are marked with brake; if any of these packets return with accelerate, there exist malicious entities on the path.

%\pg{Should we talk about CWR? Should we talk about our linux implementation here? We used pluggable TCP API, to implement \name senders.}
\subsection{Estimating Link Rate}
\label{s:linkrate}


\subsubsection{Wi-Fi\\}
\label{s:wifi}
We present how an \name access point router can estimate the link rate in the 802.11n Wi-Fi protocol. We assume that users share a single queue at the access point (AP), which is the dominant queuing strategy for Wi-Fi routers today. The link rate is defined as the aggregate throughput that would be achieved across all users when the AP is backlogged (i.e., not empty). We first describe our solution assuming a single user and then extend it to multiple users.

\textbf{Challenges:} A strawman would be to estimate link rates based on the bitrates of transmitted packets. Unfortunately, this will overestimate the link rate as packet transmission times are governed not only by bitrates, but also by delays for additional tasks (e.g., channel contention) and retransmissions. An alternative approach would be to use the fraction of time that the router queue was backlogged as a proxy for link utilization\cut{and compute link rate as the ratio of current throughput and link utilization}. Unfortunately, the Wi-Fi MAC's packet batching confounds this idea. Wi-Fi routers transmit packets (frames) in batches, a new batch in transmitted only after receiving an ACK for the last batch. Routers may accumulate packets while waiting for an ACK; this queue buildup does not necessarily imply that the link is fully utilized. Thus, accurately measuring link rates on a Wi-Fi 802.11n router requires a detailed consideration of Wi-Fi's packet transmission protocols. 
\cut{The primary challenge lies in handling several protocol-specific properties of the Wi-Fi MAC layer.}
%, and only support a single outstanding batch; subsequent batches cannot be transmitted until an ACK (acknowledging all packets in a batch) has been received.

\textbf{Understanding Wi-Fi 802.11 n:} In 802.11n, data frames, also known as MAC Protocol Data Units (MPDUs), are transmitted in batches called A-MPDUs (Aggregated MPDUs). The maximum number of MPDUs that can be included in a single A-MPDU, $M$, is negotiated by each receiver and the router. When a given user is not backlogged, the router might not have enough data to send a full-sized A-MPDU of size $M$, but will instead use an A-MPDU size $x < M$. Upon receiving an A-MPDU, a receiver responds with a single Block ACK. Thus, at a time $t$, given an A-MPDU size of $x$ frames, a frame size of $S$,\footnote{For simplicity, we assume that all frames are of the same size, though our formulas can be generalized in a straightforward manner for varying frame sizes.} and an ACK inter-arrival time (i.e., the time between receptions of consecutive block ACKs) of $T_{IA}(x,t)$, the instantaneous throughput, $cr(t)$, may be estimated as
%that acknowledges each individual MPDU in the A-MPDU.
\begin{equation}
     cr(t) = \frac{x . S}{T_{IA}(x,t)}.
     \label{eq:inst_throughput}
\end{equation}

%We can further break down the duration that routers spend between block ACKs.Part of this time is spent performing ``overhead'' tasks including physically receiving an ACK, contending for the shared channel, and transmitting the physical layer preamble~\cite{ginzburg2007performance}. Each of these overhead tasks is independent of the A-MPDU size; as a result, we refer to the overhead time spent on these tasks using a separate term $h(t)$. If $R$ is the bitrate used for transmission, the router's ACK inter-arrival time can be given by
%\begin{align}
%     T_{IA}(x,t) \;&=\; \frac{x . S}{R} + h(t).
%     \label{eq:inter_ack}
%\end{align}

% When the user is backlogged, the router will transmit A-MPDUs of the maximum size (i.e., $M$ frames), and the instantaneous throughput (Eq. (~\ref{eq:inst_throughput})) will be equal to the link capacity. However, if the user is not backlogged and A-MPDUs only include $x < M$ frames, how can the router estimate the link capacity? Our approach is to calculate $\hat{T}_{IA}(M,t)$, estimated ACK inter-arrival time if the router could have included $M$ frames in the last A-MPDU (rather than only including the $x$ frames that the user had provided). Using $\hat{T}_{IA}(M,t)$, we can estimate the link capacity as
When the user is backlogged, the instantaneous throughput will be equal to the link capacity. However, if the user is not backlogged and A-MPDUs only include $x < M$ frames, how can the router estimate the link capacity? Our approach calculates $\hat{T}_{IA}(M,t)$, the estimated ACK inter-arrival time if the router could have included $M$ frames in the last A-MPDU (rather than only including the $x$ frames).\cut{that the user had provided).Using $\hat{T}_{IA}(M,t)$,.} Thus, we can estimate the link capacity, $\hat{\mu}(t)$, as
  \begin{align}
    \hat{\mu}(t) = \frac{M .  S}{\hat{T}_{IA}(M,t)}. 
         \label{eq:capacity_backlog}
  \end{align}


 \begin{figure}[t]
     \centering
     \includegraphics[width=\columnwidth]{images/ampdu.pdf}
     \vspace{-8mm}
     \caption{\small {\bf Inter-ACK time vs A-MPDU size ---} Inter-ACK for a given A-MPDU exhibits variation. The solid black line represents the average Inter-ACk time for  given A-MPDU. The slope of the line is $S/R$.}
     \label{fig:ampdu_burst}
     \vspace{-4mm}
\end{figure}

To accurately estimate $\hat{T}_{IA}(M,t)$, we turn to the relationship between A-MPDU size and ACK inter-arrival time. We can break down ACK interval time between transmission time and time spent in performing ``overhead'' tasks, including physically receiving an ACK, contending for the shared channel, and transmitting the physical layer preamble~\cite{ginzburg2007performance}. Each of these overhead tasks is independent of the A-MPDU size; as a result, we refer to the overhead time spent on these tasks using a separate term $h(t)$. If $R$ is the bitrate used for transmission, the router's ACK inter-arrival time is
 \begin{align}
     T_{IA}(x,t) \;&=\; \frac{x . S}{R} + h(t).
     \label{eq:inter_ack}
 \end{align}

\Fig{ampdu_burst} illustrates this independence. There are two key properties to note. First, for a given A-MPDU size, ACK inter-arrival times vary due to overhead tasks~\cite{ginzburg2007performance}. Second, because the overhead time and A-MPDU size are independent (Equation~\ref{eq:inter_ack}), connecting the average values of ACK inter-arrival times across all considered A-MPDU values will produce a line with slope $S/R$. Using this independence, we can estimate the ACK inter-arrival time for a backlogged user as


%\Fig{ampdu_burst} illustrates this relationship for a sender who transmits packets below the average Wi-Fi link capacity. There are two key properties to note. First, for a given A-MPDU size, ACK inter-arrival times vary due to overhead tasks~\cite{ginzburg2007performance}. Second, because the overhead time and A-MPDU size are independent (Equation~\ref{eq:inter_ack}), connecting the average values of ACK inter-arrival times across all considered A-MPDU values will produce a line with slope $S/R$. Using this independence, we can use Equation~\ref{eq:inter_ack} to estimate the ACK inter-arrival time for a backlogged user as
\vspace{-3mm}
 \begin{align}
    \hat{T_{IA}}(M,t) \;&=\;  \frac{MS}{R} + h(t)\nonumber\\
    \hat{T}_{IA}(M,t) \;&=\; T_{IA}(x,t) + \frac{(M - x) S}{R}.
    \label{eq:inter-ack-time}
 \end{align}
 \vspace{-3mm}

We can then use $\hat{T}_{IA}(M,t)$ to estimate the link capacity with Equation~\ref{eq:capacity_backlog}. This computation occurs for each A-MPDU transmission, and we compute a weighted moving average of link capacity over a sliding window of time $T$. $T$ must be greater than Inter-ACK Time (up to 20 ms in \Fig{ampdu_burst}), we use $T = 40$ ms. Additionally, since \name cannot increase its rate more than twice per RTT, we cap the predicted link rate to twice the current rate. 
%This equation ensures that $T_{IA}(x,t) \leq \hat{T_{IA}}(M,t)$. Additionally, since \name cannot set a target rate to be greater than twice the current rate, we cap the predicted link rate with $T_{IA}(x,t) \leq \hat{T}_{IA}(M,t) \leq 2 . T_{IA}(x,t)$. We can then use these estimates of ACK inter-arrival times to estimate link capacity for a backlogged user with Equation~\ref{eq:capacity_backlog}. This computation occurs for each A-MPDU transmission, and we compute a weighted moving average of link capacity using these values; our implementation uses a sliding time window of 40 ms.

%This equation ensures that $T_{IA}(x,t) \leq \hat{T_{IA}}(M,t)$. Additionally, since \name cannot set a target rate to be greater than twice the current rate, we cap the predicted link rate with $T_{IA}(x,t) \leq \hat{T}_{IA}(M,t) \leq 2 . T_{IA}(x,t)$. We can then use these estimates of ACK inter-arrival times to estimate link capacity for a backlogged user with Equation~\ref{eq:capacity_backlog}. This computation occurs for each A-MPDU transmission, and we compute a weighted moving average of link capacity using these values; our implementation uses a sliding time window of 40 ms.

\textbf{Multiple users:} When multiple users share the bottleneck router's queue, we compute an aggregate link rate across all users. In particular, we can use Eq. (~\ref{eq:inter-ack-time})~and~(\ref{eq:capacity_backlog}) to compute the link capacity for each A-MPDU transmission. Because the router transmits only one A-MPDU at a time, although users can negotiate different A-MPDU values with the router, link rate calculations can occur in a user-independent way by considering only the size of each A-MPDU transmission.

 \begin{figure}[t]
     \centering
     \includegraphics[width=\columnwidth]{images/prediction.pdf}
     \vspace{-8mm}
     \caption{\small {\bf Wi-Fi Link Rate Prediction ---} \name router link rate predictions for a user that was not backlogged and sent traffic at multiple different rates over 3 distinct Wi-Fi links. Horizontal lines represent the true link capacity, solid lines summarize the \name router's link capacity prediction (each point is an average over 30 seconds of predictions), and the dashed slanted line represents the prediction rate caps. \name's link rate predictions are within 5\% of the ground truth across all sending rates.}
     \label{fig:prediction}
     \vspace{-4mm}
\end{figure}

\textbf{Evaluating link rate estimates:} To evaluate the accuracy of our link rate estimates, we had a single user send traffic through our modified \name router (implementation described below) at multiple different fixed rates (i.e., offered loads) over three distinct Wi-Fi links. \Fig{prediction} summarizes the accuracy of the \name router's link rate estimates. With this method, the \name Wi-Fi router is able to predict link rates within 5\% of the observed link capacities.

\subsubsection{Cellular Networks}
\label{cellular_estimation}
Cellular Networks schedule users from separate queues to ensure inter-user fairness. Each user will observe a different link capacity and queuing delay. As a result, every user should run a separate instance of \name router. Prior work~\cite{3GPP} has shown how to use scheduling information at the cellular base station to calculate per-user link rates. The described method is able to estimate capacity accurately even if a given user is not backlogged.

\subsection{Prototype Implementation}
\label{s:prototype implementation}
\noindent {\bf \name transport:} We implemented \name endpoints in Linux as kernel modules using the pluggable TCP API. 

\noindent{\bf \name router:} We implemented \name as a Linux queuing discipline (qdisc) kernel module using OpenWrt, an open source operating system for embedded networked devices~\cite{openwrt}. We used a NETGEAR WNDR 3800 router configured to 802.11n. However, we note that our implementation is portable as OpenWrt is supported on numerous other commodity Wi-Fi routers.

%An \name router must be able to estimate link capacities, compute target rates, and mark packets as accelerates or brakes. 
\name's WiFi link rate prediction strategy exploits the inner workings of the MAC 802.11n protocol, and thus requires fine-grained values at this layer. In particular, the \name qdisc must know A-MPDU sizes, Block ACK receive times, and packet transmission bitrates. Unfortunately, these values are not natively exposed to Linux router qdiscs, and instead are only available at the network driver. To bridge this gap, we modified the router to log the relevant MAC layer data in the cross-layer socket buffer data structure (skb) that it already maintains per packet. 

%Each time a Block ACK is received, the driver frees the memory which houses the socket buffer for each ACKed packet. We use Linux tracepoints to monitor all such events, and extract the necessary MAC-layer data for \name's link rate estimation.

%An alternative design choice would be to estimate link rates directly in the network driver because MAC-layer data is readily available. However, we chose to implement \name as a qdisc for increased portability and ease of use (i.e., enabling or disabling qdiscs is straightforward using tools like \texttt{tc}). 

==> wifi.tex <==
\section{WiFi Implementation}
\label{s:wifi}

In this section, we describe our implementation of \name on a WiFi router. We implemented \name as a queuing discipline kernel module in Linux atop OpenWrt, a linux operating system targeted for embedded systems.  OpenWrt build system allows users to create firmware for a number of commodity WiFi routers, we use NETGEAR WNDR 3800 (with ath9k driver) in MAC 802.11 n for our experiments.

\subsection{Link Rate Calculation}
We now describe the link rate ($\mu$) calculation for WiFi downlink. Assuming users share the bottleneck queue, the link rate is defined as aggregate throughput achieved by users when the link is backlogged. For simplicity, we first describe our solution assuming one user and then expand it to include multiple users. 

If the link is backlogged (i.e. it has queue build up), then the current dequeue rate can be used as an estimate of the link rate. For \name to achieve high performance, the router must able to calculate the link rate even when the link is not backlogged.

In MAC 802.11 n, frames (MAC Protocol Data Unit [MPDU]) are sent in a batch in the form of an A-MPDU (Aggregated MPDU). On receiving an A-MPDU, the receiver sends a selective Block-ACK acknowledging individual MPDU's in the A-MPDU. At time $t$, given a A-MPDU of $x$ frames, frame size $S$ and inter-ACK time of $T_{IA}(x,t)$ (time between the last and current block-ACK), the instantaneous throughput can be given by, $cr(t)$ =($x . S$)/$T_{IA}(x,t)$. 
 
 If $R$ is the physical data rate (bit rate) used for transmission of an A-MPDU of size $x$ frames, then $T_{IA}(x,t)$ can be given by sum of transmission time and over head time ($O(t)$).
 
 \begin{align}
     T_{IA}(x,t) \;&=\; \frac{x . S}{R} + 0(t)
 \end{align}
 
Th over head time includes DIFS (distributed intern frame space), time spent in receiving an ACK, time spent in contending for the channel, time spent in sending a common physical layer preamble, etc. \cite{ginzburg2007performance}. Since none of these durations depend on the A-MPDU size, we use $O(t)$ notation to show independence with A-MPDU size.
  
 \begin{figure}[tbh]
     \centering
     \includegraphics[width=\columnwidth]{images/ampdu.pdf}
     \caption{\small {\bf Inter-ACK time vs A-MPDU size ---} Inter-ACK for a given A-MPDU exhibits variation.}
     \label{fig:ampdu_burst}
\end{figure}
 
 If the link is backlogged, then the A-MPDU size $x$ will be equal to the maximum A-MPDU size $M$. Maximum A-MPDU size is negotiated by the receiver (user) and router, and might be different for different users. If the user is not backlogged, then $x$ will be lesser than $M$. To calculate link rate we estimate $\hat{T}_{IA}(M,t)$, the inter-ACK time if the user was backlogged and had sent a maximum sized A-MPDU. The link rate can then be given by,  $\hat{\mu}$ = ($M . S$)/$\hat{T}_{IA}(M,t)$. 
 
 Figure~\ref{fig:ampdu_burst} shows the relationship between A-MPDU size and burst time. We make two observations. First, for a given A-MPDU size, $x$, there is a spread in the inter-ACK time. This spread is the result of variation in overhead time arising from contention with other devices sharing the channel with \name router. Second, the line formed average of inter-ACK time for a given $x$, is $S/R$, implying over head time is independent of A-MPDU size. We use this independence to estimate $\hat{T}_{IA}(M,t)$. Given an A-MPDU of size x, we can give  $\hat{T}_{IA}(M,t)$ by the following formulae
 
 \begin{align}
    \hat{T_{IA}}(M,t) \;&=\;  \frac{M . S}{R} + 0(t)\nonumber\\
    \hat{T}_{IA}(M,t) \;&=\; T_{IA}(x,t) + \frac{(M - x) . S}{R}
    \label{eq:inter-ack-time}
 \end{align}
 
 The equation above ensures that $T_{IA}(x,t) \leq \hat{T_{IA}}(M,t) $. Since \name cannot set target rate more than twice the current rate, we cap the predicted link rate to twice the current rate. This implies, $T_{IA}(x,t) \leq \hat{T}_{IA}(M,t) \leq 2 . T_{IA}(x,t)$
 
 Figure~\ref{fig:prediction} shows average rate predicted by \name, on 3 different WiFi links with 1 user, at different sending rates (offered load). The horizontal line represents the maximum throughput achievable on each link, calculated as average throughput achieved by a backlogged user.  The dashed line passing through the origin has a slope of 2 and represents the prediction rate cap at any given offered load. \name predicts the link rate within 5\% of the average link rate values.

 \begin{figure}[tbh]
     \centering
     \includegraphics[width=\columnwidth]{images/prediction.pdf}
     \caption{\small {\bf Link Rate Prediction ---} \name router predicts the link rate withing 5\% of ground truth across all sending rates.}
     \label{fig:prediction}
\end{figure}

\textbf{Multiple Users:}
In case of multiple users, similar to single user setting, for each A-MPDU transmission, we use the Equation~\ref{eq:inter-ack-time} to estimate $\hat{T}_{IA}(M,t)$. A-MPDU for different users can have different bit rate, $R$ and maximum A-MPDU size, $M$. \name calculates an aggregate the current dequeue rate and link rate for all the users, by averaging $x$, $T_{IA}(x,t)$ and $\hat{T}_{IA}(M,t)$ over a window of time (40ms in our WiFi implementation).

\subsection{Implementation in the Linux Kernel}
 %\todo{Anup: Please Review this @Prateesh.}
 %Like any other network assisted explicit congestion control scheme, the router has to provide feedback to the sender regarding the current status of the link. In ABC, the middle box router marks a fraction of packets with ECN markings in the IP header which are echoed back in the TCP header by the receiver and sent to the sender. The sender interprets this fraction to do multiplicative increase or decrease (MIMD). 
 
 The router uses the link rate estimation above to calculate a target rate and mark accelerate/brakes on packets. This marking is done in a dedicated \name queuing discipline which is an abstraction exposed by the Linux kernel, allowing a programmer to provide routines to alter the scheduling of the packets in transit, filter / classify them, mark ECN or drop packets. 
 
 To ease independent development of the various layers of protocols, Linux kernel follows a philosophy in which each layer does whatever processing the layer is responsible for and then forwards the packet to the lower layers, thereafter there is no communication between the layers regarding that packet, and it becomes the responsibility of the lower layer to forward the packet to the appropriate paths thereafter.
 
 This gap in communication, however, lead to an unfortunate situation during implementation of ABC. One of the major components of ABC is the link rate calculation module which, in our implementation, exploits the inner workings of the MAC 802.11n protocol. For this, ABC requires the knowledge of the size of the MPDU aggregate($x$), the time a block-Acknowledgment ws received, along with the bit-rate ($R$) used to send the A-MPDU. This information is obscured from the queuing discipline layer. The Linux kernel provides common abstractions and functionalities for the MAC protocols, but it is the responsibility of the driver to do the actual formation and handling of the A-MPDUs.
 
 To bypass this gap in communication, we log all the required details at the driver in the socket buffer (sk\textunderscore buff) (structure which contains all the meta details associated with the packet viz. IP header, MAC header, data, rate information etc.). Whenever a Block ACK is received, the driver frees the memory assigned to the socket buffers whose packets have been ACKed using the consume\textunderscore skb function. We monitor the calls to this function using the trace points (another abstraction in Linux kernel which allows the programmer to gain insights about the system by inserting callbacks). We then use the information extracted from the socket buffer to calculate the link rate; the queue size is available at the queuing discipline; with all the required ingredients, we calculate the fraction of packets to be marked and use a credit based system to do the supposedly probabilistic marking in a deterministic fashion.
 
 %\todo{assuming block ACKs are explained earlier, I think we can have a brief overview of 802.11n (also we can see if 802.11 ac is quite similar then we can say it can be implemented in a similar way for that as well.)}
 
 Alternatively, we could have done all the processing and marking at the driver itself, but we chose to do the marking in the queuing discipline because of ease of implementation, driver agnostic implementation and ease of setting and changing algorithm parameters using traffic control (tc - utility in Linux distributions which allows a user to add, remove and  reorganize queuing disciplines).
 
 Note that while our implementation is in MAC 802.11 n, our solution is applicable to MAC 802.11 ac, as well. Our link rate calculation was described in the scenario where users have a shared queue. In case users are isolated by a scheduler using per-user queues (e.g., wifi router air-time fairness), the marking for each user should be done independently by calculating per-user link rate.
 
 

==> wifi2.tex <==
%%%%% IMPLEMENTATION DETAILS
%
%and implement a method for estimating link capacities on a Wi-Fi router, which incorporates MAC 802.11n-specific properties and assumes a single queue \pg{across users (the dominant queuing strategy on commodity routers). Our method works even if the Wi-Fi router is not backlogged.} Similarly, a cellular base station implementing ABC can use resource allocation information \pg{to calculate the target rate}. Base stations typically employ per-user queues for isolation, so target rate calculations should consider per-user link capacities and queuing delay measurements. This strategy preserves the inter-user fairness provided by the base station scheduler.\footnote{This approach also applies to Wi-Fi routers that use per-user scheduled queues.} \pg{The 3GPP technical specification for LTE~\cite{3GPP} describes how to calculate the per user-link capacity at the base station.}

%Selecting the calculation window involves a tradeoff. Small time windows handle quickly varying link rates, but windows that are too short can suffer from incorrect rate estimates. The window duration should be selected to be larger than the average inter-schedule time of a user at the router. At cellular network base stations, this corresponds to windows being larger than $\frac{N \cdot S}{M}$, where $N$ is the number of active users, $S$ is the sub-frame size ($\approx$ 1 ms for LTE), and $M$ is the number of ``resource blocks'' per sub-frame. We use a window size of 20 ms for our trace-driven cellular network experiments. For Wi-Fi, we observe that MAC 802.11n inter-schedule times can be as high as 20 ms (Figure~\ref{fig:ampdu_burst}), so we use a window duration of 40 ms.



\section{Wi-Fi Implementation}
\label{s:wifi}

In this section, we describe our implementation of \name on a \pg{commodity  NETGEAR WNDR 3800} Wi-Fi 802.11 n router. The primary challenge lies in computing link rates for \name's target rate estimation given the semantics of MAC 802.11n packet transmissions. 
%We will first describe our link rate estimation approach for Wi-Fi, and then discuss implementation details.



\subsection{Calculating Link Rates}

We assume that users share a single bottleneck router queue, which is the dominant queuing strategy for Wi-Fi routers today. The link rate is defined as the aggregate throughput that would be achieved across all users when the router is backlogged (i.e., not empty). We first describe our solution assuming a single user and then expand it to multiple users.

\textbf{Challenges:} One must handle several protocol-specific properties of the Wi-Fi MAC layer. A strawman would be to estimate link rates based on the bitrates of transmitted packets. Unfortunately, this will overestimate the link rate as packet transmission times are governed not only by bitrates, but also by delays for additional tasks (e.g., channel contention) and retransmissions. \pg{An alternative approach would be to use the fraction of time that the router queue was backlogged as a proxy for link utilization and compute link rate as the ratio of current throughput and link utilization.} Unfortunately, the Wi-Fi MAC's packet batching confounds this idea. Wi-Fi routers transmit packets (frames) in batches, and only support a single outstanding batch; subsequent batches cannot be transmitted until an ACK (acknowledging all packets in a batch) has been received. Thus, routers may accumulate packets while waiting for an ACK; this queue buildup does not necessarily imply that the link is \pg{fully} utilized. Thus, accurately measuring link rates on a Wi-Fi 802.11n router requires a detailed consideration of Wi-Fi's packet transmission protocols. 

\textbf{\pg{Understanding Wi-Fi 802.11 n:}} In 802.11n, data frames, also known as MAC Protocol Data Units (MPDUs), are transmitted in batches called A-MPDUs (Aggregated MPDUs).
The maximum number of MPDUs that can be included in a single A-MPDU ($M$) is separately negotiated by each receiver and the router. When a given user is not backlogged\pg{, the router might not have enough packets to send a full sized A-MPDU and will instead use} an A-MPDU size $x < M$. Upon receiving an A-MPDU, a receiver responds with a Block ACK that acknowledges each individual MPDU in the A-MPDU. Thus, at a time $t$, given an A-MPDU size of $x$ frames, a frame size of $S$,\footnote{For simplicity, we assume that all frames are of the same size, though our formulas can be generalized in a straightforward manner for varying frame sizes.} and an ACK inter-arrival time (i.e., the time between receptions of consecutive block ACKs) of $T_{IA}(x,t)$, \pg{the instantaneous throughput, $cr(t)$, can be given by}

\begin{equation}
     cr(t) = \frac{x . S}{T_{IA}(x,t)}.
     \label{eq:inst_throughput}
\end{equation}

We can further break down the duration that routers spend between block ACKs.
Part of this time is spent performing ``overhead'' tasks including physically receiving an ACK, contending for the shared channel, and transmitting the physical layer preamble~\cite{ginzburg2007performance}. Each of these overhead tasks is independent of the A-MPDU size; as a result, we refer to the overhead time spent on these tasks using a separate term $h(t)$. \pg{If $R$ is the bitrate used for transmission, the router's ACK inter-arrival time can be given by}
\abovedisplayskip
 \begin{align}
     T_{IA}(x,t) \;&=\; \frac{x . S}{R} + h(t).
     \label{eq:inter_ack}
 \end{align}
  \belowdisplayskip
 \pg{When the user is backlogged, the router will transmit A-MPDUs of the maximum size (i.e., $M$ frames), and the instantaneous throughput (Eq. (~\ref{eq:inst_throughput})) will be equal to the link capacity. However, if the user is not backlogged and A-MPDUs only include $x < M$ frames, how can the router estimate the link capacity? Our approach is to calculate $\hat{T}_{IA}(M,t)$, estimated ACK inter-arrival time if the router could have included $M$ frames in the last A-MPDU (rather than only including the $x$ frames that the user had provided). Using $\hat{T}_{IA}(M,t)$, we can estimate the link capacity as}
\abovedisplayskip
  \begin{align}
    \hat{\mu} = \frac{M .  S}{\hat{T}_{IA}(M,t)}. 
         \label{eq:capacity_backlog}
  \end{align}
 \belowdisplayskip
 
 \if 0
 When the user is backlogged, the router will transmit A-MPDUs of the maximum size (i.e., $M$ frames), and we can estimate the link capacity as
  \begin{align}
    \hat{\mu} = \frac{M . S}{\hat{T}_{IA}(M,t)}. 
         \label{eq:capacity_backlog}
  \end{align}
However, if the user not backlogged and A-MPDUs only include $x < M$ frames, how can the router estimate the link capacity? Using Eq. (~\ref{eq:capacity_backlog}) directly would underestimate the link capacity as the router could have included $M$ frames in the last A-MPDU (rather than only including the $x$ frames that the user had provided).
\fi



 \begin{figure}[t]
     \centering
     \includegraphics[width=\columnwidth]{images/ampdu.pdf}
     \vspace{-8mm}
     \caption{\small {\bf Inter-ACK time vs A-MPDU size ---} Inter-ACK for a given A-MPDU exhibits variation. The solid black line represents the average Inter-ACk time for  given A-MPDU. The slope of the line is $S/R$.}
     \label{fig:ampdu_burst}
     \vspace{-4mm}
\end{figure}

To accurately estimate the link capacity, or equivalently $\hat{T}_{IA}(M,t)$, when a user is not backlogged, we turn to the relationship between A-MPDU size and ACK inter-arrival time. \Fig{ampdu_burst} illustrates this relationship for a sender who transmits packets below the average Wi-Fi link capacity. There are two key properties to note. First, for a given A-MPDU size, ACK inter-arrival times vary due to overhead tasks~\cite{ginzburg2007performance}. Second, because the overhead time and A-MPDU size are independent (Equation~\ref{eq:inter_ack}), connecting the average values of ACK inter-arrival times across all considered A-MPDU values will produce a line with slope $S/R$. Using this independence, we can use Equation~\ref{eq:inter_ack} to estimate the ACK inter-arrival time for a backlogged user as
\abovedisplayskip
 \begin{align}
    \hat{T_{IA}}(M,t) \;&=\;  \frac{MS}{R} + h(t)\nonumber\\
    \hat{T}_{IA}(M,t) \;&=\; T_{IA}(x,t) + \frac{(M - x) S}{R}.
    \label{eq:inter-ack-time}
 \end{align}
  \belowdisplayskip
This equation ensures that $T_{IA}(x,t) \leq \hat{T_{IA}}(M,t)$. Additionally, since \name cannot set a target rate to be greater than twice the current rate, we cap the predicted link rate with $T_{IA}(x,t) \leq \hat{T}_{IA}(M,t) \leq 2 . T_{IA}(x,t)$. We can then use these estimates of ACK inter-arrival times to estimate link capacity for a backlogged user with Equation~\ref{eq:capacity_backlog}. This computation occurs for each A-MPDU transmission, and we compute a weighted moving average of link capacity using these values; our implementation uses a sliding time window of 40 ms.

\textbf{Multiple Users:} To support a scenario where multiple users share the bottleneck router's queue, we compute an aggregate link rate across all users. In particular, we can use Eq. (~\ref{eq:inter-ack-time})~and~(\ref{eq:capacity_backlog}) to compute the link capacity for each A-MPDU transmission. Recall that routers transmit only a single A-MPDU at a time. Thus, even though users can negotiate different A-MPDU values with a router, link rate calculations can occur in a user-independent way by solely considering the size of each A-MPDU transmission.


 \begin{figure}[t]
     \centering
     \includegraphics[width=\columnwidth]{images/prediction.pdf}
     \vspace{-8mm}
     \caption{\small {\bf Wi-Fi Link Rate Prediction ---} \name router link rate predictions for a user that was not backlogged and sent traffic at multiple different rates over 3 distinct Wi-Fi links. Horizontal lines represent the true link capacity, solid lines summarize the \name router's link capacity prediction (each point is an average over 30 seconds of predictions), and the dashed slanted line represents the prediction rate caps. \name's link rate predictions are within 5\% of the ground truth across all sending rates.}
     \label{fig:prediction}
     \vspace{-4mm}
\end{figure}

\textbf{Evaluating Link Rate Estimates:} To evaluate the accuracy of our link rate estimates, we had a single user send traffic through our modified \name router (implementation described below) at multiple different fixed rates (i.e., offered loads) over three distinct Wi-Fi links; all send rates were below the corresponding link capacities.
\Fig{prediction} summarizes the accuracy of the \name router's link rate estimates. As shown, our \name Wi-Fi router is able to predict link rates within 5\% of the observed link capacities.

\subsection{Implementation Details}

We implemented \name as a Linux queuing discipline (qdisc) kernel module using OpenWrt, an open source operating system for embedded networked devices~\cite{openwrt}. We used a NETGEAR WNDR 3800 router (which uses an ath9k driver), configured to 802.11n. However, we note that our implementation is portable as OpenWrt is supported on numerous commodity Wi-Fi routers.

An \name router must be able to estimate link capacities, compute target rates, and mark packets as accelerates or brakes. \name's WiFi link rate prediction strategy exploits the inner workings of the MAC 802.11n protocol, and thus requires fine-grained values at this layer. In particular, the \name qdisc must know A-MPDU sizes, Block ACK receive times, and packet transmission bitrates. Unfortunately, these values are not natively exposed to Linux router qdiscs, and instead are only available at the network driver. To bridge this gap, we modified the router to log the relevant MAC layer data in the cross-layer socket buffer data structure (skb) that it already maintains per packet. Each time a Block ACK is received, the driver frees the memory which houses the socket buffer for each ACKed packet. We use Linux tracepoints to monitor all such events, and extract the necessary MAC-layer data for \name's link rate estimation.

An alternative design choice would be to estimate link rates directly in the network driver because MAC-layer data is readily available. However, we chose to implement \name as a qdisc for increased portability and ease of use (i.e., enabling or disabling qdiscs is straightforward using tools like \texttt{tc}). 
